Triangle and Four Cycle Counting with Predictions in Graph Streams

We propose data-driven one-pass streaming algorithms for estimating the number of triangles and four cycles, two fundamental problems in graph analytics that are widely studied in the graph data stream literature. Recently, (Hsu 2018) and (Jiang 2020) applied machine learning techniques in other data stream problems, using a trained oracle that can predict certain properties of the stream elements to improve on prior "classical" algorithms that did not use oracles. In this paper, we explore the power of a "heavy edge" oracle in multiple graph edge streaming models. In the adjacency list model, we present a one-pass triangle counting algorithm improving upon the previous space upper bounds without such an oracle. In the arbitrary order model, we present algorithms for both triangle and four cycle estimation with fewer passes and the same space complexity as in previous algorithms, and we show several of these bounds are optimal. We analyze our algorithms under several noise models, showing that the algorithms perform well even when the oracle errs. Our methodology expands upon prior work on "classical" streaming algorithms, as previous multi-pass and random order streaming algorithms can be seen as special cases of our algorithms, where the first pass or random order was used to implement the heavy edge oracle. Lastly, our experiments demonstrate advantages of the proposed method compared to state-of-the-art streaming algorithms.

==> Learning Augmented Triangles ICLR 22/OldStuff/CMUGang/experiment.tex <==
\section{Experiments}
\label{sec: experiments}
We perform our triangle counting experiments on the following two networks:
\begin{itemize}[topsep = 1 pt]
\setlength{\itemsep}{1pt}
\setlength{\parsep}{0pt}
\setlength{\parskip}{0pt}

    \item \textbf{Twitch}\cite{rozemberczki2019}: A user-user social network of gamers who stream in a certain language. Vertices are the users themselves and the links are mutual friendships between them. Each vertex contains a binary vector of features, based on the games the user played and liked, location of the user, and the user's streaming habits. The entire dataset contains six network graphs for six different languages, and the one that is used for testing our algorithm contains 6549 nodes and 112666 edges.
    % \footnote{http://snap.stanford.edu/data/twitch-social-networks.html}
    \item \textbf{Wikipedia}\cite{MM11}: This is a co-occurrence network of words appearing in the first million bytes of the Wikipedia dump. The network has 4777 nodes, 92406 edges, and 40 different labels associated.
\end{itemize}
\textbf{Experimental Setup}: %The experiment setting is as follows: 
For each of the two networks, we randomly remove $50\%$ of the total edges to be the training data set, and use the remaining edges as the testing data set. For the Twitch network, our set of links that we will try to predict are between two nodes that have a common neighbor in the training network, but do not form a link in the training network. This is about 3.8 million pairs, and we call this the candidate set. We do this for memory considerations. For the remaining node pairs, we set the probability they form a link to be $0$. For the Wikipedia network, we randomly select a link candidate set of size $20$ times the number of edges (about $1$ million pairs) from the entire set of testing links. These link candidate sets will be used by the oracle to determine heaviness. 

% A brief results summary?

\textbf{Training of the Oracle}: Our oracle is based on Link Prediction, where the task is to
estimate the likelihood of the existence of edges or to find missing links in the network. Here we use the method and code proposed in~\cite{ZC18}. For each target link, it will extract a local enclosing subgraph around a node pair, and use a Graph Neural Network to learn general graph structure features for link prediction. For the Twitch network, we use all the training links as the training data for the graph neural network, while for the Wikipedia network, we use $30\%$ of the training links as the training data due to memory limitations. Then, we use this network to do our prediction for all links in our candidate sets for the two networks.

Now we are ready to build our heavy edge oracle. For the adjacency list model, when we see the edge $uv$ in the stream, we know all the neighbors of $u$, and hence, we only need to predict the neighbors of $v$. Let $\mathrm{deg}(v)$ be the degree of $v$ in the training graph. The training graph and testing graph are randomly split. Hence, we can use the training set to provide a good estimation to the degree of $v$.  
Next, we choose the largest $\mathrm{deg}(v)$ edges incident to $v$ from the candidate set, in terms of their predicted likelihood given by the the neural network, as our prediction of $N(v)$, which leads to an estimate of $R_{uv}$. For the arbitrary order model, we use the same technique as above to predict $N(u)$ and $N(v)$, and estimate $N_{uv}$. 

% We show the accuracy of the oracle in Appendix~\ref{appendix:F}.
\begin{figure*}[ht]

\centering
\begin{minipage}{0.45\textwidth}
\vspace{-0.3cm}
\includegraphics[width=7cm]{images/twitch_adj_new.png}
%\hfill
\end{minipage}
\begin{minipage}{0.45\textwidth}
\vspace{-0.3cm}
\includegraphics[width=7cm]{images/Wikipedia_new.png}
\end{minipage}
\caption{Estimation error in the adjacency list model. The left is for Twitch and the right is for Wikipedia.}
\label{fig:1}
\end{figure*}

\begin{figure*}[ht]

\centering

\begin{minipage}{0.45\textwidth}
\vspace{-0.4cm}
\includegraphics[width=7cm]{images/twitch_arb.png}
%\hfill
\end{minipage}
\begin{minipage}{0.45\textwidth}
\vspace{-0.4cm}
\includegraphics[width=7cm]{images/Wikipedia_arb.png}
\end{minipage}

\caption{Estimation error in the arbitrary order model. The left is for Twitch and the right is for Wikipedia.}
\label{fig:2}

\end{figure*}
\subsection{Adjacency List Model}

In the adjacency list model, we compare our learning-based algorithms with the sampling-based algorithms in~\cite{MVV16} by fixing the sampling rate $p$ and comparing the multiplicative error of these two algorithms. 
For the sampling-based algorithm, we know when $R_{uv} \ge \epsilon^{-2} / p$, and so we can obtain a $(1 \pm \epsilon)$-approximation to $R_{uv}$ using the edges we have sampled. However, it is not easy to determine the optimal threshold for $R_{uv}$. To make it easier to compare, we assume that one can obtain the exact value of $R_{uv}$ when $R_{uv} \ge 5 / p$ for the sampling-based algorithm. This assumption will only make the results of the sampling-based algorithm better. 
For the learning-based algorithm, we set the $k = M / 10$ edges with the highest predicted $R_{uv}$ values to be the heavy edges, and store them during the stream, where $M$ is the expected space complexity (i.e., we use $10\%$ of the total space for storing the heavy edges). For the remaining edges, we use a similar sampling-based method. Note that it is impossible to know the $k$-heaviest edges before we see all the edges in the stream. However, in our implementation we can maintain the $k$ heaviest edges we currently have seen so far, and evict the smallest edge in the set when a new heavy edge is predicted by the oracle. We also consider the multi-layer sub-sampling algorithm mentioned in Section~\ref{sec:adj_mul}, which uses more information from the oracle. For this algorithm, we use $10\%$ of the total space for storing the top $k = M / 10$ edges, $20\%$ of the space for sub-sampling the edges $xy$ for which the oracle predicts $R_{xy} \ge 10$ (there are about $10^3$ such edges in both networks), and $70\%$ of the space for sub-sampling the remaining edges. 

The results are shown in Figure~\ref{fig:1}. We plot the estimation error vs. the expected number of edges we store (computed by the sampling rate) where the error takes an average over 1000 independent trials and all trials share a same node arrival order. From the plots we can see our learning-based algorithm can reduce $20\%$-$30\%$ error in all cases for the Twitch network and $30\%$-$40\%$ error for the Wikipedia network. Compared to the learning-based algorithm that just uses the oracle to select the top edges, our multi-layer sampling algorithm can still reduce error by $20\%$-$30\%$ in the Twitch network and reduce error by $10\%$-$20\%$ in the Wikipedia network. We also plot the curve when the oracle is perfectly accurate, and we can see that the performance of our trained oracle is very close to the ideal oracle.

\subsection{Arbitrary Order Model}

In the arbitrary order model, we compare our learning-based algorithm with the one-pass edge sampling algorithm mentioned in section~\ref{sec:arbitrary_triangle_intuition}. In both networks, we say an edge $uv$ is a heavy edge if the prediction value $N_{uv} \ge 60$, which corresponds roughly to the top $100$ edges in the Twitch network and top $200$ in Wikipedia network. For the heavy edge $uv$, we use the prediction $\hat{N}_{uv}$ as our estimate of $N_{uv}$ and $\sum_{uv \textnormal{ is heavy}} N_{uv}$ as our estimate of the number of triangles that have at least one heavy edge (this may cause some triangles to be counted more than once, but the number of the heavy edges is small so we ignore such double counting). We then count the triangles with three light edges with the same edge sampling algorithm. 

The results are shown in Figure~\ref{fig:2}. We plot the estimation error vs. the expected number of edges stored, where the error is calculated by averaging over 100 independent trial streams, each with a random arrival order. From the plot we can see that for the Twitch network, our learning-based algorithm can reduce the error by $10\%$-$20\%$. For the Wikipedia network, the learning-based algorithm can reduce the error by $20\%$-$35\%$.

We also study the relationship between the accuracy and the threshold $k$ we set in the experiments. The results are in Appendix~\ref{appendix:E}.


==> Learning Augmented Triangles ICLR 22/OldStuff/CMUGang/introduction.tex <==

\section{Introduction}
Counting the number of cycles is an extremely important problem in the graph stream model, especially with the special case of counting triangles being one of the most widely studied problems \cite{AGD08, BC17, S13, Kolountzakis_2010, Yossef}. There are a wide range of applications for triangle counting in graph streams, including discovering motifs in protein interaction networks \cite{Milo824}, understanding social networks \cite{Welles10}, and evaluating large graph models \cite{Leskovec08}. It is also closely connected to the field of fine-grained complexity, where studies involve various computational models such as distributed shared-memory and MapReduce \cite{S13, AGD08}. More recently, attention has been focused on the more general problem of counting larger cycles and subgraphs \cite{BC17, KJM19}. 

While detecting whether a graph contains a triangle or four-cycle is not possible in sublinear space with constant probability of success, a lot of work has been focused on computing a $(1 \pm \epsilon)$-approximation to the subgraph count $T$ using a small space randomized algorithm. A common difficulty in designing these algorithms is that the edges that are involved in a lot of triangles or four-cycles, i.e., the \textit{heavy} edges, are not known in advance. For a sub-sampling algorithm, these edges are often the key to accurate estimation, and people have developed multiple techniques to determine whether an edge is heavy such as processing a smaller subset of the stream as an oracle in the random order model \cite{McGregor2020, BS20} or using more passes \cite{MVV16}. 

Recently, machine learning techniques were incorporated into the data stream model, with the training of a heavy-hitter oracle, based on the observation that many underlying patterns in real world data sets such as the heavy link in a network does not change from day-to-day \cite{hsu2018}. It turns out that with the assistance of such a learning-based supporting oracle, a wide range of significant problems in big data processing, including estimating the number of distinct elements, computing the $F_p$-Moment, calculating the $(k,p)$-Cascaded Norm, support estimation, and nearest neighbor search, can all achieve better or even optimal space bounds, see, e.g., \cite{Jiang2020, EINR+2021, Dong2020}. 

One may wonder whether such techniques can be applied to the problem of subgraph counting. Namely, 
\begin{quote}
\em   
Is it possible to train a heavy edge oracle, and how does it improve the space complexity of subgraph counting in the graph stream model?
\end{quote}
% We consider estimating triangles and four cycles in the following two graph stream models:
% \begin{itemize}
%     \item 
%     Adjacency List Model: the edges incident to the same node arrive together.
%     \item
%     Arbitrary Order Model: the edges arrive in arbitrary order. 
% \end{itemize}
\subsection{Our Results and Comparison to Previous Work}

There are two major graph edge streaming models: the adjacency list model and arbitrary order models.
We show that the training of a heavy edge oracle is possible in practice, and it can lead to new algorithms that greatly improve the space complexity of triangle and four-cycle counting under both models.

\textbf{Adjacency List Model}. In the adjacency list model, the edges incident to the same node arrive together.
The best existing one-pass, $(1 \pm \epsilon)$-approximation algorithm for triangle counting has space complexity $\tilde{O}(\epsilon^{-2} m/\sqrt{T})$\footnote{ We use $\tilde{O}(f)$ to denote $O(f \mathrm{polylog}(f))$} \cite{MVV16}. Our first result is as follows: 

\textbf{Theorem~\ref{theorem_adjacency}}
\textit{There exists a one-pass algorithm with space complexity $\tilde{O}( \min(\epsilon^{-2}m^{2/3}/T^{1/3}, \epsilon^{-1} m^{1/2}))$ in the adjacency list model using a learning-based oracle that returns a $(1 \pm \epsilon)$-approximation to T with probability $7 / 10$. \footnote{the success probability can be replaced by $1 / \delta$ by running $\log(1/\delta)$ copies of the algorithm and taking the median.}  }


We also study the case when the oracle cannot only indicate an edge is heavy or not, but give an  $\alpha$-approximation to the value of the heavy edges. 
%We also show a lower bound for this setting.
%and show that a lower order bound could be achieved in theory.

\textbf{Arbitrary Order Model}. In the arbitrary order model, the edges arrive in the stream in an arbitrary order. 
In this model, we present a one-pass algorithm for triangle counting and another one-pass algorithm for four cycle counting, both reducing the number of passes from the algorithms with the currently best known space complexity. 

For triangle counting in this model, the best known space complexity for a general graph is $\tilde{O}(\epsilon^{-2}m^{3/2}/T)$ with three passes, or $\tilde{O}(\epsilon^{-2}m/\sqrt{T})$ using two passes \cite{MVV16}. Other results often contain specific parameters of the graph, including an $\tilde{O}(\epsilon^{-2}(m/\sqrt{T} + m \Delta_E / T))$ space bound using one pass\cite{PT12}, an  $\tilde{O}(\epsilon^{-2}(m/T^{2/3} + m \Delta_E / T + \sqrt{\Delta_V} / T))$ space bound using one pass\cite{KP17}, where $\Delta_E$ and $\Delta_V$ mean the maximum number of triangles sharing an edge or a vertex, respectively, and an almost tight bound of $\Tilde{O}(\mathrm{poly}(\epsilon^{-1})m\kappa/T)$, where $\kappa$ is the degeneracy of the graph, but requiring a constant number of passes \cite{BS20}. Our next result is as follows: 

\textbf{Theorem~\ref{theorem_arbitrary}}
\textit{There exists a one-pass algorithm with space complexity $\tilde{O}(\epsilon^{-2}\max(m/\sqrt{T}, \sqrt{m}))$ in the arbitrary order model using a learning-based oracle that returns a $(1 \pm \epsilon)$-approximation to T with probability at least $7 / 10$.
}

We also show a lower bound for this setting(Theorem~\ref{thm:lower_bound_arbitrary}).

For four cycle counting, the best existing bound for a $(1 \pm \epsilon)$-approximation is $\tilde{O}(\epsilon^{-4}m/T^{1/2})$ using 2 passes and $\tilde{O}(\epsilon^{-2}m/T^{1/3})$ using 3 passes \cite{McGregor2020, SV20}. We design our algorithm based on the 3-pass algorithm with a trained oracle for predicting heavy edges. We show:

\textbf{Theorem~\ref{theorem_four_cycle}}
\textit{
There exists a one-pass algorithm with space complexity $\tilde{O}(T^{1 / 3} + \epsilon^{-2}m / T^{1/3})$ in the arbitrary order model using a learning-based oracle that returns a $(1 \pm \epsilon)$-approximation to $T$ with probability at least $7 / 10$.}

We refer the reader to Table~\ref{comparison-table} for a summary of our results in comparison to prior work.

\textbf{Experiments.}
We conduct experiments to verify our results for triangle counting using two real world networks: a Twitch user-user social network and a word co-occurrence network from Wikipedia. In the training of the heavy edge oracle, we apply the method of link prediction \cite{ZC18}. 
%In particular, we first train a degree predictor for each vertex, and upon seeing edge $xy$, we perform link prediction on a target set of vertices to estimate whether $xy$ have a large number of common neighbors, which serves as our heavy edge oracle. 
More details of our experiments will be discussed in Section~\ref{sec: experiments}.

We found that in the adjacency list model, when using the same amount of memory, our learning-augmented algorithm reduces the error by $20\%$-50$\%$ compared to the baseline algorithm without learning. In the arbitrary order model, our algorithm can reduce the error by around $20\%$ when using the same amount of space compared to the non-augmented %$\tilde{O}(m/\sqrt{T})$ algorithm while using only 
$\tilde{O}(\epsilon^{-2}(m/\sqrt{T} + m \Delta_E / T))$ one-pass edge sampling algorithm. 

\begin{table}[t]
% \vspace{-3pt}
\caption{Our results compared to existing algorithms}
\label{comparison-table}

\begin{center}

\begin{tabular}{ | m{4em} | m{8em}| m{8em} | } 

\hline
Problem & Previous Results & Our Results \\
\hline
\multirow{2}{4em}{Triangle, Adjacency} & \multirow{2}{8em}{$\tilde{O}(\epsilon^{-2} m/\sqrt{T})$} &  $\tilde{O}(\min(\epsilon^{-2}\frac{m^{2/3}}{T^{1/3}},$ \\
& & $\epsilon^{-1} m^{1/2}))$ \\
\hline

\multirow{12}{4em}{Triangle, Arbitrary}& 
\multirow{2}{8em}{$\tilde{O}(\epsilon^{-2}m^{3/2}/T)$, 3-pass}& \multirow{12}{8em}{$O(\epsilon^{-2}\max(m/\sqrt{T},$ $m^{1/2}))$, 1-pass} \\
& & \\
& \multirow{2}{8em}{$\tilde{O}(\epsilon^{-2}m/\sqrt{T})$, 2-pass} & \\
& & \\
& \multirow{3}{8em}{$\tilde{O}(\epsilon^{-2}(m/\sqrt{T} + m \Delta_E / T))$, 1-pass} & \\
& & \\
& & \\
& \multirow{3}{8em}{$\tilde{O}(\epsilon^{-2}(m/T^{2/3} + m \Delta_E / T + \sqrt{\Delta_V} / T))$, 1-pass} & \\
& & \\
& & \\
& \multirow{3}{8em}{$\Tilde{O}(\mathrm{poly}(\epsilon^{-1})m\kappa/T)$, multi-pass} & \\
& & \\
& & \\
\hline

\multirow{6}{4em}{4-cycle, Arbitrary} &
\multirow{3}{8em}{$\tilde{O}(\epsilon^{-4}m/T^{1/2})$, 2-pass} &
\multirow{6}{8em}{$\tilde{O}(T^{1/3} + \epsilon^{-2}m/T^{1/3})$, 1-pass} \\
& & \\
& & \\
& \multirow{3}{8em}{$\tilde{O}(\epsilon^{-2}m/T^{1/3})$, 3-pass} & \\
& & \\
& & \\
\hline
\end{tabular}

\end{center}
\vspace{-20pt}
\end{table}

==> Learning Augmented Triangles ICLR 22/OldStuff/CMUGang/new_value_prediction.tex <==
\section{New Value Prediction Oracle for Adjacency List Model}
\label{sec:value_oracle}

In this section, we consider the following oracle model.

\textbf{Definition~\ref{def:value_oracle}}
\textit{
A value-prediction oracle with parameter $(\alpha,\beta)$ can, for a given edge $e$, 
%indicate if (i) $R_{xy} \le T / \beta$, or (ii) $R_{xy} > T / \beta$, and 
output a value $p(e)$ for which $\alpha t(e) + \beta \ge \mathbb{E}[p(e)]$, and $\mathbf{Pr}[p(e) < \frac{t(e) - \beta}{\lambda}] \le e^{-\lambda}$.
%$\alpha$-approximation of $R_{xy}$ .
}

Our algorithm is based on the following stability property of exponential random variables (see e.g.~\cite{Andoni17})

\begin{lemma}
\label{lem:exp_stable}
Let $x_1, x_2, ..., x_n > 0$ be real numbers, and let $u_1, u_2, ...u_n$ be i.i.d. standard exponential random variables with parameter $\lambda = 1$. Then we have that the random variable $\max(\frac{x_1}{u_1}, ..., \frac{x_n}{u_n}) \sim \frac{x}{u}$, where $x = \sum_i x_i$ and $u \sim \mathrm{Exp}(1)$.
\end{lemma}

\begin{lemma}
\label{lem:exp_median}
Let $r = O(\ln(1 / \delta) / \epsilon^{2})$ and $\epsilon \le 1/3$. If we take $r$ independent samples $X_1, X_2, ... , X_r$ from $\mathrm{Exp}(1)$ and let $X = \mathrm{median}(X_1, X_2, ..., X_r)$, then with probability $1 - \delta$, $X \in [\ln{2}(1-\epsilon), \ln{2}(1 + 5\epsilon)]$.
\end{lemma}
\begin{proof}
We first prove the following statement: with probability $1-\delta$, $F(X) \in [1/2-\epsilon, 1/2 + \epsilon]$, where $F$ is the cumulative density function of a standard exponential random variable.

Consider the case when $F(X) \le 1/2 - \epsilon$. We use the indicator variable $Z_i$ where $Z_i = 1$ if $F(X_i) \le 1/2 - \epsilon$ or $Z_i = 0$ otherwise. Notice that when $F(X) \le 1/2 - \epsilon$, at least half of the $Z_i$ are $1$, so $Z = \sum_i Z_i \ge r / 2$. On the other hand, we have $\mathbb{E}[Z] = r / 2 - r \epsilon$, by a Chernoff bound. We thus have 
\[
\mathbf{Pr}[|Z - \mathbb{E}[Z]| \ge \epsilon r] \le 2e^{-\epsilon^{2}r/3} \le \delta / 2\; .
\]
Therefore, we have with probability at most $\delta/2$, $F(X) \le 1/2 - \epsilon$. Similarly, we have that with probability at most $\delta / 2$, $F(X) \ge 1/2 + \epsilon$. Taking a union bound, we have that with probability at least $1-\delta$, $F(X) \in [1/2-\epsilon, 1/2 + \epsilon]$.

Now, condition on $F(X) \in [1/2-\epsilon, 1/2 + \epsilon]$. Note that $F^{-1}(x) = -\ln(1 - x)$, so if we consider the two endpoints of $F(X)$, we have 
\[
F^{-1} (1/2 -\epsilon) = -\ln(1/2 + \epsilon) \ge (1-\epsilon)\ln{2},
\]
and
\[
F^{-1} (1/2 +\epsilon) = -\ln(1/2 - \epsilon) \le (1+5\epsilon)\ln{2}.
\]
which indicates that $X \in [\ln{2}(1-\epsilon), \ln{2}(1 + 5\epsilon)]$.
\end{proof}

The algorithm is shown in Algorithm~\ref{alg:4}. For the light edges, from the assumption of the oracle we know that $R_{xy} \le T / \beta$, we can sub-sample with sampling rate $O(\epsilon^{-2} \beta)$ to estimate $T_L$. For the heavy edges, we can obtain an $\alpha$-approximation to $R_{xy}$ from the oracle at this time. As shown in our algorithm, we run $O(\epsilon^{-2})$ copies of the subroutine and we will show that each subroutine will output the maximum value of $R_{xy} / u_{xy}^i$ with high probability, where the $u_{e}^i$ are exponential random variables. From Lemma~\ref{lem:exp_stable} and Lemma~\ref{lem:exp_median} we can obtain $O(\epsilon^{-2})$ independent samples from $T_H / u$, where $u \sim \mathrm{Exp}(1)$, and after taking a median among all samples we can obtain a $(1 \pm \epsilon)$-approximation to $T_H$.

\begin{algorithm}[!h]
   \caption{Counting Triangles in the Adjacency List Model with a Value Prediction Oracle}
   \label{alg:4}
\begin{algorithmic}[1]
   \STATE {\bfseries Input:} Adjacency list edge stream and an value prediction oracle with parameter$(\alpha, \beta)$. 
   \STATE {\bfseries Output:} An estimate of the number $T$ of triangles.
   \STATE Initialize $X \leftarrow \emptyset$ and $H = O(\epsilon\alpha)$\; .
   %\STATE On :$H = O(T)$
   \FOR{$i = 0$ {\bf to} ${O(\epsilon^{-2})}$}
        \STATE $S^{i} \leftarrow \emptyset, Q^{i} \leftarrow \emptyset$, and $A^i \leftarrow 0 $ \; .
        % \STATE $v_i \leftarrow 0$ \textnormal{as the maximum value in $Q^i$} \; .
        % \STATE $w_i \leftarrow 0$ \textnormal{as the minimum value in $Q_i$} \;%\textnormal{as the evict threshold in $Q^i$} 
        \STATE \textnormal{Generate} $u_{xy}^i \sim \textrm{Exp}(1)$ for all $x$ and $y$ \; . 
   \ENDFOR
    \WHILE{seeing edges adjacent to $y$ in the stream} \STATE For all $ab \in S_L$: if $a, b \in N(y)$ then $C_{ab} \leftarrow C_{ab} + 1$\; 
    % \FOR{$i = 0$ {\bf to} ${O(\epsilon^{-2})}$}
    \STATE For all $ab \in S^i$: if $a, b \in N(y)$ then $C_{ab}^i \leftarrow C_{ab}^i + 1$\; 
    %  \ENDFOR
    \FOR{each incident edge $yx$}
    
    \IF{the oracle outputs \textsc{True}}
    \IF{$xy \in S_L$} 
        \STATE $A_l \leftarrow A_l + C_{xy}$ \;.
    \ELSE 
    \STATE With probability $p_l$, $S_L \leftarrow \{yx\} \cup S_L$ \;.
    \ENDIF
    \ELSE 
        \FOR{$i = 0$ {\bf to} ${O(\epsilon^{-2})}$} 
            \IF{$xy \in S^i$} 
            \STATE $A^i \leftarrow \max(A^i,  C_{xy}^i / u_{xy}^i)$ \;.
            \ELSE
            \STATE Let $\hat{R}_{yx}$ be the predicted value of $R_{yx}$.
            \STATE $Q^i \leftarrow Q^i \cup \{\hat{R}_{yx}/u_{yx}^i\}, S^i \leftarrow S^i \cup \{xy\}$
            \IF{$|Q| > k$}
            \STATE Let $ab$ be the edge for which $\hat{R}_{ab} / u_{ab}^i$ is the smallest item in $Q^i$
            \STATE $Q^i \leftarrow Q^i / \{\hat{R}_{ab}/u_{ab}^i\}, S^i \leftarrow S^i / \{ab\}$
            \ENDIF
            \ENDIF
    \ENDFOR
    
    \ENDIF
    \ENDFOR
    \ENDWHILE
    \FOR{$i = 0$ {\bf to} ${O(\epsilon^{-2})}$}
        \STATE $u^i \leftarrow \max(Q^i)$ and $v^i \leftarrow \min(Q^i)$  \; .
        \IF{$u^i > \alpha v^i$}
        \STATE $X \leftarrow X \cup \{A^i\}$
        \ENDIF
   \ENDFOR
    \STATE {\bfseries return:} $A_l / p_l + \mathrm{median}(X) / \ln{2}$ \; .
\end{algorithmic}
\end{algorithm}

\textbf{Theorem~\ref{thm:value_oracle}}
\textit{
Given an oracle with parameter $(\alpha, \beta)$, there exists a one-pass algorithm with space complexity $O(\epsilon^{-2} (m / \beta + \alpha + \log n(\log\log n)^2))$ in the adjacency list model that returns a $(1 \pm \epsilon)$-approximation to $T$ with probability at least $7 / 10$. 
}

\begin{proof}
For the light edges, from Lemma~\ref{lem:adjlist_light} we get that with probability at least $9/10$, 
\[
A_l / p_l = T_L \pm \epsilon T \;.
\]
Now we focus on estimating $T_H$. It is easy to see that for the $i$-th subroutine, $Q^i$ and $S^i$ sample the edge $xy$ for which $\hat{R}_{xy} / u_{xy}^i$ is among the current top $k$ values we have seen. At the end of the stream, $Q^i$ and $S^i$ sample edge $xy$ for which $\hat{R}_{xy} / u_{xy}^i$ is among the top $k$ largest values among all edges. If the edge $ab$, for which the true value $R_{ab} / u_{ab}^i$ is the maximum value among $E$, is included in $S^i$, then the output of the $i$-th subroutine will be a sample from $T_H / u$, where $u \sim \mathrm{Exp}(1)$. Recall that $\hat{R}_{xy}$ is an $\alpha$-approximation to $R_{xy}$, and hence we have that 
\[
\max_{xy \in E} \hat{R}_{xy} / u_{xy}^i \le \alpha \hat{R}_{ab} / u_{ab}^i \;,
\]
which means if $u_i \ge \alpha v_i$ ($u_i$ and $v_i$ are the maximum and minimum values in $Q^i$ after the stream), then $ab$ should be included in $S^i$.

From Claim~2.1 in~\cite{Andoni17}, for each subroutine $i$, in expectation there will be at most $O(\alpha)$ edges $wz$ satisfying 
\[
\max_{xy \in E} \hat{R}_{xy} / u_{xy}^i \le \alpha \hat{R}_{wz} / u_{wz}^i \;,
\]
Hence, using Markov's inequality, with probability at least $9 / 10$, $u_i > \alpha v_i$ holds for the $i$-th subroutine (this is because, at this time there are at most $O(\alpha)$ edges within an $\alpha$ factor of $\max_{xy \in E} \hat{R}_{xy} / u_{xy}^i$, and $v_i$ is the $k = l \alpha$ largest edge). Therefore, in expectation there will be at least a $9/10$-fraction of our total  $O(\epsilon^{-2})$ number of subroutines which can output a sample drawn from $T_H / u$. From Lemma~\ref{lem:exp_median}, we get that after taking a median, we obtain a $(1 \pm O(\epsilon))$-approximation to $T_H$.

Next we analyze the space complexity. For the light edges, we sample each edge with probability $O(\epsilon^{-2}/\beta)$, and hence the expected space we use is $O(\epsilon^{-2} m / \beta)$. For the heavy edges, we run $O(1/\epsilon^{2})$ subroutines and the number of edges each subroutine stores is $O(\alpha)$. From Theorem~5 in \cite{JW18}, generating the exponential random variables can be derandomized in $O(\epsilon^{-2} (\log n (\log\log n)^2))$ space. Therefore, we get that the total expected space we use is $O(\epsilon^{-2}(m / \beta + \alpha + \log n (\log\log n)^2))$.
\end{proof}

\begin{remark}
An alternative way to solve this problem is to divide the triangles into the intervals $[0, T/\beta], [2T/ \beta, 4T/ \beta],..., [2^i T/\beta, 2^{i+1} T / \beta], ...$ and put the edges into the intervals according to the predicted value the oracle gives. For the edges in interval $[2^i T / \beta, 2^{i + 1} T / \beta]$, we can sub-sample with rate $O(\epsilon^{-2} \alpha 2^{i + 1} /\beta )$. The total space we use will be $\tilde{O}(\epsilon^{-2} (m / \beta + \alpha \log n))$.
\end{remark}

==> Learning Augmented Triangles ICLR 22/OldStuff/MITGang/preamble.tex <==
%packages

\usepackage{amsthm}
\usepackage{mathtools} 
\usepackage{paralist}
\usepackage[colorlinks,urlcolor=blue,citecolor=blue,linkcolor=blue]{hyperref}
\usepackage{xcolor,soul}


%comments
\DeclareRobustCommand{\hltalya}[1]{{\sethlcolor{yellow}\hl{#1}}}
\newcommand{\tnote}[1]{\hltalya{[\textbf{T}: #1]}}

%theorems and proofs
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{notation}[theorem]{Notation}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{claim}[theorem]{Claim}
%\theoremstyle{remark}
\newtheorem{remark}{Remark}

%shortcuts
\newcommand{\eps}{\epsilon}
\newcommand{\mO}{\mathcal{O}_\theta}
\newcommand{\heavy}{\textsf{heavy}}
\newcommand{\light}{\textsf{light}}
\newcommand{\mT}{\mathcal{T}}
\newcommand{\mH}{\mathcal{H}}
\newcommand{\mS}{\mathcal{S}}
\newcommand{\oT}{\overline{T}}

%procedures
\newcommand{\AT}{\hyperref[AT]{\textup{\color{black}{\sf Approx-Triangles}}}}

%useful
\newcommand{\EX}{\textbf{\textrm{Ex}}}
\newcommand{\Var}{\textbf{\textrm{Var}}}
\newcommand{\Cov}{\textbf{\textrm{Cov}}}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\paren}[1]{\left(#1\right)}
\newcommand{\set}[1]{\left\{#1\right\}}
\newcommand{\sqb}[1]{\left[#1\right]}
\newcommand{\sucht}{\,\middle|\,}
\renewcommand{\th}{^{\textrm{th}}}
\newcommand{\poly}{\textrm{poly}}

==> Learning Augmented Triangles ICLR 22/additional_experiments.tex <==
\section{Additional Experimental Results}\label{sec:additional_experiments}
All of our graph experiments were done on a CPU with i5 2.7 GHz dual core and 8 GB RAM or a CPU with i7 1.9 GHz 8 core and 16GB RAM. The link prediction training was done on a single GPU.

\subsection{Dataset descriptions}
\begin{itemize}
    \item \textbf{Oregon:} $9$ graphs sampled over $3$ months representing a communication network of internet routers \cite{snapnets, oregon1}.
    \item \textbf{CAIDA:} $98$ graphs sampled approximately weekly over $2$ years, representing a communication network of internet routers \cite{snapnets, oregon1}.
    \item \textbf{Reddit Hyperlinks:} Network where nodes represent sub communities (subreddits) and edges represent posts that link two different sub communities \cite{snapnets, reddit}.  
    \item \textbf{WikiBooks:} Network representing Wikipedia users and pages, with editing relationships between them \cite{wikibooks}.
    \item \textbf{Twitch:} A user-user social network of gamers who stream in a certain language. Vertices are the users themselves and the links are mutual friendships between them. \cite{rozemberczki2019}
    \item \textbf{Wikipedia:} This is a co-occurrence network of words appearing in the first million bytes of the Wikipedia dump. \cite{MM11}
    \item \textbf{Synthetic Power law:} Power law graph sampled from the Chung-Lu-Vu (CLV) model with the expected degree of the $i$th vertex proportional to $1/i^2$ \cite{CLV}. To create this graph, the vertices are `revealed' in order. When the $j$th vertex arrives, the probability of forming an edge between the $j$th vertex and $i$th vertex for $i < j$ is proportional to $1/(ij)^2$.
\end{itemize}


\subsection{Details on link prediction oracle}\label{sec:prediction_oracle_details}

Our oracle for the Twitch and Wikipedia graphs is based on Link Prediction, where the task is to
estimate the likelihood of the existence of edges or to find missing links in the network. Here we use the method and code proposed in~\cite{ZC18}. For each target link, it will extract a local enclosing subgraph around a node pair, and use a Graph Neural Network to learn general graph structure features for link prediction. For the Twitch network, we use all the training links as the training data for the graph neural network, while for the Wikipedia network, we use $30\%$ of the training links as the training data due to memory limitations. For the Twitch network, our set of links that we will try to predict are between two nodes that have a common neighbor in the training network, but do not form a link in the training network. This is about 3.8 million pairs, and we call this the candidate set. We do this for memory considerations. For the remaining node pairs, we set the probability they form a link to be $0$. For the Wikipedia network, we randomly select a link candidate set of size $20$ times the number of edges (about $1$ million pairs) from the entire set of testing links. These link candidate sets will be used by the oracle to determine heaviness. Then, we use this network to do our prediction for all links in our candidate sets for the two networks. 

Now we are ready to build our heavy edge oracle. For the adjacency list model, when we see the edge $uv$ in the stream, we know all the neighbors of $u$, and hence, we only need to predict the neighbors of $v$. Let $\mathrm{deg}(v)$ be the degree of $v$ in the training graph. The training graph and testing graph are randomly split. Hence, we can use the training set to provide a good estimation to the degree of $v$.  
Next, we choose the largest $\mathrm{deg}(v)$ edges incident to $v$ from the candidate set, in terms of their predicted likelihood given by the the neural network, as our prediction of $N(v)$, which leads to an estimate of $R_{uv}$. For the arbitrary order model, we use the same technique as above to predict $N(u)$ and $N(v)$, and estimate $N_{uv}$. 

\subsection{Parameter Selection for Algorithm \ref{alg:4}}\label{sec:param}
We need to set two parameters for Algorithm \ref{alg:4}: $p$, which is the edge sampling probability, and $\theta$, which is the heaviness threshold. In our theoretical analysis, we assume knowledge of a lower bound on $T$ in order to set $p$ and $\theta$, as is standard in the theoretical streaming literature. However, in practice, such an estimate may not be available; in most cases, the only parameter we are given is a space bound for the number of edges that can be stored. To remedy this discrepancy, we modify our algorithm in experiments as follows.

First, we assume we only have access to the stream, a space parameter $Z$ indicating the maximum number of edges that we are allowed to store, and an estimate of $m$, the number of edges in the stream. Given $Z$, we need to 
designate a portion of it for storing heavy edges, and the rest for storing light edges. The trade-off is that the more heavy edges we store, the smaller our sampling probability of light edges would be. We manage this trade off in our implementation by 
reserving $0.3 \cdot Z$ of the edge `slots' for heavy edges. The constant $0.3$ is \emph{fixed} throughout all our experiments. We then set $p = 0.7 \cdot Z/m$. 
To improve the performance of our algorithm, we optimize for space usage by \emph{always} insuring that we are storing exactly $Z$ space (after observing the first $Z$ edges of the stream). To do so and still maintain our theoretical guarantees, we perform the following procedure. Call the first $Z$ edges of the stream the early phase and the rest of the edges the late phase. 

We always keep edges in the early phase to use our space allocation $Z$ and also keep track of the $0.3$-fraction of the heaviest edges. After the early phase is over, i.e., more than $Z$ edges have passed in the stream, if a new incoming edge is heavier than the lightest of the stored heavy edges, we replace the least heavy stored edge with the new arriving edge and re-sample the replaced edge with probability $p$. Otherwise, if the new edge is not heavier than the lightest stored edge, we sample the new incoming edge with probability $p$. If we exceed $Z$, the space threshold, we replace one of the light edges sampled in the early phase. Then similarly as before, we re-sample this replaced edge with probability $p$ and continue this procedure until one of the early light edges has been evicted. In the case that there are no longer any of the light edges sampled in the early phase stored, we replace a late light edge and then any arbitrary edge (again performing the re-sampling procedure for the evicted edge).

Note that in our modification, we only require our predictor be able to compare the heaviness between two edges, i.e., we do not need the predictor to output an estimate of the number of triangles on an edge. This potentially allows for more flexibility in the choice of predictors.

If the given space bound meets the space requirements of Theorem~\ref{thm:imperfect_arbitrary}, then the theoretical guarantees of this modification simply carry over from Theorem~\ref{theorem_arbitrary}: we always keep the heaviest edges and always sample light edges with probability at least $p$. In case the space requirements are not met, the algorithm stores the most heavy edges as to reduce the overall variance.


\subsection{Additional Figures from Arbitrary Order Triangle Counting Experiments}\label{sec:additional_figures_arbitrary}
Additional figures for our arbitrary order triangle counting experiments are given in Figures \ref{fig:space_additional} and \ref{fig:space_additional_rebuttal}.


\begin{figure}[!ht]
    \centering
    \subfigure[CAIDA $2007$ \label{fig:caida7_space}]{\includegraphics[scale=0.2]{images/caida7_space_neurips.pdf}} 
            \subfigure[Twitch \label{fig:twitch_space}]{\includegraphics[scale=0.2]{images/twitch_space_neurips.pdf}} 
    \caption{Error as a function of space for various graph datasets.  \label{fig:space_additional}}
\end{figure}

\begin{figure}[t]
    \centering
    \subfigure[CAIDA $2006$, Graph $\#20$ \label{fig:caida_add1}]{\includegraphics[scale=0.2]{images/caida6_space_iclr1.pdf}} 
    \subfigure[CAIDA $2006$, Graph $\#40$ \label{fig:caida_add2}]{\includegraphics[scale=0.2]{images/caida6_space_iclr2.pdf}} \\
    \subfigure[Oregon, Graph $\#3$ \label{fig:oregon_add1}]{\includegraphics[scale=0.2]{images/oregon1_space_iclr1.pdf}} 
    \subfigure[Oregon, Graph $\#7$ \label{fig:oregon_add2}]{\includegraphics[scale=0.2]{images/oregon1_space_iclr2.pdf}} \\
    \caption{Error as a function of space for various graph datasets.  \label{fig:space_additional_rebuttal}}
\end{figure}



\subsection{Experimental Design for Adjacency List Experiments}\label{sec:adjacency_experiments_info}
We now present our adjacencly list experiments. At a high level overview, similarly to the arbitrary order experiments, for our learning-based algorithm, we reserve the top $10\%$ of the total space for storing the heavy edges.
To do this in practice, we can maintain the heaviest edges currently seen so far and evict the smallest edge in the set when a new heavy edge is predicted by the oracle and we no longer have sufficient space.
We also consider a multi-layer sub-sampling version of the algorithm in Section~\ref{sec:adj_value_oracle}. Here we use more information from the oracle by adapting the sub-sampling rates of edges based on their predicted value. For more details, see Section \ref{sec:adjacency_experiments_info}. Our results are presented in Figure \ref{fig:space_adj_list} (with additional plots given in Figure \ref{fig:space_adj_list_additional}). Our algorithms soundly outperform the MVV baseline for most graph datasets. We only show the error bars for the multi-layer algorithm and MVV for clarity. Additional details follow.


We use the same predictor for $N_{xy}$ in Section~\ref{sec: experiments} as a prediction for $R_{xy}$. The experiment is done under a random vertex arrival order. For the learning-based algorithm, suppose $Z$ is the maximum number of edges that we are allowed to store. we set the $k = Z / 10$ edges with the highest predicted $R_{uv}$ values to be the heavy edges, and store them during the stream (i.e., we use $10\%$ of the total space for storing the heavy edges). For the remaining edges, we use a similar sampling-based method. Note that it is impossible to know the $k$-heaviest edges before we see all the edges in the stream. However, in the implementation we can maintain the $k$ heaviest edges we currently have seen so far, and evict the smallest edge in the set when a new heavy edge is predicted by the oracle. 

We also consider the multi-layer sub-sampling algorithm mentioned in Section~\ref{sec:adj_value_oracle}, which uses more information from the oracle. We notice that in many graph datasets, most of the edges having very few number of triangles attached to. Taking an example of the Oregon and CAIDA graph, only about 3\%-5\% of edges will satisfy $R_e \ge 5$ under a random vertex arrival order. Hence, for this edges, intuitively we can estimate them using a slightly smaller space.

For the implementation of this algorithm(we call it multi-layer version), we use $10\%$ of the total space for storing the top $k = Z / 10$ edges, and $70\%$ of the space for sub-sampling the edges that the oracle predict value is very tiny(the threshold may be slightly different for different datasets, like for the Oregon and CAIDA graph, we set the threshold to be 5). Then, we use $20\%$ of the space for sub-sampling the remaining edges, for which we call them the medium edges.

\subsection{Figures from Adjacency List Triangle Counting Experiments}\label{sec:additional_figures_adjacency}

\begin{figure}[!ht]
    \centering
    \subfigure[CAIDA $2006$ \label{fig:caida6_space_list}]{\includegraphics[scale=0.18]{images/Caida06_space_list.pdf}} 
    \subfigure[Wikipedia \label{fig:wikipedia_space_list}]{\includegraphics[scale=0.18]{images/Wikipedia_space_list.pdf}}
    \subfigure[Powerlaw \label{fig:random_space_list}]{\includegraphics[scale=0.18]{images/Powerlaw_space_list.pdf}} 
    \setlength{\belowcaptionskip}{-10pt}
    \caption{Error as a function of space in the adjacency list model.  \label{fig:space_adj_list}}
\end{figure}

Additional figures from the adjacency list triangle counting experiments are shown in Figure \ref{fig:space_adj_list_additional}. They are qualitatively similar to the results presented in Figure \ref{fig:space_adj_list} as the multi-layer sampling algorithm is superior over the MVV baseline for all of our datasets.
\begin{figure}[!ht]
    \centering
    \subfigure[Oregon \label{fig:oregon1_space_list}]{\includegraphics[scale=0.2]{images/Oregon_space_list.pdf}} 
    \subfigure[CAIDA $2007$ \label{fig:caida7_space_list}]{\includegraphics[scale=0.2]{images/Caida07_space_list.pdf}} 
    \subfigure[Wikibooks \label{fig:wiki_space_list}]{\includegraphics[scale=0.2]{images/Wikibooks_space_list.pdf}} \\
    \subfigure[Twitch \label{fig:twitch_space_list}]{\includegraphics[scale=0.2]{images/Twitch_space_list.pdf}}
    \caption{Error as a function of space for various graph datasets.  \label{fig:space_adj_list_additional}}
\end{figure}

\subsection{Accuracy of the Oracle}

In this section, we evaluate the accuracy of the predictions the oracle gives in our experiments. 
\paragraph{Value Prediction Oracle}: We use the prediction of $N_{xy}$ in Section~\ref{sec: experiments} as a value prediction for $R_{xy}(x \le_s y)$, under a fixed random vertex arrival order. The results are shown in Figure~\ref{fig:adj_oracle_error}. For a fixed approximation factor $k$, we compute the failure probability $\delta$ of the value prediction oracle as follows: $\delta = \# / m$, where $m$ is the number of total edges and $\#$ equals to the number of edges $e$ that $p(e) \ge k \alpha R_e + \beta$ or $p(e) \le \frac{1}{k} R_e - \beta$, respectively. Here we set $\alpha = 1, \beta = 10$ for all graph datasets. 

We can see for the smaller side, there are very few edges $e$ such that $p(e) \le \frac{1}{k}R_e - \beta$. This meets the assumption of the exponential decay tail bound of the error. For the larger side, it also meets the assumption of the linear decay tail bound on most of the graph datasets.

\begin{figure}[!ht]
    \centering
    \subfigure[Oregon \label{fig:oregon_error}]{\includegraphics[scale=0.2]{images/Oregon_error.pdf}} 
    \subfigure[CAIDA $2006$
    \label{fig:caida6_error}]{\includegraphics[scale=0.2]{images/Caida06_error.pdf}} 
    \subfigure[CAIDA $2007$
    \label{fig:caida7_error}]{\includegraphics[scale=0.2]{images/Caida07_error.pdf}} 
    \subfigure[Wikibooks \label{fig:wikibooks_error}]{\includegraphics[scale=0.2]{images/Wikibooks_error.pdf}}
    \subfigure[Twitch \label{fig:twitch_error}]{\includegraphics[scale=0.2]{images/Twitch_error.pdf}}
    \subfigure[Wikipedia \label{fig:wikipedia_error}]{\includegraphics[scale=0.2]{images/wikipedia_error.pdf}} \\
    \subfigure[Powerlaw \label{fig:random_error}]{\includegraphics[scale=0.2]{images/random_error.pdf}}
    \caption{Failure probability as a function of approximation factor $k$ for various graph datasets.  \label{fig:adj_oracle_error}}
\end{figure}

\label{sec:oracle_accuracy}


\subsection{Details on Oracle Training Overhead}

The overhead of the oracles used in our experiments vary from task to task. For the important use case illustrated by the Oregon and CAIDA datasets in which we are interested in repeatedly counting triangles over many related streams, we can pay a small upfront cost to create the oracle which can be reused over and over again. Thus, the time complexity of building the oracle can be amortized over many problem instances, and the space complexity of the oracle is relatively small as we only need to store the top $10\%$ of heavy edges from the first graph (a similar strategy is used in prior work on learning-augmented algorithms in \cite{hsu2019learning}). To give more details, for this snapshot oracle, we simply calculate the $N_e$ values for all edges only in the first graph. We then keep the heaviest edges to form our oracle. Note that this takes polynomial time to train. The time complexity of using this oracle in the stream is as follows: when an edge in the stream comes, we simply check if it’s among the predicted heavy edges in our oracle. This is a simple lookup which can even be done in constant time using hashing.

For learning-based oracles like the linear regression predictor, we similarly need to pay an upfront cost to train the model, but the space required to store the trained model depends on the dimension of the edge features. For the Reddit dataset with $\sim 300$ features, this means that the storage cost for the oracle is a small fraction of the space of the streaming algorithm. Training of this oracle can be done in polynomial time and can even be computed in a stream via sketching and sampling techniques which reduce the number of constraints from m (number of edges) to roughly linear in the number of features.

Our expected value oracle exploits the fact that our input graph is sampled from the CLV random graph model. Given this, we can explicitly calculate the expected value of $N_e$ for every edge which requires no training time and nearly constant space. For training details for our link prediction model, see Section \ref{sec:prediction_oracle_details}. Note that in general, there is a wide and rich family of predictors which can be trained using sublinear space or in a stream such as regression \cite{Woodruff2014SketchingAA}, classification for example using SVMs \cite{Andoni2020StreamingCO, Rai2009StreamedLO} and even deep learning models\cite{Gomes2019MachineLF}. 


==> Learning Augmented Triangles ICLR 22/adjacency_main.tex <==

\section{Triangle Counting in the Adjacency List Model}
\label{sec:adjacency list}
We describe an algorithm with a heavy edge oracle, and one with a value oracle.
\vspace{-3mm}
\paragraph{Heavy Edge Oracle.} We present an overview of our one-pass algorithm, Algorithm~\ref{alg:adj_tri_perfect},  with a space complexity of $\tilde{O}(\min(\epsilon^{-2}m^{2/3}/T^{1/3}, \epsilon^{-1} m^{1/2}))$, given in Theorem~\ref{theorem_adjacency}.
We defer the pseudocode and  proof of the theorem  to Appendix~\ref{sec:adj_missing}.
The adaptations and proofs for
%~\ref{thm:adj_noisy},
Theorems~\ref{thm:imperfect_adj},~\ref{thm:value_oracle:1} and~\ref{thm:value_oracle:2} for the various noisy oracles  appear in Appendix~\ref{sec:adj_noisy_oracles} and Appendix~\ref{sec:adj_value_oracle}.


\iffalse
Our algorithm roughly keeps track of a random sample of edges.
For each edge $(x, y)$ in the sample,
we keep a counter $C_{xy}$ for the number of nodes $z$ for which $\{x, y, z\}$ forms a triangle and $x <_s z <_s y$. We increment $C_{xy}$ for each $z$ in the stream connected to both $x$ and $y$, after we see the edge $xy$ but before we see the edge $yx$. When $yx$ arrives, our counter for $xy$ equals $R_{xy}$. By summing these counters over all sampled edges, we obtain an estimate that equals $T$ in expectation, up to a scaling factor, since $\sum_{(x, y) \in E} R_{xy} = T$. If all $R_{xy}$ are small, our estimate will have low variance. Otherwise, we would like to sample all edges $xy$ for which $R_{xy}$ is large, in order to reduce the variance and optimize our overall space complexity. We will not actually store these edges: instead, we approximate each $R_{xy}$ for these edges, and just keep a running total of these approximations.
\fi

Our algorithm works differently depending on the value of $T$. We first consider the case that $T \ge (m/\epsilon)^{1/2}$. 
Assume that for each sampled edge $xy$ in the stream, we can exactly know the number of triangles $R_{xy}$ this edge contributes to $T$. Then the rate at which we would need to sample each edge would be proportional to $p_{naive}\approx\eps^{-2}\Delta_{E}/T$, where $\Delta_E$ is the maximum number of triangles incident to any edge. Hence, our first idea is to separately consider light and non-light edges using the heavy edge oracle. This allows us to sample edges that are deemed light by the oracle at a lower rate, $p_1$, and compute their contribution by keeping track of $R_{xy}$ for each such sampled edge. Intuitively, light edges offer us more flexibility and thus we can sample them with a lower probability while ensuring the estimator’s error does not drastically increase.
In order to estimate the contribution due to  non-light edges, we again partition them into two types: medium and heavy, according to some threshold $\rho$. We then use an observation from ~\cite{MVV16}, that since for heavy edges $R_{xy}>\rho$, it is sufficient to sample from the entire stream  at rate $p_3\approx \eps^{-2}/\rho$, in order to both detect if some edge $xy$ is heavy  and if so to estimate $R_{xy}$.  


Therefore, it remains to estimate the contribution to $T$ due to medium edges (these are the edges that are deemed non-light by the oracle, and also non-heavy according to the sub-sampling above). Since the number of triangles incident to medium edges is higher than that of light ones, we have to sample them at some higher rate $p_2>p_1$. However, since their number is bounded, this is still space efficient. 
We get the desired bounds by correctly setting the thresholds between light, medium and heavy edges. 




When $T < (m/\epsilon)^{1/2}$ our algorithm becomes much simpler. 
We only consider two types of edges, light and heavy, according to some threshold $T/\rho$. To estimate the contribution due to heavy edges we simply store them and keep track of their $R_{xy}$ values. To estimate the contribution due to light edges we sub-sample them with rate $\eps^{-2}\cdot \Delta_{E}/T=\eps^{-2}/\rho$. 
The total space we use is $ \tilde{O} (\epsilon^{-1} \sqrt{m})$, which is optimal in this case. See Algorithm~\ref{alg:adj_tri_perfect} for more details of the implementation. 


\iffalse
We first consider the case when $T \ge (m/\epsilon)^{1/2}$. Let $\rho = (mT)^{1/3}$. We define the edge $xy$ to be \textit{heavy} if $R_{xy} \ge \rho$, \textit{light} if $R_{xy} \le \frac{T}{\rho}$, and \textit{medium} if $\frac{T}{\rho} < R_{xy} < \rho$. We train the oracle to predict, upon seeing $xy$, whether $R_{xy}$ is light or not. We define $H, M$, and $L$ as the set of heavy, medium, and light edges, respectively. Define $T_L = \sum_{xy \in L} R_{xy}$. We define $T_H$ and $T_M$ similarly. Since $\sum_{xy \in E} R_{xy} = T = T_L+T_M+T_H$, it suffices to estimate each of these three terms.

For the light edges, as shown in Lemma~\ref{lem:adjlist_light}, if we sample edges with rate $p_1\approx \epsilon^{-2} / \rho$, with high probability we obtain an estimate of $T_L$ within error $\pm \epsilon T$. For the heavy edges, we recall an observation in~\cite{MVV16}: for an edge $xy$ where $R_{xy}$ is large, even if we do not sample $xy$ directly, 
\textcolor{black}{if we sample from the stream (at rate $p_3\approx \epsilon^{-2} / \rho$)}, 
we are likely to sample some edges in the set $ |xz: \{x, y, z\} \in \Delta \textnormal{ and } x <_s z <_s y|$. We refer to the sampled set of these edges as $S_{aux}$.

Further, we will show that not only can we use $S_{aux}$ to recognize whether $R_{xy}$ is large, but also to estimate $R_{xy}$ (Lemma~\ref{lem:adjlist_heavy}). 
What remains to handle is the medium edges.
%We sample them with a larger sampling rate. 
Since medium edges have higher values of $R_{xy}$ than light edges, we sample with a larger rate, $p_2$, to reduce variance. However, we show there cannot be too many medium edges, so we do not pay too much extra storage space. The overall space we use is $\tilde{O} (\epsilon^{-2} m^{2/3} / T^{1/3})$. 

When $T < (m/\epsilon)^{1/2}$ our algorithm becomes much simpler. Let $\rho = \sqrt{m} / \epsilon$. We define the edge $xy$ to be \textit{heavy} if $R_{xy} \ge T / \rho$, and \textit{light} otherwise (so in this case all the medium edges become heavy edges). We directly store all the heavy edges and sub-sample with rate $\epsilon^{-2} / \rho$ to estimate $T_L$. The total space we use is $\tilde{O} (\epsilon^{-1} \sqrt{m})$, which is optimal in this case. See Algorithm~\ref{alg:adj_tri_perfect} for more details of the implementation. 

\todo{expand as in rebuttal}\todo{T: I added a new par in blue with some more intuition. perhaps the other pars are now redundant?}
\fi
\vspace{-3mm}
\paragraph{Value-Based Oracle.} We also consider the setting where the predictor returns an estimate
$p(e)$ of $R_e$, and we assume $R_e \leq p(e) \leq \alpha \cdot R_e$, where $\alpha \geq 1$ is an approximation factor. We relax this assumption to also handle additive error as well as noise, but for intuition we focus on this case. The value-based oracle setting requires the use of novel techniques, such as the use of exponential random variables (ERVs).
%Empirically, we found this  oracle to be justified on a number of data sets.   
%PIOTR:  we need  a pointer to  experiments. 
Given  this oracle, for an edge $e$, we compute $p(e)/u_e$, were $u_e$
is a standard ERV. We then store the $O(\alpha \log(1/\epsilon))$ edges $e$ for which $p(e)/u_e$ is largest.  Since we are in the adjacency list model, once we start tracking edge $e = xy$, we can also compute the true value $R_e$ of triangles that the edge $e$ participates in  (since for each future vertex $z$ we see, we can check if $x$ and $y$ are both neighbors of $z$). Note that we track this quantity only for the $O(\alpha \log(1/\epsilon))$ edges that we store. Using the max-stability property of ERVs, $\max_e R_e/u_e$ is equal in distribution to $T/u$, where $u$ is another ERV. Importantly, using the density function of an ERV, one can show that the edge $e$ for which $R_e/u_e$ is largest is, with probability $1 - O(\epsilon^3)$, in our list of the $O(\alpha \log(1/\epsilon))$ largest $p(e)/u_e$ values that we store. Repeating this scheme $r = O(1/\epsilon^2)$ times, we obtain independent estimates $T/u^1, \ldots, T/u^r$, where $u^1, \ldots, u^r$ are independent ERVs. Taking the median of these then gives a $(1 \pm \epsilon)$-approximation to the total number $T$ of triangles. We note that ERVs are often used in data stream applications (see, e.g., \cite{Andoni17}), though to the best of our knowledge they have not previously been used in the context of triangle estimation. We also give an alternative algorithm, based on subsampling at $O(\log n)$ scales, which has worse logarithmic factors in theory but performs well empirically. 

\iffalse
\begin{algorithm}[!ht]
   \caption{Counting Triangles in the Adjacency List Model}
   \label{alg:adj_tri_perfect}
\begin{algorithmic}[1]
   \STATE {\bfseries Input:} Adjacency list edge stream and an oracle $O_{\theta}$ that outputs \textsc{heavy} if $R_{xy} \ge \theta$ and \textsc{light} otherwise.
   \STATE {\bfseries Output:} An estimate of the triangle count $T$.
   \STATE Initialize $A_l \leftarrow 0$, $A_m \leftarrow 0$, $A_h \leftarrow 0$, $S_l \leftarrow \emptyset$, $S_m \leftarrow \emptyset$, $S_{aux} \leftarrow \emptyset$. Set $\rho \leftarrow (mT)^{1/3}$, $\theta \leftarrow T / \rho$, $p_1 \leftarrow \alpha \epsilon^{-2} / \rho$, $p_2 \leftarrow  \min(\beta\epsilon^{-2} \rho / T, 1)$, $p_3 \leftarrow \gamma \epsilon^{-2} \log n / \rho$ when $T \ge (m / \epsilon)^{1/2}$ or $\rho \leftarrow m^{1/2} / \epsilon$, $p_1 \leftarrow 0$, $p_2 \leftarrow 1$, $p_3 \leftarrow \gamma\epsilon^{-2} / \rho$ otherwise. Here $\alpha$, $\beta$, and $\gamma$ are large enough constants.
   %\STATE On :
    \WHILE{seeing edges adjacent to $v$ in the stream} \STATE For all $ab \in S_L \cup S_M$: If $a, b \in N(v)$ then $C_{ab} \leftarrow C_{ab} + 1$\; .
    \STATE For all $av \in S_{aux} $: $O_{av} \leftarrow 1$ (means we have seen $av$ twice)\; .
    \FOR{each incident edge $vu$}
    \STATE With probability $p_3$, $S_{aux} \leftarrow \{vu\} \cup S_{aux}$ and $O_{vu} \leftarrow 0$ \;.
    \IF{$O_{\theta}$ outputs \textsc{light}}
    \IF{$uv \in S_L$} 
        \STATE $A_l \leftarrow A_l + C_{uv}$ \;.
    \ELSE 
    \STATE With probability $p_1$, $S_L \leftarrow \{vu\} \cup S_L$ \;.
    \ENDIF
    \ELSE 
    \STATE $\# := |\{z: uz \in S_{aux}, O_{uz}=1, z \in N(v)\}|$ \;. % Let 
    \IF{$\# \ge p_3 \rho$} 
        \STATE $A_h \leftarrow A_h + \#$ \; .
    \ELSIF{$uv \in S_M$} 
        \STATE $A_m \leftarrow A_m + C_{uv}$ \; .
    \ELSE
     \item With probability $p_2$, $S_M \leftarrow \{vu\} \cup S_M$ \;.
     \ENDIF
    \ENDIF
    \ENDFOR
    \ENDWHILE
    \STATE {\bfseries return:} $A_l / p_1 + A_m / p_2 + A_h / p_3$ \; .
\end{algorithmic}
\end{algorithm}
\fi


\iffalse
\subsection{Algorithm with a Value Prediction Oracle}
\label{sec:adj_mul}
In the adjacency list model, when we see an edge $xy$, we know all the neighbors of the node $x$ or $y$, which can help the oracle give a more accurate prediction. Motivated by our empirical results in Section~\ref{sec: experiments}, it is reasonable in some settings to assume we have access to an oracle that can predict a good approximation to $R_{xy}$ when $xy$ is not light. We consider the following oracle model.

\begin{definition}
\label{def:value_oracle}
A heavy edge $(\alpha,\beta)$ oracle is an oracle that, for a given edge $xy$, indicate if (i) $R_{xy} \le T / \beta$, or (ii) $R_{xy} > T / \beta$, and output a value  $\hat{R}_{xy}$ for which $R_{xy} \le \hat{R}_{xy} \le \alpha R_{xy}$.\footnote{This form is equivalent to an oracle that can output $\tilde{R}_{xy}$ for which $\sqrt{\alpha} R_{xy} \ge \tilde{R}_{xy} \ge \frac{1}{\sqrt{\alpha}}R_{xy}$}
%$\alpha$-approximation of $R_{xy}$ .
\end{definition}
\todo{the second part of the oracle is only in case (i)?}

Given the above oracle, we have the following theorem. 
%The main idea is for the edge $xy$, if we know $R_{xy}$ is in different value level, we can use different sub-sampling rate.

\begin{theorem}
\label{thm:value_oracle}
Given an $(\alpha, \beta)$ oracle (as in Definition~\ref{def:value_oracle}), there exists a one-pass algorithm with space complexity $\tilde{O}(\epsilon^{-2} (m / \beta + \alpha))$ in the adjacency list model that returns a $(1 \pm \epsilon)$-approximation to $T$ with probability at least $7 / 10$. 
\end{theorem}

\textbf{Update}: we have a new version of the value prediction oracle(with two slightly definitions), which is put in Appendix~B now.
\todo{remove update once everything is in place}
\fi

% \paragraph{Results for Noisy Oracles.}\todo{Possibly remove this paragraph?}
% The adaptations and proofs for
% %~\ref{thm:adj_noisy},
% Theorems~\ref{thm:imperfect_adj},~\ref{thm:value_oracle:1} and~\ref{thm:value_oracle:2} for the various noisy oracles  appear in Appendix~\ref{sec:adj_noisy_oracles} and Appendix~\ref{sec:adj_value_oracle}.



==> Learning Augmented Triangles ICLR 22/arbitrary_lower_bound.tex <==
\subsection{Lower Bound}\label{sec:arbitrary_lower_bound}

In this section, we  prove a lower bound for algorithms in the arbitrary order model that have access to a perfect heavy edge oracle. Here heavy means $N_{uv} \ge T / c$ for a pre-determined threshold $c$, and we assume $c = o(m)$ and $T / c > 1$, as otherwise the threshold will be too small or too close to the average to give an accurate prediction. The following theorem shows an $\Omega(\min(m / \sqrt{T}, m^{3/2} / T))$ lower bound even with such an oracle.

\begin{theorem}
\label{thm:lower_bound_arbitrary}
Suppose that the threshold of the oracle $c = O(m^q)$, where $0 \le q < 1$. Then for any $T$ and $m$, $T \le m$, there exists $m^\prime = \Theta(m)$ and $T^\prime = \Theta(T)$ such that any one-pass arbitrary order streaming algorithm that distinguishes between $m^\prime$ edge graphs with $0$ and $T^\prime$ triangles with probability at least $2/3$ requires $\Omega(m / \sqrt{T})$ space. For any $T$ and $m$, $T = \Omega(m^{1 + \delta})$ where $\max(0, q - \frac{1}{2}) \le \delta < \frac{1}{2}$, there exists $m^\prime = \Theta(m)$ and $T^\prime = \Theta(T)$ such that any one-pass arbitrary order streaming algorithm that distinguishes between $m^\prime$ edge graphs with $0$ and $T^\prime$ triangles with probability at least $2/3$ requires $\Omega(m^{3/2} / T)$ space.
\end{theorem}

When $T \le m$, we consider the hubs graph mentioned in~\cite{KP17}.

\begin{definition}[Hubs Graph, \cite{KP17}]
The hubs graph $H_{r,d}$ consists of a single vertex $v$ with $2rd$ incident edges, and $d$ edges connecting disjoint pairs of $v$’s neighbors to form triangles.
\end{definition}

It is easy to see that in $H_{r, d}$, each edge has at most one triangle. Hence, there will not be any heavy edges of this kind in the graph. In~\cite{KP17}, the authors show an $\Omega(r\sqrt{d})$ lower bound for the hubs graph.

\begin{lemma}[\cite{KP17}]
Given $r$ and $d$, there exist two distributions $\mathcal{G}_1, \mathcal{G}_2$ on subgraphs $G_1$ and $G_2$ of $H_{r, d}$, such that any algorithm which distinguishes them with probability at least $2/3$ requires $\Omega(r\sqrt{d})$ space, where $G_i$ has $\Theta(rd)$ edges and $T(G_1) = d, T(G_2) = 0$.
\end{lemma}

Now, given $T$ and $m$, where $T \le m$, we let $r = \Theta(m/T)$ and $d = T$. We can see $H_{r, d}$ has $\Theta(m)$ edges and $T$ triangles, and we need $\Omega(r\sqrt{d}) = \Omega(m / \sqrt{T})$ space. 

When $T > m$, we consider the following $\Omega(m^{3/2} /  T)$ lower bound in~\cite{BC17}. % hard instances

Let $H$ be a complete bipartite graph with $b$ vertices on each side (we denote the two sides of vertices by $A$ and $B$). We add an additional $N$ vertex blocks $V_1, V_2, ... V_N$  with each $|V_i| = d$. Alice has an $N$-dimensional binary vector $x$. Bob has an $N$-dimensional binary vector $y$. Both $x$ and $y$ have exactly $N/3$ coordinates that are equal to $1$. Then, we define the edge sets 
\[
E_{\mathrm{Alice}} = \bigcup_{i:x_i = 1} \{\{u, v\}, u \in A, v \in V_i\}
\]
and
\[
E_{\mathrm{Bob}} = \bigcup_{i:y_i = 1} \{\{u, v\}, u \in B, v \in V_i\} \; .
\]
Let the final resulting graph be denoted by $G = (V, E)$ where $V = V_H \cup V_1 \cup ... \cup V_N$ and $E = E_H \cup E_{\mathrm{Alice}} \cup E_{\mathrm{Bob}}$.

In~\cite{BC17}, the authors show by a reduction to the $\textsc{DISJ}_N^{N/3}$ problem in communication complexity, that we need $\Omega(N)$ space to distinguish the case when $G$ has $0$ triangles from the case when $G$ has at least $b^2d$ triangles.

Given $m$ and $T $, $ T = \Theta(m^{1 + \delta})$ where $1 \le \delta < 1/2$, as shown in~\cite{BC17}, we can set $b = N^{s}$ and $d = N^{s - 1}$ where $s = 1/(1 - 2\delta)$. This will make $m = \Theta(N^{2s})$ and $T = \Theta(N^{3s - 1})$, which will make the $\Omega(m^{3/2} / T)$ lower bound hold. Note that at this time each edge will have an $O(\frac{1}{m})$-fraction of triangles or  an $O(\frac{1}{m^{1-\frac{1}{2s}}})$-fraction of triangles. Assume the threshold of the oracle $c = O(m^q)$. When $\delta \ge \max(0, q - \frac{1}{2})$, there will be no heavy edges in the graph.



Theorem~\ref{thm:lower_bound_arbitrary} follows from 
the above discussion.

==> Learning Augmented Triangles ICLR 22/arbitrary_main.tex <==
\section{Triangle Counting in the Arbitrary Order Model} \label{sec:arbitrary_main}

In this section we discuss Algorithm~\ref{alg:arb_tri_perfect} for estimating the number of triangles in an arbitrary order stream of edges. The pseudo-code of the algorithm as well as omitted proofs for the different  oracles are given in Supplementary Section \ref{sec:arbitrary_missing}. Here we give the intuition behind the algorithm. Our approach relies on sampling the edges of the stream as they arrive
and checking if every new edge forms a triangle with the previously sampled edges. 
However, as previously discussed, this approach alone fails if some edges have a large number of triangles incident to them as ``overlooking'' such edges might lead to an underestimation of the number of triangles. Therefore, we utilize a 
heavy edge oracle, and refer to edges that are not heavy as \emph{light}. Whenever a new edge arrives, we first query the oracle to determine if the edge is heavy. If the edge is heavy  we keep it, and otherwise we sample it with some probability. As in the adjacency list  arrival model case, this strategy allows us to reduce the variance of our estimator. By balancing the sampling rate and our threshold for heaviness, we ensure that the space requirement is not too high, 
while simultaneously guaranteeing that our estimate is accurate.


% Consider for example a graph $G$ in which there is one edge $e = (u, v)$ such that $u, v$ are connected to all other $n-2$ vertices in the graph, and there are no other edges, so $m=\Theta(n)$ and $T=\Theta(n)$. Unless we store the edge $e$, we cannot correctly approximate the number of triangles in $G$, as we cannot distinguish between $G$ and an almost identical graph that is missing the edge $e$ and has no triangles.\footnote{Indeed one could say that the edge $e$ could be identified by the large degree of its endpoints, but it is easy to generate an example with many high degree edges where only one contributes to the triangle count of the graph.} In general, ``overlooking'' edges with many incident triangles might lead to an underestimation of the number of triangles. Therefore, we utilize a 
% heavy edge oracle as before, and refer to edges that are not heavy as \emph{light}.
%  Whenever a new edge arrives, we first query the oracle to determine if the edge is heavy. If the edge is heavy  we keep it, and otherwise we sample it with probability $p$.
% As in the adjacency list  arrival model case, this strategy allows us to reduce the variance of our estimator.
% As each  light edge is sampled with probability $p$, and the set $\mH$ of all heavy edges is stored, this leads to an $O(mp+|\mH|)$ expected space algorithm.
% By balancing $p$ and our threshold for heaviness, we ensure that the space requirement is not too high, 
% while simultaneously guaranteeing that our estimate is accurate.
% \todo{This paragraph can probably be significantly reduced, and moved after the next paragraph}

% \algrenewcommand\algorithmicindent{0.1em}%




%   \begin{figure}[!ht]
    
%     \begin{subfigure}{2cm}
%       \centering
%       \begin{algorithmic}
%         \WHILE{$N \neq 0$}
%           \IF{$N$ is even}
%             \STATE $X \Leftarrow X \times X$
%             \STATE $N \Leftarrow N / 2$
%           \ENDIF
%         \ENDWHILE
%       \end{algorithmic}
%       \caption{Test Algorithm No.1}\label{alg:alg-1}
%     \end{subfigure}
% 		\hfill
%     \begin{subfigure}{2cm}
    
%       \begin{algorithmic}
%         \WHILE{$N \neq 0$}
%           \IF{$N$ is even}
%             \STATE $X \Leftarrow X \times X$
%             \STATE $N \Leftarrow N / 2$
%           \ENDIF
%         \ENDWHILE
%       \end{algorithmic}
%       \caption{Test Algorithm No.2}\label{alg:alg-2}
%     \end{subfigure}
%     \caption{Two algorithms side by side}\label{fig:twoalg}
%   \end{figure}

\iffalse
\algsetup{linenodelimiter=.} 
\renewcommand{\algorithmiccomment}[1]{\;\;// #1}
\renewcommand{\algorithmicindent}{.7em}%

\begin{minipage}[t]{0.49\textwidth}
    \begin{algorithm}[H]
  \caption{Counting Triangles in the Adjacency List Model}
  \label{alg:adj_tri_perfect}
\begin{algorithmic}[1]
   \STATE {\bfseries Input:} Adjacency list edge stream and an oracle $O_{\theta}$ that outputs \textsc{heavy} if $R_{xy} \ge \theta$ and \textsc{light} otherwise.
   \STATE {\bfseries Output:} An estimate of the triangle count $T$.
   \STATE Initialize $A_l,A_m,A_h = 0$, $S_l,S_m,S_{aux}=\emptyset$
   \STATE \vspace{-0.3cm} If $T \ge (m / \epsilon)^{1/2}$ then set
   $\rho = (mT)^{1/3}$, $\theta = T / \rho$, $p_1 = \alpha \epsilon^{-2} / \rho$, $p_2 =  \min(\beta\epsilon^{-2} \rho / T, 1)$, $p_3 = \gamma \epsilon^{-2} \log n / \rho$.
%   when $T \ge (m / \epsilon)^{1/2}$ 
Otherwise, set  $\rho = m^{1/2} / \epsilon$, $p_1 = 0$, $p_2 = 1$, $p_3 = \gamma\epsilon^{-2} / \rho$. Here $\alpha$, $\beta$, and $\gamma$ are large enough constants.
   %\STATE On :
    \WHILE{seeing edges adjacent to $v$} 
    \FOR{all $ab \in S_L \cup S_M$} 
    \STATE \textbf{if} $a, b \in N(v)$ \textbf{then} $C_{ab} = C_{ab} + 1$.
    \ENDFOR
    \FOR{all $av \in S_{aux} $} 
    \STATE $O_{av} = 1$  \COMMENT{seen $av$ twice}.
    \ENDFOR
    \FOR{each incident edge $vu$}
    \STATE W.p. $p_3$: $S_{aux} = \{vu\} \cup S_{aux}$, $O_{vu} = 0$
    \IF{$O_{\theta}$ outputs \textsc{light}}
    \STATE \textbf{if} $uv \in S_L$ \textbf{then} $A_l = A_l + C_{uv}$.
    % \IF{$uv \in S_L$} 
    % \STATE $A_l = A_l + C_{uv}$ .
    % \ELSE
    \STATE \textbf{else} w.p. $p_1$, $S_L = \{vu\} \cup S_L$
    % \ENDIF
    \ELSE 
    \STATE $\# := |\{z: uz \in S_{aux}, O_{uz}=1, z \in N(v)\}|$ . % Let 
    \STATE \textbf{if} $\# \ge p_3 \rho$ \textbf{then}
    $A_h = A_h + \#$.
    \STATE \textbf{else if} $uv \in S_M$ \textbf{then}
      $A_m = A_m + C_{uv}$.
    \STATE \vspace{-.4cm}\textbf{else}  w.p. $p_2$, $S_M = \{vu\} \cup S_M$.
    % \IF{$\# \ge p_3 \rho$} 
    %     \STATE $A_h = A_h + \#$ .
    % \ELSIF{$uv \in S_M$} 
    %     \STATE $A_m = A_m + C_{uv}$ .
    % \ELSE
    %  \item With probability $p_2$, $S_M = \{vu\} \cup S_M$ .
    %  \ENDIF
    \ENDIF
    \ENDFOR
    \ENDWHILE
    \STATE {\bfseries return:} $A_l / p_1 + A_m / p_2 + A_h / p_3$.
\end{algorithmic}
\end{algorithm}
\end{minipage}
\hfill
\begin{minipage}[t]{0.49\textwidth}
\begin{algorithm}[H]
    \centering
  \caption{Counting Triangles in the Arbitrary Order Model}
  \label{alg:arb_tri_perfect}
\begin{algorithmic}[1]
   \STATE {\bfseries Input:} Arbitrary order edge stream and an oracle $\mO$ that outputs \textsc{heavy} if $N_{xy} > \theta$ and \textsc{light} otherwise.
   \STATE {\bfseries Output:} An estimate of the triangle count $T$.
   \STATE Initialize $\theta=\max\big\{\frac{\eps T}{\sqrt{m}}, 1\big\}$, $p=C\max\big\{\frac{1}{\eps\sqrt{T}},\frac{\theta}{\eps^2\cdot T}\big\}$ for a constant $C$.
   \STATE Initialize $\ell_1, \ell_2, \ell_3 = 0$, and $\mS, \mH = \emptyset$.
   \FOR{every arriving edge $e$ in the stream}
        \IF{the oracle $\mO$ outputs \textsc{heavy}}
            \STATE Add $e$ to $\mH$
        \ELSE
            \STATE Add $e$ to $\mS$ with probability $p$.
        \ENDIF
        \FOR{each $w \in w_{\mS, \mS}$}
            \IF{$(e, w)$ is a triangle}
                \STATE Increment $\ell_{1}=\ell_{1}+1$.
            \ENDIF
        \ENDFOR
        \FOR{each $w \in w_{\mS, \mH}$}
            \IF{$(e, w)$ is a triangle}
                \STATE Increment $\ell_{2}=\ell_{2}+1$.
            \ENDIF
        \ENDFOR
        \FOR{each $w \in w_{\mH, \mH}$}
            \IF{$(e, w)$ is a triangle}
                \STATE Increment $\ell_{3}=\ell_{3}+1$.
            \ENDIF
        \ENDFOR
   \ENDFOR
   \STATE \textbf{return:} $\ell = \ell_1/p^2+ \ell_2/p+\ell_3$.
\end{algorithmic}
\end{algorithm}
\end{minipage}
\fi



\iffalse
\begin{figure}[htb!] 
\fbox{
\begin{minipage}{0.45\linewidth}\label{AT}
Algorithm~\ref{alg:3}
\smallskip
\begin{compactenum}
   \item {\bfseries Input:} Adjacency list edge stream and an oracle $O_{\theta}$ that outputs \textsc{heavy} if $R_{xy} \ge \theta$ and \textsc{light} otherwise.
   \item {\bfseries Output:} An estimate of the triangle count $T$.
   \vspace{0.2cm}
   \item Initialize $A_l,A_m,A_h = 0$, $S_l,S_m,S_{aux}=\emptyset$
   \item \vspace{-0.3cm} If $T \ge (m / \epsilon)^{1/2}$ then set
   $\rho = (mT)^{1/3}$, $\theta = T / \rho$, $p_1 = \alpha \epsilon^{-2} / \rho$, $p_2 =  \min(\beta\epsilon^{-2} \rho / T, 1)$, $p_3 = \gamma \epsilon^{-2} \log n / \rho$.
%   when $T \ge (m / \epsilon)^{1/2}$ 
Otherwise, set  $\rho = m^{1/2} / \epsilon$, $p_1 = 0$, $p_2 = 1$, $p_3 = \gamma\epsilon^{-2} / \rho$. Here $\alpha$, $\beta$, and $\gamma$ are large enough constants.
   %\STATE On :
    \item \textbf{while} {seeing edges adjacent to $v$}: 
    \begin{compactenum}    
        \item \textbf{for all} {$ab \in S_L \cup S_M$}: 
        \begin{compactenum}    
            \item \textbf{if} $a, b \in N(v)$ \textbf{then} $C_{ab} = C_{ab} + 1$.
        \end{compactenum}
        \item \textbf{for all} $av \in S_{aux}$:
        \begin{compactenum}
            \item  $O_{av} = 1$  \;\;\;{seen $av$ twice}.
        \end{compactenum}    
    \item \textbf{for}{ each incident edge $vu$}:
        \begin{compactenum}
            \item W.p. $p_3$: $S_{aux} = \{vu\} \cup S_{aux}$, $O_{vu} = 0$
            \IF{$O_{\theta}$ outputs \textsc{light}}
            \item \textbf{if} $uv \in S_L$ \textbf{then} $A_l = A_l + C_{uv}$.
            % \IF{$uv \in S_L$} 
            % \item $A_l = A_l + C_{uv}$ .
            % \ELSE
            \item \textbf{else} w.p. $p_1$, $S_L = \{vu\} \cup S_L$
            % \ENDIF
            \ELSE 
            \item $\# := |\{z: uz \in S_{aux}, O_{uz}=1, z \in N(v)\}|$ . % Let 
            \item \textbf{if} $\# \ge p_3 \rho$ \textbf{then}
            $A_h = A_h + \#$.
            \item \textbf{else if} $uv \in S_M$ \textbf{then}
              $A_m = A_m + C_{uv}$.
            \item \vspace{-.4cm}\textbf{else}  w.p. $p_2$, $S_M = \{vu\} \cup S_M$.
    % \IF{$\# \ge p_3 \rho$} 
    %     \STATE $A_h = A_h + \#$ .
    % \ELSIF{$uv \in S_M$} 
    %     \STATE $A_m = A_m + C_{uv}$ .
    % \ELSE
    %  \item With probability $p_2$, $S_M = \{vu\} \cup S_M$ .
    %  \ENDIF
    \end{compactenum}
    \end{compactenum}
    \STATE {\bfseries return:} $A_l / p_1 + A_m / p_2 + A_h / p_3$.
\end{compactenum}
\end{minipage}
}
\fbox{
\begin{minipage}{0.45\linewidth}\label{AT}
Algorithm~\ref{alg:3}
\smallskip
\begin{compactenum}
	\item Set $\theta=\max\big\{\frac{\eps \oT}{\sqrt{m}}, 1\big\}$, $p=C\max\big\{\frac{1}{\eps\sqrt{\oT}},\frac{\theta}{\eps^2\cdot \oT}\big\}$. 
	\item Set $\ell_1, \ell_2, \ell_3 = 0$.
	\item Let $\mS, \mH$ be empty sets.
    \item For every arriving edge $e$ in the stream:
	\begin{compactenum}
	    \item If $\mO(e)=\heavy$, then add $e$ to $\mH$. 
	    \item Otherwise  ($\mO(e)=\light$):
	        \begin{compactenum}
	        \item Add  $e$ to $\mS$ with probability $p$. 
	    \end{compactenum}
	    \item For each $w \in w_{\mS, \mS}$, if $(e, w)$ is a triangle:
	        \begin{compactenum}
	        \item Increment $\ell_{1}=\ell_{1}+1$.
	        \end{compactenum}
	    \item For each $w \in w_{S, \mH}$, if $(e, w)$ is a triangle:
	        \begin{compactenum}
	        \item Increment $\ell_{2}=\ell_{2}+1$.
	        \end{compactenum}
	    \item For each $w \in w_{\mH, \mH}$, if $(e, w)$ is a triangle:
	        \begin{compactenum}
	        \item Increment $\ell_{3}=\ell_{3}+1$.
	        \end{compactenum}
	\end{compactenum}
	\item After the pass:
	\begin{compactenum}
	\item Return $\ell = \ell_1/p^2+ \ell_2/p+\ell_3$.
	\end{compactenum}
\end{compactenum}
\end{minipage}
}
\end{figure}
\fi


In more detail, our algorithm works as follows. 
First, we set a heaviness threshold $\rho$, so that if we predict an edge $e$ to be part of $\rho$ or more triangles, we label it as heavy. 
We also set a sampling parameter $p$. 
We let  $\mH$ be the set of edges predicted to be heavy and let $\mS$ be a random sample of edges predicted to be light. 
Then, we count three types of triangles. 
The first counter, $\ell_1$, counts the triangles $\Delta = (e_1, e_2,e)$, where  the first two edges seen in this triangle by the algorithm, represented by $e_1$ and $e_2$, are both in $\mS$. Note that we only count the triangle if $e_1$ and $e_2$,were both in $\mS$ at the time $e$ arrives in the stream.
Similarly, $\ell_2$ counts triangles whose first two edges are in $\mS$ and $\mH$ (in either order), and $\ell_3$ counts triangles whose first two edges are in $\mH$. 
Finally, we return the estimate $\ell = \ell_1/p^2 + \ell_2/p + \ell_3$. 
Note that if the first two edges in any triangle are light, they will both be in $\mS$ with probability $p^2$, and if exactly one of the first two edges is light, it will be in $\mS$ with probability $p$.
Therefore, we divide $\ell_1$ by $p^2$ and $\ell_2$ by $p$ so that $\ell$ is an unbiased estimator.



%To describe the intuition for why $\ell$ is a good estimate, first we assume $p = 1,$ i.e., we sample everything. Then, for any triangle $\Delta,$ each of the first two edges are either in $S$ or $\mH,$ so the wedge they form is in one of $w_{S, S}, w_{S, \mH},$ or $w_{\mH, \mH}$. Therefore, each triangle is counted by exactly one of $\ell_1, \ell_2,$ or $\ell_3$. To reduce the space usage, we sample edges with lower probability. Each wedge of two light edges is part of $w_{S, S}$ with probability $p^2$, since both light edges must be sampled as part of $S$. Likewise, each wedge of one light edge and one heavy edge is part of $w_{S, \mH}$ with probability $p$, since the single light edge must be sampled as part of $S$. As a result, to make sure our estimates are unbiased, we divide $\ell_1$ by $p^2$ and $\ell_2$ by $p$. We need to balance the parameter $p$: we want $p$ to be small so that the space to store $S$ is low, but not too small or else our estimate will have high variance. Moreover, it is well-established \todo{cite?} that sampling edges that are part of several triangles with some probability $p$ contributes more to the variance than sampling edges that are part of few triangles. This is why we choose some heaviness threshold $\theta$ and store all heavy edges. We balance $\theta$ to be large enough so that we don't store too many heavy edges, but small enough so that light edges do not contribute greatly to the variance of our estimator $\ell$.

\medskip

% \paragraph{Results for Noisy Oracles.} \todo{Possibly remove this paragraph?}
%  The proof of the variant of Theorem \ref{theorem_arbitrary}  for the  case that the oracle is a  $K$-noisy oracle (Theorem~\ref{thm:imperfect_arbitrary}), 
%  follows a similar approach to the above. 
% %  We remark that Theorem \ref{thm:imperfect_arbitrary} is a stronger statement than Theorem \ref{theorem_arbitrary}. 
%  Both proofs are deferred to Supplementary Section \ref{sec:arbitrary_missing}.


% The proofs of Theorem \ref{thm:imperfect_arbitrary} and Theorem \ref{thm:imperfect_arbitrary} 
% for the  arbitrary error oracle and $K$-noisy oracle, respectively,  
% follow a similar approach, to the above. We remark that Theorem \ref{thm:imperfect_arbitrary} is a stronger statement than Theorem \ref{theorem_arbitrary}. Both proofs are deferred to Supplementary Section \ref{sec:arbitrary_missing}.





==> Learning Augmented Triangles ICLR 22/iclr_style/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

% \def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
% \def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
% \def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
% \def\mS{{\bm{S}}}
% \def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
% \newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
% \newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> Learning Augmented Triangles ICLR 22/justifying_noisy.tex <==
\section{Implicit Predictor in Prior Works }\label{sec:justify_noisy}

We prove that the first pass of the two pass 
triangle counting Algorithm given in Section $3.1$ of \cite{MVV16}, satisfies the conditions of the $K$-noisy oracle in Definition~\ref{dfn:noisy-oracle}. Therefore, our work can be seen as a generalization of their approach when handling multiple related data sets, where instead of performing two passes on each data set and using the first of which to train the heavy edge oracle, we perform the training once according to the first related dataset, and we get a one pass algorithm for all remaining sets.

We first recall the first pass of~\cite[Section 3.1]{MVV16}:
\begin{enumerate}
    \item Sample each node $z$ of the graph with probability $p= C \eps^{-2} \log m / \rho$ for some large constant $C > 0$. Let $Z$ be the set of sampled nodes.
    \item Collect all edges incident on the set $Z$.
    \item For any edge $e=\{u,v\}$, let $\tilde{t}(e)= |\{z \in Z : u,v \in N(z)\}|$ and define the oracle as 
     \[ \text{oracle}(e) =
 \begin{cases} \textsc{light} &\mbox{if } \tilde{t}(e) < p \cdot \rho \\
\textsc{heavy} & \mbox{if } \tilde{t}(e) \ge p \cdot \rho.  \end{cases} 
\]
\end{enumerate}
\begin{lemma}
For any edge $e = (u,v)$, $\textup{oracle}(e) = \textsc{light}$ implies $N_e \le 2 \rho$ and $\textup{oracle}(e) = \textsc{heavy}$ implies $N_e > \rho / \sqrt{2}$ with failure probability at most $1/n^{10}$.
\end{lemma}
\begin{proof}
For any edge $e$, it follows that $\tilde{t}(e) \sim \text{Bin}(N_e, p)$. Therefore if $N_e > 2\rho$,
\[\Pr[\tilde{t}(e) < p \cdot \rho] \le  \exp(-\Omega(p \cdot  \rho)) \le 1/n^{10}\]
by picking $C$ large enough in the definition of $p$. The other case follows similarly.
\end{proof}

\begin{lemma}
The expected space used by the above oracle is $O(pm)$.
\end{lemma}
\begin{proof}
Each vertex is sampled in $Z$ with probability $p$ and we keep all of its incident edges. Therefore, the expected number of edges saved is $O(p \sum_v d_v) = O(pm)$.
\end{proof}

Note that the oracle satisfies the conditions of the $K$-noisy oracle in Definition~\ref{dfn:noisy-oracle}. For example, if $N_e \ge C' \rho$ for $C' \gg 1$,  Definition~\ref{dfn:noisy-oracle} only assumes that we incorrectly classify $e$ with probability $1/C'$, whereas the oracle presented above incorrectly classifies $e$ with probability $\exp(- C')/n^{10}$ which is much smaller than the required $1/C'$. 


==> Learning Augmented Triangles ICLR 22/learning.tex <==


\section{Learnability Results}
In this section, we give formal learning bounds for efficient predictor learning for edge heaviness. In particular, we wish to say that a good oracle or predictor for edge heaviness and related graph parameters can be learned efficiently using few samples if we observe graph instances drawn from a distribution. We can view the result of this section, which will be derived via the PAC learning framework, as one formalization of data driven algorithm design. Our results are quite general but we state simple examples throughout the exposition for clarity. Our setting is formally the following.

Suppose there is an underlying distribution $\mathcal{D}$ which generates graph instances $H_1, H_2, \cdots$ all on $n$ vertices. Note that this mirrors some of our experimental setting, in particular our graph datasets which are similar snapshots of a dynamic graph across time. 

Our goal is to efficiently learn a good predictor $f$ among some family of functions $\mathcal{F}$. The input of each $f$ is a graph instance $H$ and the output is a feature vector in $k$ dimensions. The feature vector represents the prediction of the oracle and can encapsulate a variety of different meanings. One example is when $k = |E|$ and $f$ outputs an estimate of edge heaviness for all edges. Another is when $k <<|E|$ and $f$ outputs the id's of the $k$ heaviest edges. We also think of each input instance $H$ as encoded in a vector in $\R^{p}$ for $p \ge \binom{n}2$ (for example, each instance is represented as an adjacency matrix). Note that we allow for $p > \binom{n}2$ if for example, each edge or vertex for $H \sim \mathcal{D}$ also has an endowed feature vector.

To select the `best' $f$, we need to precisely define the meaning of best. Note that in many settings, this involves a loss function which captures the quality of a solution. Indeed, suppose we have a loss function $L: f \times H \rightarrow \R$ which represents how well a predictor $f$ performs on some input $H$. An example of $L$ could be squared error from the output of $f$ to the true edge heaviness values of edges in $H$. Note that such a loss function clearly optimizes for predicting the heavy edges well.

Our goal is to learn the best function $f \in \mathcal{F}$ which minimizes the following objective:
\begin{equation}\label{eq:best_f}
    \E_{H \sim D}[L(f,H)].
\end{equation}
Let $f^*$ be such the optimal $f \in \mathcal{F}$, and  assume that for each instance $H$ and each $f \in F$, $f(H)$ can be computed in time $T(p,k)$. For example, suppose graphs drawn from $\mathcal{D}$ possess edge features in $\R^d$,  and that our family $\mathcal{F}$ is parameterized by a single vector $\theta \in \R^d$ and represents linear functions which outputs the dot product of each edge feature with $\theta$. Then it is clear that $T(p,k)$ is a (small) polynomial in the relevant parameters.

Our main result is the following.

\begin{theorem}\label{thm:main_learning}
There is an algorithm which after $\poly(T(p,k), 1/\epsilon)$ samples, returns a function $\hat{f}$ that satisfies
\[  \E_{H \sim D}[L(\hat{f},H)] \le  \E_{H \sim D}[L(f^*,H)] + \epsilon \]
with probability at least $9/10$. 
\end{theorem}
We remark that one can boost the probability of success to $1-\delta$ by taking additional $\log(1/\delta)$ multiplicative samples.

The above theorem is a PAC-style bound which shows that only  a small number of samples are needed in order to ensure a good probability of learning an approximately-optimal function $\hat{f}$. The algorithm to compute $\hat{f}$ is the following: we simply minimize the empirical loss after an appropriate number of samples are drawn, i.e., we perform empirical risk minimization. This result is proven by Theorem \ref{thm:uni-dim}. Before introducing it, we need to define the concept of pseudo-dimension for a function class which is the more familiar VC dimension, generalized to real functions.
\begin{definition}[Pseudo-Dimension, Definition $9$ \cite{feldman_gaussians}]
Let $\mathcal{X}$ be  a  ground  set  and $\mathcal{F}$ be a set of functions from $\mathcal{X}$ to the interval $[0,1]$. Fix a set $S= \{x_1,\cdots ,x_n\} \subset \mathcal{X}$, a set of real numbers $R=\{r_1, \cdots, r_n\}$ with $r_i \in [0, 1]$ and a function $f \in \mathcal{F}$. The set $S_f= \{x_i \in S  \mid f(x_i) \ge r_i\}$ is called the induced subset of $S$ formed by $f$ and $R$. The set $S$ with associated values $R$ is shattered by $\mathcal{F}$ if $|\{S_f \mid f \in \mathcal{F} \}|= 2^n$. 
The \emph{pseudo-dimension} of $\mathcal{F}$ is the cardinality of the largest shattered subset of $\mathcal{X}$ (or $\infty$).
\end{definition}
The following theorem relates the performance of empirical risk minimization and the number of samples needed, to the notion of pseudo-dimension. We specialize the theorem statement to our situation at hand. For notational simplicity, we define $\mathcal{A}$ be the class of functions in $f$ composed with $L$:
\[\mathcal{A} := \{L \circ f : f \in \mathcal{F} \}.  \]
Furthermore, by normalizing, we can assume that the range of $L$ is equal to $[0,1]$.
\begin{theorem}[\cite{anthony_bartlett_1999}]\label{thm:uni-dim}
 Let $\mathcal{D}$ be a distribution over graph instances and $\mathcal{A}$ be a class of functions $a: H \rightarrow[0, 1]$ with pseudo-dimension $d_{\mathcal{A}}$. Consider $t$ i.i.d.\ samples $H_{1}, H_{2}, \ldots, H_{t}$ from $\mathcal{D} .$ There is a universal constant $c_{0}$, such that for any $\epsilon>0$, if $t \geq c_{0} \cdot d_{\mathcal{A}}/\epsilon^2,$ then we have
$$
\left|\frac{1}{t} \sum_{i=1}^{t} a\left(H_{i}\right)-\mathbb{E}_{H \sim \mathcal{D}} \, a(H)\right| \leq \epsilon
$$
for all $a \in \mathcal{A}$ with probability at least $9/10 .$
\end{theorem}
The following corollary follows from the triangle inequality.
\begin{corollary}\label{cor:uni-dim-cor}
Consider a set of $t$ independent samples $H_1, \ldots, H_t$ from $\mathcal{D}$ and let $\hat{a}$ be a function in $\mathcal{A}$ which minimizes $\frac{1}t \sum_{i=1}^t a(H_i)$. If the number of samples $t$ is chosen as in Theorem \ref{thm:uni-dim}, then
\[\E_{H \sim D} [\hat{a}(H)] \le \E_{H \sim D}[a^*(H)] + 2 \epsilon \]
holds with probability at least $9/10$.
\end{corollary}
The main challenge  is to bound the pseudo-dimension of our given function class $\mathcal{A}$. To do so, we first relate the pseudo-dimension to the VC dimension of a related class of threshold functions. This relationship has been fruitful in obtaining learning bounds in a variety of works such as \cite{feldman_gaussians, barycenter}.
\begin{lemma}[Pseudo-dimension to VC dimension, Lemma $10$ in \cite{feldman_gaussians}]\label{lem:PD_to_VC}
For any $a \in \mathcal{A}$, let $B_a$ be the indicator function of the region on or below the graph of $a$, i.e., $B_a(x,y)  =  \text{sgn}(a(x)-y)$. The pseudo-dimension of $\mathcal{A}$ is equivalent to the VC-dimension of the subgraph class $B_{\mathcal{A}}=\{B_a \mid a \in \mathcal{A}\}$.
\end{lemma}
Finally, the following theorem relates the VC dimension of a given function class to its computational complexity, i.e., the complexity of computing a function in the class in terms of the number of operations needed.
\begin{lemma}[Theorem $8.14$ in \cite{anthony_bartlett_1999}]\label{lem:VC_bound}
Let $w: \R^{\alpha} \times \R^{\beta} \rightarrow \{ 0,1\}$, determining the class
\[ \mathcal{W} = \{x \rightarrow w(\theta, x) : \theta \in \R^{\alpha}\}. \]
Suppose that any $w$ can be computed by an algorithm that takes as input the pair $(\theta, x) \in \R^{\alpha} \times \R^{\beta}$ and returns $w(\theta, x)$ after no more than $r$ of the following operations:
\begin{itemize}
    \item arithmetic operations $+, -,\times,$ and $/$ on real numbers,
    \item jumps conditioned on $>, \ge ,<, \le ,=,$ and $=$ comparisons of real numbers, and
    \item output $0,1$,
\end{itemize}
then the VC dimension of $\mathcal{W}$ is $O(\alpha^2 r^2 + r^2 \alpha \log \alpha)$.
\end{lemma}
Combining the previous results allows us prove Theorem \ref{thm:main_learning}. At a high level, we are instantiating Lemma \ref{lem:VC_bound} with the complexity of \emph{computing} any function in the function class $\mathcal{A}$.
\begin{proof}[Proof of Theorem \ref{thm:main_learning}]
First by Theorem \ref{thm:uni-dim} and Corollary \ref{cor:uni-dim-cor}, it suffices to bound the pseudo-dimension of the class $\mathcal{A} = L \circ \mathcal{F}$. Then from Lemmas \ref{lem:PD_to_VC}, the pseudo-dimension of $\mathcal{A}$ is the VC dimension of threshold functions defined by $\mathcal{A}$. Finally from Lemma \ref{lem:VC_bound}, the VC dimension of the appropriate class of threshold functions is polynomial in the complexity of computing a member of the function class. In other words, Lemma \ref{lem:VC_bound} tells us that the VC dimension of $B_{\mathcal{A}}$ as defined in Lemma \ref{lem:PD_to_VC} is polynomial in the number of arithmetic operations needed to compute the threshold function associated to some $a \in \mathcal{A}$. By our definition, this quantity is polynomial in $T(p,k)$. Hence, the pseudo-dimension of $\mathcal{G}$ is also polynomial in $T(p,k)$ and the result follows.
\end{proof}
Note that we can consider initializing Theorem \ref{thm:main_learning} with specific predictions. If the family of oracles we are interested in is efficient to compute (which is the case of the predictors we employ in our experiments), then Theorem \ref{thm:main_learning} assures us that only  polynomially many samples are required (in terms of the computational complexity of our function class), to be able to learn a nearly optimal oracle. Furthermore, computing the empirical risk minimizer needed in Theorem \ref{thm:main_learning} is also efficient for a wide verity of function classes. For example in practice, we can simply use gradient descent or stochastic gradient descent for a range of predictor models, such as regression or even general neural networks.

We remark that our learnability result is in similar in spirit to one given in the recent learning-augmented paper \cite{learned_duals}. There, they derive sample complexity learning bounds for the different algorithmic problem of computing matchings in a graph (not in a stream). Since they specialize their analysis to a specific function class and loss function, their bounds are tighter compared to the possibly loose polynomial bounds we have stated. However, our analysis above is more general as it allows for a variety of predictors and loss functions to measure the quality of the predictions.


==> Learning Augmented Triangles ICLR 22/runtime_analysis.tex <==


\section{Runtime Analysis} \label{sec:runtime}

In this section, we verify the runtimes of our Algorithms \ref{alg:adj_tri_perfect}, \ref{alg:4}, \ref{alg:value_prediction:2}, \ref{alg:arb_tri_perfect}, and \ref{alg:3}.

\begin{proposition}
    Algorithm \ref{alg:adj_tri_perfect} runs in expected time at most $\tilde{O}\left(\min(\eps^{-2} m^{5/3}/T^{1/3}, \eps^{-1} m^{3/2})\right)$ in the setting of Theorem \ref{theorem_adjacency}, or $\tilde{O}\left(\min(\eps^{-2} m^{5/3}/T^{1/3}, K \cdot \eps^{-1} m^{3/2})\right)$ in the setting of Theorem \ref{thm:imperfect_adj}.
\end{proposition}

\begin{proof}
    For each edge $ab \in S_L \cup S_M$, we check whether we see both $va$ and $vb$ (lines 9-10) when looking at edges adjacent to $v$. So, this takes time $|S_L|+|S_M|$ per edge in the stream. We similarly check for each edge in $S_{aux}$ (lines 11-12), so this takes time $|S_{aux}|$. Finally, for each edge $vu$ (line 13), we note that lines 14-17 can trivially be implemented in $O(1)$ time, along with $1$ call to the oracle. The remainder of the oracle simply involves looking through the set $S_{aux}$ and $S_M$ to search or count for elements. Thus, the overall runtime is $O(|S_L|+|S_M|+|S_{aux}|)$ per stream element, so the runtime is $O\left(m \cdot (|S_L|+|S_M|+|S_{aux}|)\right)$.
    
    This is at most $O(m \cdot S)$, where $S$ is the space used by the algorithm. So, the runtime is $\tilde{O}\left(\min(\eps^{-2} m^{5/3}/T^{1/3}, \eps^{-1} m^{3/2}\right)$ in the setting of Theorem \ref{theorem_adjacency}, and is at most $\tilde{O}\left(\min(\eps^{-2} m^{5/3}/T^{1/3}, K \cdot \eps^{-1} m^{3/2})\right)$ in the setting of Theorem \ref{thm:imperfect_adj}.
\end{proof}

\begin{proposition}
    Algorithm \ref{alg:4} runs in time $\tilde{O}(\eps^{-2} (\alpha + m\beta / T) m)$.
\end{proposition}

\begin{proof}
    For each edge $ab \in S^i$ for each $0 \le i \le c \eps^{-2}$, we check whether we see both $ya$ and $yb$ in the stream when looking at edges adjacent to $y$. So, lines 7-8 take time $O(\sum |S^i|)$ for each edge we see in the stream. By storing each $S^i$ (and each $Q^i$) in a balanced binary search tree or a similar data structure, we can search for $xy \in S^i$ in time $O(\log n)$ in line $11$, and it is clear that lines 12-16 take time $O(\log n)$ (since insertion into the data structure for $Q^i, S^i$ can take time $O(\log n)$). Since we do this for each $i$ from $0$ to $c \eps^{-2}$ and for each incident edge $yx$ we see, in total we spend $O(\eps^{-2} \log n + \sum |S^i|)$ time up to line 16. The remainder of the lines take time $O(\eps^{-2} \cdot m \log n)$, since the slowest operation is potentially deleting an edge from each $S^i$ and a value from each $Q^i$ up to $m$ times (for each edge). 
    
    Overall, the runtime is $\tilde{O}(\eps^{-2} \cdot m + m \cdot \sum |S^i|) = \tilde{O}(m \cdot S)$, where $S$ is the total space used by the algorithm. Hence, the runtime is $\tilde{O}(\eps^{-2} (\alpha + m\beta / T) m)$.
\end{proof}

\begin{proposition}
    Algorithm \ref{alg:value_prediction:2} runs in time $\tilde{O}(K \eps^{-2} (\alpha + m\beta / T) m)$.
\end{proposition}

\begin{proof}
    For each edge $ab \in S_i^j$ for each $1 \le i \le O(\log n), 1 \le j \le O(\log \log n)$, we check whether we see both $ya$ and $yb$ in the stream when looking at edges adjacent to $y$. So, line 5 takes time $O(\sum |S_i^j|)$ for each edge we see in the stream. By storing each $S_i^j$ in a balanced binary search tree or a similar data structure, we can search for $xy \in S^i$ in time $O(\log n)$ in line $7$, and it is clear that lines 8-12 take time $O(\log n)$ (since insertion into the data structure for $Q_i^j$ can take time $O(\log n)$). Since we do this for each $i$ from $0$ to $c \eps^{-2}$ and for each incident edge $yx$ we see, in total we spend $\poly\log n \cdot O(\sum |S^i|)$ time up to line 12. Finally, lines 13-15 take time $\poly\log n$.
    
    Overall, the runtime is $\tilde{O}(m \cdot \sum |S^i|) = \tilde{O}(m \cdot S)$, where $S$ is the total space used by the algorithm. Hence, the runtime is $\tilde{O}(K \eps^{-2} (\alpha + m\beta / T) m)$.
\end{proof}

\begin{proposition}
    Algorithm \ref{alg:arb_tri_perfect} runs in time $\tilde{O}\left(\eps^{-1} \cdot m^2/\sqrt{T} + \eps^{-1} \cdot m^{3/2}\right).$
\end{proposition}

\begin{proof}
    For each edge $e$ in the stream, first we check the oracle, and we either add $e$ to $H$ or to $S_L$ with probability $p$ (lines 6-9), which take $O(1)$ time. The remaining lines (lines 10-18) involve operations that take $O(1)$ time for each $w$ which represents a pair $(e_1, e_2)$ of edges where $e_1, e_2 \in S_L \cup H$ and $(e, e_1, e_2)$ forms a triangle. So, the runtime is bounded by the amount of time it takes to find all $e_1, e_2 \in S_L \cup H$ such that $(e, e_1, e_2)$ forms a triangle. If the edge $e = (u, v)$, we just find all edges in $S_L \cup H$ adjacent to $u$, and all edges in $S_L \cup H$ adjacent to $v$. Then, we sort these edges based on their other endpoint and match the edges if they form triangles. So, the runtime is $\tilde{O}(|S_L|+|H|)$ per edge $e$ in the stream. Finally, line 19 takes O(1) time.
    
    Overall, the runtime is $\tilde{O}(m \cdot (|S_L|+|H|)) = \tilde{O}(m \cdot S)$ where $S$ is the total space of the algorithm. So, the runtime is $\tilde{O}\left(\eps^{-1} \cdot m^2/\sqrt{T} + \eps^{-1} \cdot m^{3/2}\right).$
\end{proof}

\begin{proposition}
    Algorithm \ref{alg:3} runs in time $\tilde{O}\left(\eps^{-2}/T^{1/3} \cdot (n^3+m^2)\right)$.
\end{proposition}

\begin{proof}
    We note that for each edge $uv$ in the stream (line 4), the code in the loop (lines 5-11) can be implemented using $1$ oracle call and $\tilde{O}(|E_L|)$ time. The only nontrivial step here is to find pairs $(w, z)$ such that $uw, wz, zv$ are all in $E_L$. However, by storing $E_L$ in a balanced binary search tree or similar data structure, one can enumerate through each edge $wz \in E_L$ and determine if $uw$ and $zv$ are in $E_L$ in $O(\log |E_L|)$ time. So, lines 4-11 take time $\tilde{O}(|E_L|)$ per stream element.
    
    Next, lines 12-16 can easily be implemented in time $O(n^2 \cdot |S|)$, lines 17-19 can be easily implemented in time $\tilde{O}(|D|)$ if the vertices in $W$ are stored properly, and lines 20-23 can be done in $\tilde{O}(|E_H| \cdot |E_L|)$ time. The last part is true since we check each $uv \in E_H$ and $e=(u',v') \in E_L$, and then check if $u, u', v', v$ form a $4$-cycle by determining if $u, u'$ and $v, v'$ are in $E_L \cup E_H$ (which takes time $O(\log |E_L|+\log |E_H|)$ time assuming $E_L, E_H$ are stored in search tree or similar data structure).
    
    Overall, we can bound the runtime as $\tilde{O}(m \cdot |E_L|+n^2 \cdot |S|+|D|+|E_H| \cdot |E_L|) = \tilde{O}(m \cdot |E_L|+n^2 \cdot |S|)$. As each edge is in $E_L$ with probability at most $p$ and each edge is in $S$ with probability at most $p$, the total runtime is $\tilde{O}\left((m^2 +n^3) \cdot p\right) = \tilde{O}\left(\eps^{-2}/T^{1/3} \cdot (n^3+m^2)\right)$.
\end{proof}


==> Learning Augmented Triangles ICLR 22/sup_adj_list.tex <==
\section{Omitted Proofs from Section~\ref{sec:adjacency list}}\label{sec:adj_missing}

In this section, we prove correctness and bound the space of Algorithm~\ref{alg:adj_tri_perfect}, thus proving Theorem~\ref{theorem_adjacency}. In the adjacency list model, recall that we have a total ordering on nodes $<_s$ based on the stream ordering, where $x <_s y$ if and only if the adjacency list of $x$ arrives before the adjacency list of $y$ in the stream. For each $xy \in E(G)$, we define $R_{xy} = |z: \{x, y, z\} \in \Delta \textnormal{ and } x <_s z <_s y|$. Note that if $y <_s x$, then $R_{xy} = 0$. It holds that
$ \sum_{xy \in E} R_{xy} = T $.

We first give a detailed overview of the algorithm. We first consider the case when $T \ge (m/\epsilon)^{1/2}$. Let $\rho = (mT)^{1/3}$. We define the edge $xy$ to be \textit{heavy} if $R_{xy} \ge \rho$, \textit{light} if $R_{xy} \le \frac{T}{\rho}$, and \textit{medium} if $\frac{T}{\rho} < R_{xy} < \rho$. We train the oracle to predict, upon seeing $xy$, whether $R_{xy}$ is light or not. We define $H, M$, and $L$ as the set of heavy, medium, and light edges, respectively. Define $T_L = \sum_{xy \in L} R_{xy}$. We define $T_H$ and $T_M$ similarly. Since $\sum_{xy \in E} R_{xy} = T = T_L+T_M+T_H$, it suffices to estimate each of these three terms.

For the light edges, as shown in Lemma~\ref{lem:adjlist_light}, if we sample edges with rate $p_1\approx \epsilon^{-2} / \rho$, with high probability we obtain an estimate of $T_L$ within error $\pm \epsilon T$. For the heavy edges, we recall an observation in~\cite{MVV16}: for an edge $xy$ where $R_{xy}$ is large, even if we do not sample $xy$ directly, 
\textcolor{black}{if we sample from the stream (at rate $p_3\approx \epsilon^{-2} / \rho$)}, 
we are likely to sample some edges in the set $ |xz: \{x, y, z\} \in \Delta \textnormal{ and } x <_s z <_s y|$. We refer to the sampled set of these edges as $S_{aux}$.

Further, we will show that not only can we use $S_{aux}$ to recognize whether $R_{xy}$ is large, but also to estimate $R_{xy}$ (Lemma~\ref{lem:adjlist_heavy}). 
What remains to handle is the medium edges.
%We sample them with a larger sampling rate. 
Since medium edges have higher values of $R_{xy}$ than light edges, we sample with a larger rate, $p_2$, to reduce variance. However, we show there cannot be too many medium edges, so we do not pay too much extra storage space. The overall space we use is $\tilde{O} (\epsilon^{-2} m^{2/3} / T^{1/3})$. 

When $T < (m/\epsilon)^{1/2}$ our algorithm becomes much simpler. Let $\rho = \sqrt{m} / \epsilon$. We define the edge $xy$ to be \textit{heavy} if $R_{xy} \ge T / \rho$, and \textit{light} otherwise (so in this case all the medium edges become heavy edges). We directly store all the heavy edges and sub-sample with rate $\epsilon^{-2} / \rho$ to estimate $T_L$. The total space we use is $\tilde{O} (\epsilon^{-1} \sqrt{m})$, which is optimal in this case. See Algorithm~\ref{alg:adj_tri_perfect} for more details of the implementation. 


\begin{algorithm}[ht]
  \caption{Counting Triangles in the Adjacency List Model}
  \label{alg:adj_tri_perfect}
\begin{algorithmic}[1]
   \STATE {\bfseries Input:} Adjacency list edge stream and an oracle $O$ that outputs \textsc{heavy} if $R_{xy} \ge T/\rho$ and \textsc{light} otherwise.
   \STATE {\bfseries Output:} An estimate of the triangle count $T$.
   \STATE Initialize $A_l,A_m,A_h = 0$, $S_L,S_M,S_{aux}=\emptyset$
   \IF{$T \ge (m / \epsilon)^{1/2}$} 
   \STATE Set
   $\rho = (mT)^{1/3}$, $p_1 = \alpha \epsilon^{-2} / \rho$, $p_2 =  \min(\beta\epsilon^{-2} \rho / T, 1)$, $p_3 = \gamma \epsilon^{-2} \log n / \rho$.
%   when $T \ge (m / \epsilon)^{1/2}$ 
    \ELSE
    \STATE Set  $\rho = m^{1/2} / \epsilon$, $p_1 = 0$, $p_2 = 1$, $p_3 = \gamma\epsilon^{-2} / \rho$. \COMMENT{$\alpha$, $\beta$, and $\gamma$ are large enough constants.}
    \ENDIF
   %\STATE On :
%   \STATE  Set $\theta = T / \rho$. 
    \WHILE{seeing edges adjacent to $v$} 
    
    \FORALL{$ab \in S_L \cup S_M$} 
    \STATE \textbf{if} $a, b \in N(v)$ \textbf{then} $C_{ab} = C_{ab} + 1$. \COMMENT{Update the counter for all the sampled light and medium edges}
    \ENDFOR
    
    \FORALL {$av \in S_{aux} $} 
    \STATE $B_{av} = 1$  \COMMENT{seen $av$ twice}.
    \ENDFOR
    \FOR{ each incident edge $vu$}
    \STATE W.p. $p_3$: $S_{aux} = \{vu\} \cup S_{aux}$, $B_{vu} = 0$
    \IF{$O(uv)$ outputs \textsc{light}}
    \STATE \textbf{if} $uv \in S_L$ \textbf{then} $A_l = A_l + C_{uv}$. \COMMENT{Finished counting $R_{uv}$}
    % \IF{$uv \in S_L$} 
    % \STATE $A_l = A_l + C_{uv}$ .
    % \ELSE
    \STATE \textbf{else} w.p. $p_1$, $S_L = \{vu\} \cup S_L$
    % \ENDIF
    \ELSE[$uv$ is either \textsc{medium} or \textsc{heavy}]
    \STATE $\# := |\{z: uz \in S_{aux}, B_{uz}=1, z \in N(v)\}|$ . 
        \IF[$uv$ is \textsc{heavy}]{$\# \ge p_3 \rho$} 
            \STATE $A_h = A_h + \#$ .
        \ELSIF{$uv \in S_M$} 
            \STATE $A_m = A_m + C_{uv}$. \COMMENT{Finished counting $R_{uv}$}
        \ELSE
         \item With probability $p_2$, $S_M = \{vu\} \cup S_M$ .
         \ENDIF
    \ENDIF
    \ENDFOR
    \ENDWHILE
    \STATE {\bfseries return:} $A_l / p_1 + A_m / p_2 + A_h / p_3$.
\end{algorithmic}
\end{algorithm}

\begin{remark}
In the adjacency list model, we assume the oracle can predict whether $R_{xy} \ge \frac{T}{c}$ or not, where $R_{xy}$ is dependent on the node order. This may sometimes be impractical. However, observe that $N_{xy} \ge R_{xy}$ and $\sum N_{xy} = 3T$. Hence, our proof still holds if we assume what the oracle can predict is whether $N_{xy} \ge \frac{T}{c}$, which could be a more practical assumption. 
\end{remark}


Recall the following notation from Section~\ref{sec:adjacency list}.
We define the edge $xy$ to be \textit{heavy} if $R_{xy} \ge \rho$, \textit{light} if $R_{xy} \le \frac{T}{\rho}$, and \textit{medium} if $\frac{T}{\rho} < R_{xy} < \rho$.  We define $H, M$, and $L$ as the set of heavy, medium, and light edges, respectively. Define $T_L = \sum_{xy \in L} R_{xy}$. We define $T_H$ and $T_M$ similarly. Also, recall that since $\sum_{xy \in E} R_{xy} = T = T_L+T_M+T_H$, it suffices to estimate of these three terms.



\begin{lemma}
\label{lem:adjlist_light}
Let $A$ be an edge set such that for each edge $xy \in A$, $R_{xy} \le \frac{T}{c}$, for some parameter $c$, and let $S$ be a subset of $A$ such that every element in $A$ is included in $S$ with probability $p=\frac{1}{\tau}$
for $\tau = \eps^2\cdot c/\alpha,$ so that 
$1/\tau= \alpha \epsilon^{-2} \frac{1}{c}$ independently, for a sufficient large constant $\alpha$. Then, with probability at least $9 / 10$, we have 
\[
\tau \sum_{xy \in S} R_{xy} = \sum_{xy \in A} R_{xy}  \pm \epsilon T % +
\]
\end{lemma}

\begin{proof}
We let $Y = \tau \sum_{i \in S} R_{i} = \tau \sum_{i \in A} f_{i} R_{i}$, where $f_{i} = 1$ when $i \in S$ and $f_{i} = 0$ otherwise. It follows that $\mathbb{E}[Y] = T_A$. Then, 
\begin{align*}
\mathbf{Var}[Y]  & =  \mathbb{E}[Y^2] - {\mathbb{E}[Y]}^{2}  \\
& = \tau^2 \left( \mathbb{E}[ 
\sum \limits_{i \in A} {f_i R_i^2}  + \sum \limits_{i \neq j} f_i f_j R_i R_j ] \right) - T_{L}^2
\\
  & \le \tau^2 \left( \mathbb{E}[
\sum \limits_{i \in A} {f_i R_{i}^2}]  + \sum \limits_{i, j} \frac{1}{\tau^2} R_i R_j \right)  - T_{L}^2
  \\
  & = \tau \sum \limits_{i \in A} R_i^2
  \; .
\end{align*}

To bound this, we notice that $R_i \le \frac{T}{c}$ and $\sum_i R_i = T_A \le T$, so%{}%\setlength\abovedisplayskip{0.5pt} %\setlength\belowdisplayskip{2pt}
\[
\tau \sum \limits_{i \in A} R_i^2 \le \tau \cdot \max_{i \in A} R_i \cdot \sum \limits_{i \in A} R_i \le \tau \cdot \frac{T}{c} \cdot T = \frac{\tau}{c} T^2 = \frac{1}{\alpha} \epsilon^2 T^2 \;.
\]
By Chebyshev's inequality, we have that 
\[
    \Pr [|Y - T_A| > \epsilon T] \le \frac{\frac{1}{\alpha}\epsilon^2 T^2}{\epsilon^2 T^2}\le \frac{1}{\alpha} \;. 
\]
\end{proof}


The following lemma shows that for the heavy edges, we can use the edges we have sampled to recognize and estimate them.
\begin{lemma}
\label{lem:adjlist_heavy}
Let $xy$ be an edge in $E$. Assume we sample the edges with rate $p_3 = \beta \epsilon^{-2} \log n/ \rho$ in the stream for a sufficiently large constant $\beta$, and consider the set 
\[
\# = |xz \textnormal{ has been sampled}: \{x, y, z\} \in \Delta \textnormal{ and } x <_s z <_s y| \; .
\]
Then we have the following: if $R_{xy} \ge \frac{\rho}{2}$, with probability at least $1 - \frac{1}{n^5}$, we have $ p_3^{-1}\cdot\#= (1 \pm \epsilon) R_{xy}$. If $R_{xy} < \frac{\rho}{2}$, with probability at least $1 - \frac{1}{n^5}$, we have $p_3^{-1}\cdot  \# < \rho$.
\end{lemma}

\begin{proof}
We first consider the case when $R_{xy} \ge \frac{\rho}{2}$.

For each edge $i \in |xz : \{x, y, z\} \in \Delta \textnormal{ and } x <_s z <_s y|$, let $X_i$ = 1 if $i$ has been sampled, or $X_i = 0$ otherwise. We can see the $X_i$ are i.i.d. Bernoulli random variables and $\mathbb{E}[X_i] = p_3$. By a Chernoff bound we have
\[
\mathbf{Pr}\left[|\sum_i X_i - p_3 R_{xy}| \ge \epsilon p_3 \cdot R_{xy}\right] \le 2\exp\left(-\epsilon^2 p_3\cdot  R_{xy}/3\right) \le \frac{1}{n^5} \; .
\]
Therefore, we have
\begin{align*}
\mathbf{Pr}\left[|p_3^{-1}\cdot \# - R_{xy}| \ge \epsilon R_{xy}\right] =& \mathbf{Pr}\left[ |p_3^{-1}\cdot \sum_i X_i - R_{xy}| \ge \epsilon R_{xy}\right] 
\le \frac{1}{n^5} \; .
\end{align*}
Alternatively, when $R_{xy} < \frac{\rho}{2}$, we have 
\[
 \mathbf{Pr}\left[|p_3^{-1}\cdot \# - R_{xy}| \ge \frac{1}{2}\rho\right] \le \frac{1}{n^5} \; ,
\]
which means $p_3^{-1}\cdot \# < \rho$ with probability at least $1 - \frac{1}{n^5}$.
\end{proof}

% \textbf{Theorem~\ref{theorem_adjacency}}
% \textit{
% There exists a one-pass algorithm with $\tilde{O}( \min(\epsilon^{-2}m^{2/3}/T^{1/3}, \epsilon^{-1} m^{1/2}))$ memory in the adjacency list model using a learning-based oracle that returns a $(1 \pm \epsilon)$-approximation to $T$ with probability at least $7 / 10$. 
% }
We are now ready to prove Theorem~\ref{theorem_adjacency}, restated here for the sake of convenience. 

\theoremAdjacency*
\begin{proof}
We first consider the case when $T \ge (m / \epsilon)^{1/2}$.

For each edge $xy \in H$, from Lemma~\ref{lem:adjlist_heavy} we have that with probability at least $1 - \frac{1}{n^5}$, $\# / p_3 = (1 \pm \epsilon) R_{xy}$ in Algorithm~\ref{alg:adj_tri_perfect}. If $xy \notin H$, then with probability $1 - \frac{1}{n^5}$, $xy$ will not contribute to $A_h$. Taking a union bound, we have that with probability at least $1 - 1/n^3$, 
\[
A_h / p_3 = (1 \pm \epsilon) \sum_{xy \in H} R_{xy} = (1 \pm \epsilon) T_H \; .
\]
We now turn to deal with the light and medium edges.
For a light edge $xy$, it satisfies $R_{xy} \le T / \rho$ and therefore we can  invoke  Lemma~\ref{lem:adjlist_light} with the parameter $c$ set to $\rho$.
For a medium edge $xy$, it  satisfies $R_{xy} \le \rho = T / (T / \rho)$, and therefore  we can  invoke Lemma~\ref{lem:adjlist_light} with the parameter $c$ set to $T/\rho$.
Hence, 
we have that with probability $4/5$,
\[
A_m / p_2 = T_M \pm \epsilon T,  A_l / p_1 = T_L \pm \epsilon T\; .
\]
Putting everything together, we have that with probability $7/10$,
\[
|A_h / p_3 + A_m / p_2 + A_l / p_1 - T| \le 3 \epsilon T.
\]
%which is our need. 
Now we analyze the space complexity. We note that there are at most $\rho$ medium edges. Hence, the expected total space we use is
$O(m p_3 + \rho p_2 + m p_1) = O(\epsilon^{-2} m^{2/3} / T^{1/3}\log n)$\footnote{Using Markov's inequality, we have that with probability at least $9 / 10$, the total space we use is less than $10$ times the expected total space.}. 

When $T < (m / \epsilon)^{1/2}$, as described in Section~\ref{sec:adjacency list}, we only have two classes of edges: heavy and light. We will save all the heavy edges and use sub-sampling to estimate $T_L$. The analysis is almost the same.
\end{proof}



==> Learning Augmented Triangles ICLR 22/sup_adj_noisy_oracles.tex <==
\subsection{Noisy Oracles for the Adjacency List Model}\label{sec:adj_noisy_oracles}


\begin{proof}[Proof of Theorem~\ref{thm:imperfect_adj}]

We first consider the case that $T < (m / \epsilon)^{1/2}$. Recall that at this time, our algorithms becomes that we save all the heavy edges $xy$ such that $p(e) \ge \epsilon T / \sqrt{m}$ and sampling the light edges with rate $p_l = \epsilon^{-1}/\sqrt{m}$. We define $\mathcal{L}$ as the set of deemed \light\ edges, $\mathcal{H}$ as the set of deemed \heavy\ edges and $L = |\mathcal{L}|$, $H = |\mathcal{H}|$. Let $\rho = \epsilon T / \sqrt{m}$, then we have the condition that for every edge $e$,
\[
1 - K \cdot \frac{\rho}{R_e} \le Pr[\mO(e)=\textsc{heavy}] \le K \cdot \frac{R_e}{\rho}.
\]
We will show that, $(i)$ $\mathbb{E}[H] \le (K + 1) \frac{\sqrt{m}}{\epsilon}$,  $(ii)$ $\mathbf{Var}[A_L / p_1] \le (4K +2) \epsilon^2 T^2$. Under the above conditions we can get that with probability at least $9/10$ we can get a $(1 \pm O(\sqrt{K}) \cdot \epsilon)$-approximation of $T$ by Chebyshev's inequality.

For $(i)$, we divide $\mathcal{H} = H_h \cup H_l$, where the edges in $H_h$ are indeed \heavy  edges, and the edges in $H_l$ are indeed \light  edges. Then, it is easy to see that $|H_h| \le T / \rho$.
For every light edges, the probability that it is included in $H_l$  is at most $K \cdot \frac{R_e}{\rho}$, hence we have
\[
\mathbb{E}[|H_h|] \le K \cdot \sum_{e \in \mathcal{H}}  (\frac{R_e}{\rho}) \le K \cdot \frac{T}{\rho} = K \frac{\sqrt{m}}{\epsilon}
\]
which implies $\mathbb{E}[H] \le (K + 1) \frac{\sqrt{m}}{\epsilon}$.

For $(ii)$, we also divide $\mathcal{L} = L_l \cup L_h$ similarly. Then we have $\mathbf{Var}[A_L] \le  2(\mathbf{Var}[X] + \mathbf{Var}[Y])$, where $X = \sum_{e \in L_l, e \text{ has been sampled}} R_e$, $Y = \sum_{e \in L_h, e \text{ has been sampled}} R_e$. Similar to the proof in Lemma~\ref{lem:adjlist_light}, we have 
\[
\mathbf{Var}[X] \le p_1 \sum_{e \in \mathcal{L}} R_e^2 \le p_1 \frac{T}{\rho} \rho^2 = p_1 T \rho.
\]
Now we bound $\mathbf{Var}[Y]$. For every heavy edge we have that $\mathbf{Pr}[e \in L_h] \le K \cdot \frac{\rho}{R_e}$. Then, condition on the oracle $O_\rho$, we have 
\[
\mathbb{E}[\mathbf{Var}[Y|O_{\rho}]] \le p_1 K\sum_{e \in \mathcal{H}} \frac{\rho}{R_e} R_e^2 \le p_1 K \sum_{e \in \mathcal{H}} \rho R_e \le p_1 K \rho T \;.
\]
Also, we have
\[
\mathbf{Var}[\mathbb{E}[Y|O_\rho]] < p_1 K\sum_{e \in \mathcal{H}} \frac{\rho}{R_e} R_e^2 \le p_1 K \rho T \;.
\]
From $\mathbf{Var}[Y] = \mathbb{E}[\mathbf{Var}[Y | O_\rho]] + \mathbf{Var}[\mathbb{E}[Y | O_\rho]] $ we know $\mathbf{Var}[Y] \le 2p_1 K \rho T$, which means $\mathbf{Var}[A_l / p_1] \le \frac{1}{p_1}(4K + 2) \rho T = (4K + 2) \epsilon^2 T^2$. 

When $T \ge (m / \epsilon)^{1/2}$, recall that the oracle $O_{\rho}$ only needs to predict the edges that are medium edges or light edges. So, we can use the same way to bound the expected space for the deemed medium edges and the variance of the deemed light edges.
\end{proof}


==> Learning Augmented Triangles ICLR 22/sup_adj_value_oracle.tex <==
\subsection{A Value Prediction Oracle for the Adjacency List Model}\label{sec:adj_value_oracle}

% \todo{change $t(e)$ to $N_e$}
In this section, we consider two types of  value-prediction  oracles, and variants of Algorithm~\ref{alg:adj_tri_perfect} that take advantage of these oracles. Recall that given an edge $xy$,  $R_{xy} = |z: \{x, y, z\} \in \Delta \textnormal{ and } x <_s z <_s y|$ .
%Let $N_e$ denote the number of triangles incident to the edge $e$.

% \textbf{Definition~\ref{def:value_oracle}}
% \textit{
\begin{definition}
A value-prediction oracle with parameter $(\alpha,\beta)$ is an oracle that, for any edge $e$,
%indicate if (i) $R_{xy} \le T / \beta$, or (ii) $R_{xy} > T / \beta$, and 
outputs a value $p(e)$ for which $\mathbb{E}[p(e)]\le \alpha R_e + \beta $, and $\mathbf{Pr}[p(e) < \frac{R_e}{\lambda} - \beta] \le K e^{-\lambda}$ for some constant $K$ and any $\lambda \ge 1$.
\end{definition}
%$\alpha$-approximation of $R_{xy}$ .
% }

Our algorithm is based on the following stability property of exponential random variables (see e.g.~\cite{Andoni17})

\begin{lemma}
\label{lem:exp_stable}
Let $x_1, x_2, ..., x_n > 0$ be real numbers, and let $u_1, u_2, ...u_n$ be i.i.d. standard exponential random variables with parameter $\lambda = 1$. Then we have that the random variable $\max(\frac{x_1}{u_1}, ..., \frac{x_n}{u_n}) \sim \frac{x}{u}$, where $x = \sum_i x_i$ and $u \sim \mathrm{Exp}(1)$.
\end{lemma}

\begin{lemma}
\label{lem:exp_median}
Let $r = O(\ln(1 / \delta) / \epsilon^{2})$ and $\epsilon \le 1/3$. If we take $r$ independent samples $X_1, X_2, ... , X_r$ from $\mathrm{Exp}(1)$ and let $X = \mathrm{median}(X_1, X_2, ..., X_r)$, then with probability $1 - \delta$, $X \in [\ln{2}(1-\epsilon), \ln{2}(1 + 5\epsilon)]$.
\end{lemma}
\begin{proof}
We first prove the following statement: with probability $1-\delta$, $F(X) \in [1/2-\epsilon, 1/2 + \epsilon]$, where $F$ is the cumulative density function of a standard exponential random variable.

Consider the case when $F(X) \le 1/2 - \epsilon$. We use the indicator variable $Z_i$ where $Z_i = 1$ if $F(X_i) \le 1/2 - \epsilon$ or $Z_i = 0$ otherwise. Notice that when $F(X) \le 1/2 - \epsilon$, at least half of the $Z_i$ are $1$, so $Z = \sum_i Z_i \ge r / 2$. On the other hand, we have $\mathbb{E}[Z] = r / 2 - r \epsilon$, by a Chernoff bound. We thus have 
\[
\mathbf{Pr}[|Z - \mathbb{E}[Z]| \ge \epsilon r] \le 2e^{-\epsilon^{2}r/3} \le \delta / 2\; .
\]
Therefore, we have with probability at most $\delta/2$, $F(X) \le 1/2 - \epsilon$. Similarly, we have that with probability at most $\delta / 2$, $F(X) \ge 1/2 + \epsilon$. Taking a union bound, we have that with probability at least $1-\delta$, $F(X) \in [1/2-\epsilon, 1/2 + \epsilon]$.

Now, condition on $F(X) \in [1/2-\epsilon, 1/2 + \epsilon]$. Note that $F^{-1}(x) = -\ln(1 - x)$, so if we consider the two endpoints of $F(X)$, we have 
\[
F^{-1} (1/2 -\epsilon) = -\ln(1/2 + \epsilon) \ge (1-\epsilon)\ln{2},
\]
and
\[
F^{-1} (1/2 +\epsilon) = -\ln(1/2 - \epsilon) \le (1+5\epsilon)\ln{2}.
\]
which indicates that $X \in [\ln{2}(1-\epsilon), \ln{2}(1 + 5\epsilon)]$.
\end{proof}

 The algorithm utilizing this oracle is shown in Algorithm~\ref{alg:4}. As described in Section~\ref{sec:adjacency list}, here we runs $O(\frac{1}{\epsilon^2})$ copies of the subroutine and takes a medium of them. For each subroutine, we aim to output the maximum value $\max_e R_e / u_e$. We will show that with high probability for each subroutine, this maximum will be at least $T/\log(K/\eps)$. Hence, we only need to save the edge $e$, such that $(R_e + \beta) / u_e$ is larger than $T / \log(K/\eps)$. However, one issue here is we need the information of $T$. We can remove this assumption when $\beta = 0$ using the following way: we will show that with high probability, the total number of edges we save is less than $H = O(\frac{1}{\epsilon^2} \log^2 (K/\eps) (\alpha + m\beta / T)) $, so every time when a new edge comes, we can search the minimum value $M$ such that the total number of edges $e$ that in at least one subroutine $(p(e) + \beta)/u_e > M$ is less than $H$(we count an edge multiple times if it occurs in multiple subroutines), then use $M$ as the threshold. We can see $M$ will increase as the new edge arriving and it will be always less than $H$. 
 %For the light edges, from the assumption of the oracle we know that $R_{xy} \le T / \beta$, we can sub-sample with sampling rate $O(\epsilon^{-2} \beta)$ to estimate $T_L$. For the heavy edges, we can obtain an $\alpha$-approximation to $R_{xy}$ from the oracle at this time. As shown in our algorithm, we run $O(\epsilon^{-2})$ copies of the subroutine and we will show that each subroutine will output the maximum value of $R_{xy} / u_{xy}^i$ with high probability, where the $u_{e}^i$ are exponential random variables. From Lemma~\ref{lem:exp_stable} and Lemma~\ref{lem:exp_median} we can obtain $O(\epsilon^{-2})$ independent samples from $T_H / u$, where $u \sim \mathrm{Exp}(1)$, and after taking a median among all samples we can obtain a $(1 \pm \epsilon)$-approximation to $T_H$.

\begin{algorithm}[!ht]
   \caption{Counting Triangles in the Adjacency List Model with a Value Prediction Oracle}
   \label{alg:4}
\begin{algorithmic}[1]
   \STATE {\bfseries Input:} Adjacency list edge stream and an value prediction oracle with parameter$(\alpha, \beta)$. 
   \STATE {\bfseries Output:} An estimate of the number $T$ of triangles.
   \STATE Initialize $X \leftarrow \emptyset$ and $H = O(\frac{1}{\epsilon^2} \log^2 (K/\eps) (\alpha + m\beta / T))$, and let $c$ be some large constant.
   %\STATE On :$H = O(T)$
   \FOR[Initialize sets for $c \epsilon^{-2}$ copies of samples, where $S_i$ stores edges, $Q_i$ stores all the exponential random variables for each sampled edge, and $A_i$ stores the current maximum of each sample]{$i = 0$ {\bf to} ${c \epsilon^{-2}}$}
        \STATE $S^{i} \leftarrow \emptyset, Q^{i} \leftarrow \emptyset$, and $A^i \leftarrow 0 $ \; .
   \ENDFOR 
    \WHILE{seeing edges adjacent to $y$ in the stream}
    \FOR[Update the counters for each sample]{$i = 0$ {\bf to} ${c \epsilon^{-2}}$}
    \STATE For all $ab \in S^i$: if $a, b \in N(y)$ then $C_{ab}^i \leftarrow C_{ab}^i + 1$\;
    \ENDFOR
    %  \ENDFOR
    \FOR{each incident edge $yx$}

        \FOR{$i = 0$ {\bf to} ${c \epsilon^{-2}}$} 
            \IF[Finished counting $C_{xy}$, update the current maximum]{$xy \in S^i$} 
            \STATE $A^i \leftarrow \max(A^i,  C_{xy}^i / u_{xy}^i)$ \;.
            \ELSE[Put $yx$ into the sample sets temporarily]
            \STATE Let $\hat{R}_{yx}$ be the predicted value of $R_{yx}$.
            \STATE $\hat{R}_{yx} \leftarrow \hat{R}_{yx} + \beta$.
            \STATE Generate $u_{yx}^i \sim \mathrm{Exp}(1)$. Set $Q^i \leftarrow Q^i \cup \{u_{yx}^i\}, S^i \leftarrow S^i \cup \{yx\}$.
            \ENDIF
        \ENDFOR
    \ENDFOR
    \STATE Set $M$ to be the minimal integer such that $\sum_i s_i \le H$, where $s_i = |\{e \in E \ | \  \hat{R}_{e}/u_{e}^{i} \ge M \}|$.
     \FOR[Adjust the samples to be within the space limit]{$i = 0$ {\bf to} ${c \epsilon^{-2}}$} 
      \STATE Let $Q^i \leftarrow Q^i \setminus \{u_{ab}^i\}, S^i \leftarrow S^i \setminus \{ab\}$ if $\hat{R}_{ab}/u_{ab}^i < M$ for all $ab \in E$.
      \ENDFOR
    \ENDWHILE
    \FOR{$i = 0$ {\bf to} ${c \epsilon^{-2}}$}
        \STATE $X \leftarrow X \cup \{A^i\}$
   \ENDFOR
    \STATE {\bfseries return:} $\ln{2} \cdot \mathrm{median}(X) $ \; .
\end{algorithmic}
\end{algorithm}

We are now ready to prove Theorem~\ref{thm:value_oracle:1}. We first recall the theorem.
\thmAdjValueOne*

\begin{proof}

It is easy to see that for the $i$-th subroutine, the value $f(i) = \max_e R_{e} / u_{e}^i$ is the sample from the distribution $T/u$, where $u \sim \mathrm{Exp}(1) $. And if the edge $e_i$, for which the true value $R_{e_i} / u_{e_i}^i$ is the maximum value among $E$, is included in $S^i$, then the output of the $i$-th subroutine will be a sample from $T / u$. Intuitively, the prediction value $p(e)$ will help us find this edge.

We will first show that with probability at least $9/10$ the following events will happen:
\begin{itemize}
    \item $(i)$ $f(i) \ge c_1 T / \log(1 / \epsilon)$ for all $i$, where $c_1$ is a constant.
    \item $(ii)$ Let $s_i$ be the number of the edge $e$ in the $i$-th subroutine such that $(p(e) + \beta) / u_e^i \ge c_1^2 T / \log^2(K / \epsilon)$, then $\sum_i s_i \le c_2(\frac{1}{\epsilon^2} \log^2 (K/\eps) (\alpha + m\beta / T))$ for some constant $c_2$.
    \item $(iii)$ $p(e_i) + \beta \ge c_1 f(i) /\log(K/ \epsilon)$ for all $i$.
\end{itemize}

For $(i)$, recall that $f(i) \sim T / u,$ where $u \sim \mathrm{Exp}(1)$. Hence, we have 
\[
\mathbf{Pr}[f(i) < c_1 T / \log(1 / \epsilon)] = e^{-\log(1/\epsilon) / c_1} \le\frac{1}{100 c}\frac{1}{\epsilon^2} \; .
\]
Taking an union bound we get that with probability at least $99/100$, $(i)$ will happen. For each edge $e$, we have 
\[
\mathbf{Pr} [p(e) + \beta < R_e / \lambda] < K e^{-\lambda},
\]
similarly we can get that with probability at least $99/100$, $(iii)$ will happen.

For $(ii)$, we first bound the expectation of $s_i$. For each edge $e$, we have %\[\]
\begin{align*}
\mathbf{Pr} \left[(p(e) + \beta) / u_e^i \ge c_1^2 T / \log^2(K/\eps)\right]&= 
\mathbf{Pr} [u_e \le c_1^2 (p(e) + \beta) \log^2(K/\eps) / T] \\
& \le c_1^2(p(e) + \beta) \log^2(K/\eps) / T \\& \le c_1^2(\alpha R_e + 2\beta) \log^2(K/\eps) / T
\; .
\end{align*}
Hence, we have 
\[
\mathbb{E}[s_i] = \sum_e c_1^2\frac{(\alpha R_e + 2\beta) \log^2(K/\eps)}{T} = O(\log^2(K/\eps)(\alpha + m\beta / T)).
\]
Using Markov's inequality, we get that with probability at least $99/100$, $(ii)$ will happen.
Finally, taking a union bound, we can get with probability at least $9/10$, all the three events will happen.

Now, conditioned on the above three events, we will show that all the subroutine $i$ will output $f(i)$.
For the subroutine $i$, from $(ii)$ we know that $M$ will be always smaller than $O(T / \log^2(K / \epsilon))$, and from $(i)$ and $(iii)$ we get that $(p(e_i)+ \beta) / u_{e_i}^i \ge \Omega(T / \log^2(K / \epsilon))$. Hence, the edge $e_i$ will be saved in the subroutine $i$. From Lemma~\ref{lem:exp_median} we get that with probability at least $7/10$, we can finally get a $(1 \pm \epsilon)$-approximation of $T$. 
\end{proof}
We note that when $\beta = 0$, the space complexity will become $O(\frac{1}{\epsilon^2} \log^2 (K/\eps) \alpha )$, and in this case we will not need a lower bound of $T$.

We will also consider the following noise model.

\begin{definition}
A value-prediction oracle with parameter $(\alpha,\beta)$ is an oracle that, for any edge $e$,
%indicate if (i) $R_{xy} \le T / \beta$, or (ii) $R_{xy} > T / \beta$, and 
outputs a value $p(e)$ for which $\mathbf{Pr}[p(e) > \lambda \alpha R_e + \beta] \le \frac{K}{\lambda}$ , and $\mathbf{Pr}[p(e) < \frac{R_e}{\lambda} - \beta] \le \frac{K}{\lambda}$ for some constant $K$ and any $\lambda \ge 1$.
\end{definition}
% \begin{remark}
% An alternative way to solve this problem is to divide the triangles into the intervals $[0, T/\beta], [2T/ \beta, 4T/ \beta],..., [2^i T/\beta, 2^{i+1} T / \beta], ...$ and put the edges into the intervals according to the predicted value the oracle gives. For the edges in interval $[2^i T / \beta, 2^{i + 1} T / \beta]$, we can sub-sample with rate $O(\epsilon^{-2} \alpha 2^{i + 1} /\beta )$. The total space we use will be $\tilde{O}(\epsilon^{-2} (m / \beta + \alpha \log n))$.
% \end{remark}

The algorithm for this oracle is shown in Algorithm~\ref{alg:value_prediction:2}. 

\begin{algorithm}[!h]
   \caption{Counting Triangles in the Adjacency List Model with a Value Prediction Oracle}
   \label{alg:value_prediction:2}
\begin{algorithmic}[1]
   \STATE {\bfseries Input:} Adjacency list edge stream and an value prediction oracle with parameter$(\alpha, \beta)$. 
   \STATE {\bfseries Output:} An estimate of the number $T$ of triangles.
   \STATE Initialize $S_i^j \leftarrow \emptyset$ and $A_i^j \leftarrow 0$ where $i = O(\log n)$ and $j = O(\log \log n)$. $p_0 = c \epsilon^{-2} 2^i \beta / T$ and $p_i = c \epsilon^{-2} 2^i \beta (\log n)^2/ T$ for some constant $c$. Define $I_0 = [0, 2\beta)$ and $I_i = [2^i\beta, 2^{i + 1} \beta)$, $H \leftarrow 0$.
   
   
    \WHILE{seeing edges adjacent to $y$ in the stream} 
    \STATE For all $ab \in S_i^j$: if $a, b \in N(y)$ then $C_{ab} \leftarrow C_{ab} + 1$\; % ^j
    %  \ENDFOR
    \FOR{each incident edge $yx$}
            \IF{$xy \in S_i^j$} 
            \STATE $A_i^j \leftarrow A_i^j + C_{yx} $ \;.
            \ELSE
            \STATE Let $\hat{R}_{yx}$ be the predicted value of $R_{yx}$.
            \STATE Search $i$ such that $(\hat{R}_{yx} + \beta) \in I_i$
            \STATE For each $j$ let $S_i^j \leftarrow S_i^j \cup \{yx\}$ with probability $p_i$.
            \ENDIF
    \ENDFOR
    \ENDWHILE
    \FOR{$i = 0$ {\bf to} $O(\log n)$}
        \STATE $H \leftarrow H + \mathrm{median}(A_i^j) / p_i$
   \ENDFOR
    \STATE {\bfseries return:} $H$ \; .
\end{algorithmic}
\end{algorithm}

 We now state our theorem.

\begin{restatable}{thm}{thmAdjValueTwo}
\label{thm:value_oracle:2}
Given an oracle with parameter $(\alpha, \beta)$, there exists a one-pass algorithm, Algorithm~\ref{alg:value_prediction:2}, with space complexity $O(\frac{K}{\epsilon^2} \left(\alpha(\log n)^3 \log \log n  + m\beta / T\right))$ in the adjacency list model that returns a $(1 \pm \sqrt{K} \cdot \epsilon)$-approximation to $T$ with probability at least $7 / 10$. 
\end{restatable}



\begin{proof}
Define $q(e) = p(e) + \beta$, it is easy to see that from the condition we can get that
\[
\mathbf{Pr}[q(e) > 2\lambda \alpha R_e] \le K \frac{1}{\lambda} \ \  \mathrm{when} \ \ R_e > 2 \beta,  \mathbf{Pr}\left[q(e) < \frac{R_e}{\lambda}\right] \le K \frac{1}{\lambda}
\]
% for some constant $K_2$.

We define the set $E_i$ such that $e \in E_i$ if and only if $q(e) \in I_i$. We can see $\mathbb{E}[A_i / p_i] = \sum_{e \in E_i} R_e$. Now, we bound $\mathbf{Var} [A_i / p_i]$ when $i \ge 1$.

Let $X = \sum_{e \in E_i, R_e \le 2^{i + 1}\beta} R_e$ and $Y =  \sum_{e \in E_i, R_e > 2^{i + 1} \beta} R_e$, then we have $\mathbf{Var}[A_i] \le 2(\mathbf{Var}[X] + \mathbf{Var}[Y])$.

Similar to the proof in Lemma~\ref{lem:adjlist_light}, we can get that 
\[
\mathbf{Var}[X] \le p_i \sum_{e \in E_i, R_e \le 2^{i + 1} \beta} R_e^2 \le p_i (2^{i + 1} \beta)^2 \frac{T}{2^{i + 1} \beta} = p_i 2^{i + 1} \beta T.
%\frac{1}{p_i} \sum_{e \in E_i} t(e)^2 
%= \frac{1}{p_i} \left(\sum_{t(e) \in E_i, t(e) \le 2^{i + 1} \beta} t(e)^2
%+ \sum_{t(e) \in E_i, t(e) \ge 2^{i + 1} \beta} t(e)^2 \right)
%\]
%For the first term, we have
%\[
%\sum_{t(e) \in E_i, t(e) \le 2^{i + 1} \beta} t(e)^2 \le (2^{i + 1} \beta)^2 \frac{T}{2^{i + 1} \beta} 
%= 2^{i + 1} \beta T
\]
For $\mathbf{Var}[Y]$, recall that for an edge $e$ such that $R_e \ge 2^{i + 1} \beta$, we have $\mathbf{Pr} [e \in E_i] \le K \frac{q(e)}{R_e} \le K \frac{2^{i + 1} \beta}{R_e}$. Then, condition on the oracle $O_\theta$, we have
% \[
% \sum_{t(e) \in E_i, t(e) \ge 2^{i + 1} \beta} t(e)^2
% \]
\[
\mathbb{E}[\mathbf{Var}[Y | O_\theta]] \le p_i\sum_{R_e \ge 2^{i + 1}\beta} K \frac{2^{i + 1} \beta}{R_e} R_e^2 = p_i K 2^{i + 1} \beta \sum_{R_e \ge 2^{i + 1}\beta} R_e = p_i K 2^{i + 1} \beta T.
\]
And
\[
\mathbf{Var}[\mathbb{E}[Y | O_\theta]] < p_i \sum_{R_e \ge 2^{i + 1}\beta} K \frac{2^{i + 1} \beta}{R_e} R_e^2 = p_i K 2^{i + 1} \beta T.
\]
From $\mathbf{Var}[Y] = \mathbb{E}[\mathbf{Var}[Y | O_\theta]] + \mathbf{Var}[\mathbb{E}[Y | O_\theta]] $ we get that $\mathbf{Var}[Y] \le  2p_i K 2^{i + 1} \beta T$, from which we can get that $\mathbf{Var}[A_i / p_i] = \frac{1}{p_i^2} \mathbf{Var}[A_i] = O(K(\epsilon / \log n)^2 T^2)$. Using Chebyshev’s inequality and taking a median over $O(\log \log n)$ independent trials, we can get $X_i = \mathrm{median}(A_i^j)$ satisfies $|X_i - \sum_{e \in E_i} R_e| \le \sqrt{K}(\epsilon / \log n) T$ with probability $1 - O(1 / \log n)$. A similar argument also holds for $I_0$, which means that after taking a union bound, with probability $9 / 10$, the output of the algorithm~\ref{alg:value_prediction:2} is a $(1 \pm \sqrt{K} \cdot \epsilon)$- approximation of $T$.

Now we analyze the space complexity of Algorithm~\ref{alg:value_prediction:2}.

For $i \ge 1$, we have %\[\]
\begin{align*}
\mathbb{E}\left[|E_i|\right] & = \mathbb{E}\left[\sum_{R_e \le 2^{i - 1}\beta / \alpha} [e \in E_i] + \sum_{R_e > 2^{i - 1}\beta / \alpha} [e \in E_i] \right] 
\le \mathbb{E}\left[\sum_{R_e \le 2^{i - 1}\beta / \alpha} [e \in E_i]  \right] + \frac{T \alpha}{2^{i - 1}\beta} \\
& \le \sum_{R_e \le 2^{i - 1}\beta / \alpha} 2K \frac{R_e}{p(e)} + \frac{T \alpha}{2^{i - 1}\beta} \le \sum_{R_e \le 2^{i - 1}\beta / \alpha} K\frac{R_e}{2^{i - 1} \beta} + \frac{T \alpha}{2^{i - 1}\beta} \le (K +1) \frac{T\alpha}{2^{i - 1}\beta},
\end{align*}
and $|E_0| \le m$, hence we have that the total expectation of the space is $\sum_i p_i \mathbb{E}[|E_i|]$ = $O(\frac{K}{\epsilon^2} \left(\alpha(\log n)^3 \log \log n + m\beta / T\right))$.
\end{proof}




==> Learning Augmented Triangles ICLR 22/sup_arbitrary_order.tex <==
\section{Omitted Proofs from Section~\ref{sec:arbitrary_main}}\label{sec:arbitrary_missing}

We first present Algorithm~\ref{alg:arb_tri_perfect}, and then continue to prove Theorem~\ref{theorem_arbitrary}. In the following algorithm, for two sets $A, B$ of edges, we let $w_{A, B}$ represent the set of pairs of edges $(u, v)$, where $u \in A, v \in B$, and $u, v$ share a common vertex.

\begin{algorithm}[H]
    \centering
  \caption{Counting Triangles in the Arbitrary Order Model}
  \label{alg:arb_tri_perfect}
\begin{algorithmic}[1]
   \STATE {\bfseries Input:} Arbitrary order edge stream and an oracle $\mO$ that outputs \textsc{heavy} if $N_{xy} > \rho$ and \textsc{light} otherwise.
   \STATE {\bfseries Output:} An estimate of the triangle count $T$.
   \STATE Initialize $\rho=\max\big\{\frac{\eps T}{\sqrt{m}}, 1\big\}$, $p=C\max\big\{\frac{1}{\eps\sqrt{T}},\frac{\rho}{\eps^2\cdot T}\big\}$ for a constant $C$.
   \STATE Initialize $\ell_1, \ell_2, \ell_3 = 0$, and $\mS, \mH = \emptyset$.
   \FOR{every arriving edge $e$ in the stream}
        \IF{the oracle $\mO$ outputs \textsc{heavy}}
            \STATE Add $e$ to $\mH$
        \ELSE
            \STATE Add $e$ to $\mS$ with probability $p$.
        \ENDIF
        \FOR{each $w \in w_{\mS, \mS}$}
            \IF{$(e, w)$ is a triangle}
                \STATE Increment $\ell_{1}=\ell_{1}+1$.
            \ENDIF
        \ENDFOR
        \FOR{each $w \in w_{\mS, \mH}$}
            \IF{$(e, w)$ is a triangle}
                \STATE Increment $\ell_{2}=\ell_{2}+1$.
            \ENDIF
        \ENDFOR
        \FOR{each $w \in w_{\mH, \mH}$}
            \IF{$(e, w)$ is a triangle}
                \STATE Increment $\ell_{3}=\ell_{3}+1$.
            \ENDIF
        \ENDFOR
   \ENDFOR
   \STATE \textbf{return:} $\ell = \ell_1/p^2+ \ell_2/p+\ell_3$.
\end{algorithmic}
\end{algorithm}

\subsection{Proof of  Theorem~\ref{theorem_arbitrary}}\label{subsec:proof_arbitrary}

 Recall that we first assume that  Algorithm~\ref{alg:arb_tri_perfect} is given access to a perfect  oracle $\mO$.
That is, for every edge $e\in E$,
\[
\mO(e) =
\begin{cases}
\textsc{light} & \text{if } T_e \leq \rho\\
\textsc{heavy} & \text{if } T_e > \rho,
\end{cases}
\]
where $T_e$ as the number of triangles incident to the edge $e$.

\begin{proof}[Theorem~\ref{theorem_arbitrary}]
First, we assume that $T \ge \eps^{-2}$. If not, our algorithm can just store all of the edges, since $m \le \eps^{-1} \cdot m/\sqrt{T}.$

For each integer $i \ge 1,$ let $\mathcal{E}(i)$ denote the set of edges that are part of exactly $i$ triangles, and let $E_i = |\mathcal{E}(i)|$. Since each triangle has $3$ edges, we have that $\sum_{i \ge 1} i \cdot E(i) = 3T.$

Let $\mT_{1}$ denote the set of triangles 
whose first two edges in the stream are light (according to $\mO$).
For every triangle $t_i$ in $\mT_1$, let $\chi_i$ denote the indicator of the event that the first two edges of $t_i$ are sampled to $\mS$, and let $\ell_1=\sum_i \chi_i$.
Since each $\chi_i$ is $1$ with probability $p^2$,
$\EX[\chi_i]=p^2$, and  $\Var[\chi_i] = p^2-p^4 \leq p^2$. 
For any two  variables $\chi_i, \chi_j,$ they must be uncorrelated unless the triangles $t_i, t_j$ share a light edge that is among the first two edges of $t_i$ and among the first two edges of $t_j$. Moreover, in this case, $\Cov[\chi_i, \chi_j] \le \EX[\chi_i \chi_j] = \mathbb{P}(\chi_i = \chi_j = 1).$ This event only happens if the first two edges of both $t_i$ and $t_j$ are sampled in $\mS$, but due to the shared edge, this comprises $3$ edges in total, so $\mathbb{P}(\chi_i = \chi_j = 1) = p^3$.
Hence, if we define $t_i^{12}$ as the first two edges of $t_i$ in the stream for each triangle $t_i$, $$\EX[\ell_1] = p^2|\mT_1|,$$ and 
\begin{align*}
    \Var[\ell_1] 
    & \le\sum_{t_i\in \mT_1}p^2+ \sum_{\substack{t_i, t_j \in \mT_1\\ t_i^{12} \cap t_j^{12}\neq \emptyset}} p^3
    \;\le\; p^2 |\mT_1| + p^3 \sum_{T_e \le \rho} T_e^2 \\
    &= p^2 |\mT_1| + p^3 \cdot \sum_{t = 1}^{\rho} t^2 \cdot E(t) 
    \;\leq\; (p^2 + 3 p^3 \cdot \rho) \cdot T \;\;.
\end{align*}
    The first line follows by adding the covariance terms; the second line follows since each light edge $e$ has at most $T_e^2$ pairs $(t_i, t_j)$ intersecting at $e$; the third line follows by summing over $t = T_e$, ranging from $1$ to $\rho$, instead over $e$; and the last line follows since $\sum_{t \ge 1} t \cdot E(t) = 3T$.

Now, let $\mT_2$ denote the set of triangles whose first two edges in the stream are light and heavy (in either order). 
For every triangle $t=(e_1, e_2, e_3)$ in $\mT_2$, $e_1, e_2$ are sampled to $\mS\cup \mH$ with probability $p$. Also all other triangles have no chance to contribute to $\ell_2$.
Hence, $\EX[\ell_2]=p\cdot \mT_2$.
Also, two triangles $t_i, t_j\in \mT_2$ that intersect on an edge $e$ have $\Cov(\chi_i, \chi_j) \neq 0$ only if $e$ is light and $e \in t_i^{12}, t_j^{12}$. 
%\textcolor{blue}{
In this case. \[\Cov(\chi_i, \chi_j) \le \EX[\chi_i \chi_j] \le p,\] since if $e$ is added to $\mS$ (which happens with probability $p$) then $\chi_i=\chi_j=1$ as the other edges in $t_i^{12}, t_j^{12}$ are heavy and are added to $\mH$ with probability 1.
Therefore,  
\[\Var[\ell_2] = \sum_{t_i\in \mT_2}p + \sum_{\substack{t_i, t_j \in \mT_2 \\ t_i^{12} \cap t_j^{12} =e, \; \mO(e)=\textsc{light}}} p \le (p + 3p \cdot \rho) \cdot T,\]
by the same calculations as was done to compute $\Var[\ell_1].$

Finally, let $\mT_3$ denote the set of triangles whose first two edges in the stream are heavy. 
Then $\ell_3=|\mT_3|$.

Now, using the well known fact that $\Var[X+Y] \le 2(\Var[X]+\Var[Y])$ for any (possibly correlated) random variables $X, Y,$ we have that 
\begin{align*}
    \Var[p^{-2} \ell_1 + p^{-1} \ell_2 + \ell_3]
    &\le  2 \left(p^{-4} (p^2 + 3p^3 \rho) T + p^{-2} (p + 3p \rho) T\right) \\
    & \le  4T (p^{-2} + 3 p^{-1} \rho),
\end{align*} 
since $\ell_3$ has no variance. Moreover, $\EX[p^{-2} \ell_1 + p^{-1} \ell_2 + \ell_3] = |\mT_1| + |\mT_2|+|\mT_3| = T$. So, by Chebyshev's inequality, since $\ell = \ell_1/p^2 + \ell_2/p + \ell_3,$
\[
\Pr[|\ell-T|>\eps T] < \frac{\Var[\ell]}{\eps^2 \cdot T^2} < \frac{4(p^{-2} + 3p^{-1} \rho)}{\eps^2 \cdot T}\;.\]
Therefore, setting $p=C \cdot \max\left\{1/(\eps \cdot \sqrt{T}), \rho/(\eps^2 \cdot T)\right\}$ for some fixed constant $C$ implies that, with probability at least $2/3$, $\ell$ is a $(1\pm\eps)$-multiplicative estimate of $T$.

Furthermore, the expected space complexity is $O(mp+ \mH )=O( mp+ T/\rho)$.
Setting $\rho=\max\{\eps T/\sqrt{m}, 1\}$ implies that the space complexity is $O(\eps^{-1} m/\sqrt{T} + \eps^{-2} m/T + \eps^{-1} \sqrt{m} \cdot T/T) = O(\eps^{-1} m/\sqrt{T} + \eps^{-1} \sqrt{m} \cdot T/T)$, since we are assuming that $T \ge \eps^{-2}$. Hence, assuming that $T$ is a constant factor approximation of $T$, the space complexity is $O(\eps^{-1} m/\sqrt{T} + \eps^{-1} \sqrt{m}).$
\end{proof}




\subsection{Proof of Theorem~\ref{theorem_arbitrary}  for the K-noisy oracle}\label{subsec:proof_noise_arbitrary}
In this section, we prove Theorem~\ref{theorem_arbitrary} for the case that the given oracle is a $K$-noisy oracle, as defined in Definition~\ref{dfn:noisy-oracle}.  
That is, we prove the following:
% \begin{restatable}{thm}{thmAdjImpertArbitrary}
\begin{theorem}
\label{thm:imperfect_arbitrary}
Suppose that the  oracle in Algorithm~\ref{alg:arb_tri_perfect} is a $K$-noisy oracle as defined in Definition~\ref{dfn:noisy-oracle} for a fixed constant $K$.
  Then with probability $2/3$, Algorithm~\ref{alg:arb_tri_perfect} returns $\ell \in (1\pm\eps)T$, and uses space at most $O\left(\eps^{-1}\left(m/\sqrt{T}+ \sqrt{m}\right)\right)$.
% \end{restatable}
\end{theorem}

Recall that in Definition~\ref{dfn:noisy-oracle}, we defined a $K$-noisy oracle if the following holds.
For every edge $e$, $1 - K \cdot \frac{\rho}{N_e} \le \Pr[\mO(e)=\textsc{heavy}] \le K \cdot \frac{N_e}{\rho}$.
We first visualize this model. To visualize this error model, in Figure \ref{fig:heavy_prob} we have plotted $N_e$ versus the range $\left[1 - K \cdot \frac{\rho}{N_e}, K \cdot \frac{N_e}{\rho}\right]$ for $K = 2$.
We set $N_e$ to vary on a logarithmic scale for clarity. For example, if $N_e$ exceeds the threshold $\rho$ by a factor of $2$, there is no restriction on the oracle output, whereas if $N_e$ exceeds $\rho$ by a factor of $4$, then the oracle must classify the edge as heavy with probability at least $0.5$. In contrast, the blue piece-wise line shows the probability $\Pr[\mO(e) = \textsc{heavy}]$ if the oracle $\mO$ is a perfect oracle.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.5\linewidth]{OldStuff/MITGang/images/Heavy_Prob_3.png}
    \caption{Plot of $N_e$, the number of triangles containing edge $e$, versus the allowed oracle probability range $\Pr[\mO(e) = \textsc{heavy}]$, shaded in orange. The blue piece-wise line shows the probability $\Pr[\mO(e) = \textsc{heavy}]$ if the oracle $\mO$ is a perfect oracle.}
    \label{fig:heavy_prob}
\end{figure}


 \begin{proof}[Proof of Theorem~\ref{thm:imperfect_arbitrary}]
 We follow the proof of Theorem 4.1 from the main paper.
Let $\mT_1$ be the set of triangles  such that their first two edges in the stream are \light\ according to the oracle. Let $\mT_2$ be the set of triangles such that their first two edges in the stream are determined \light\ and \heavy\ according to the oracle. Finally, let $\mT_3$ be the set of triangles for which their first two edges are determined \heavy\ by the oracle.
Furthermore, we define $\chi_i$ for each triangle $t_i$, $t(e)$ for each edge $e$, and $\mathcal{E}(i), E_i$ for each $i \ge 1$ as done in Theorem 4.1. Finally, we define $\mathcal{L}(i)$ as the set of deemed \light\ edges that are part of exactly $i$ triangles, and $L(i) = |\mathcal{L}(i)|.$

First, note that the expectation (over the randomness of $\mO$) of $L(i)$ is at most $E(i) \cdot K \cdot \frac{\rho}{i}$, since our assumption on $\Pr[\mO(e) = \heavy]$ tells us that $\Pr[\mO(e) = \light] \le K \cdot \frac{\rho}{i}$ if $t(e) = i$. Therefore, by the same computation as in Theorem 4.1, we have that, conditioning on the oracle, $\EX[\ell_1|\mO] = p^2|\mT_1]$ and 
\begin{align*}
    \Var[\ell_1|\mO] &=\sum_{t_i\in \mT_1}p^2+ \sum_{\substack{t_i, t_j \in \mT_1\\ t_i^{12} \cap t_j^{12}\neq \emptyset}} p^3 \\
    &\le p^2 |\mT_1| + p^3 \sum_{e \text{ } \light} t(e)^2\\
    &= p^2 |\mT_1| + p^3 \cdot \sum_{t \ge 1} t^2 \cdot L(t)
\end{align*}
But since $\EX_{\mO}[L(t)] \le \frac{K \cdot \rho}{t} \cdot E(t)$ for all $t$, we have that
\begin{align*}
    \EX_{\mO}[\Var[\ell_1|\mO]] &\le \EX_{\mO}\biggr[p^2 \cdot |\mT_1|+p^3 \cdot \sum_{t \ge 1} t^2 L(t)\biggr]\\
    &= p^2|\mT_1|+K \rho \cdot p^3 \sum_{t \ge 1} t \cdot E(t)\\
    &\le (p^2 + 3 K p^3 \cdot \rho) \cdot T.
\end{align*}

A similar analysis to the above shows that $\EX[\ell_2]=p\cdot |\mT_2|$ and that
\begin{align*}
    \EX_{\mO}[\Var[\ell_2|\mO]] &\le \EX_{\mO}\biggr[p \cdot |\mT_2|+p \cdot \sum_{t \ge 1} t^2 L(t) \biggr] \\
    &= p|\mT_2|+K \rho \cdot p \sum_{t \ge 1} t \cdot E(t)\\
    &\le (p + 3 K p \cdot \rho) \cdot T.
\end{align*}
Hence, as in Theorem 4.1, we have $\EX[\ell|\mO] = T$ and $\EX_{\mO}[\Var[\ell|\mO]] \le 4T \cdot (p^{-2} + 3 K p^{-1} \rho).$ Thus, $\EX[\ell] = \EX[\EX[\ell|\mO]] = T$ and $\Var[\ell] = \EX_{\mO}[\Var[\ell|\mO]] + \Var_{\mO}[\EX[\ell|\mO]] \le 4T \cdot (p^{-2} + 3 K p^{-1} \rho)$ by the laws of total expectation/variance. Therefore, since $K$ is a constant, the variance is the same as in Theorem 4.1, up to a constant. Therefore, we still have that $\ell \in (1 \pm O(\eps)) \cdot T$ with probability at least $2/3.$

Finally, the expected space complexity is bounded by 
\begin{align*}
mp+\sum_{e \in m} Pr[\mO(e)=\heavy] &\le mp + \sum_{t \ge 1} E(t) \cdot K \cdot \frac{t}{\rho} \\
&= mp + \frac{K}{\rho} \cdot \sum_{t \ge 1} E(t) \cdot t \\
&= O(mp+T/\rho),    
\end{align*}
since $\sum_{t \ge 1} E(t) \cdot t = 3T$ and $K = O(1)$.
Hence, setting  $\rho$ and $p$ as in the proof of Theorem 4.1 implies that the returned value is a $(1\pm\eps)$-approximation of $T$, and the the space complexity is $O(\eps^{-1}(m/\sqrt{T}+\sqrt m))$ as before.
\end{proof}





\input{arbitrary_lower_bound}


==> Learning Augmented Triangles ICLR 22/supp_four_cycles.tex <==
\section{Four-Cycle Counting in the Arbitrary Order Model}\label{sec:four_cycles_appendix}

In the 4-cycle counting problem, for each $xy \in E(G)$, define $N_{xy} = |z, w: \{x, y, z, w\} \in \square|$ as the number of 4-cycles attached to edge $xy$. 


In this section, we present the one-pass $\tilde{O}(T^{1 / 3} + \epsilon^{-2}m / T^{1/3})$ space algorithm behind Theorem~\ref{theorem_four_cycle} and the proof of the theorem.\footnote{We assume$\frac{1}{T^{1/6}} \le O(\epsilon)$, which is the same assumption as in previous work} %.



\label{sec:four_cycle_intuition}
We begin with the following basic idea. 
% \todo{Fix Itemize Section?}
\begin{itemize}%[topsep=0pt,itemsep=0pt,partopsep=0pt, parsep=0pt]
    \item Initialize: $C \leftarrow 0, S \leftarrow \emptyset$. On the arrival of edge $uv$:
    \begin{itemize}
        \item With probability $p$, $S \leftarrow \{uv\} \cup S$.
        \item $C \leftarrow C + |\{\{w, z\}: uw, wz \ \textnormal{and} \ zv \in S\}|$.
    \end{itemize}
    \item Return  $C / p^3$.
\end{itemize}
Following the analysis in~\cite{SV20}, we have 
\[
\textbf{Var}[C] \le O(T p^3 + T\Delta_E p^5 + T\Delta_W p^4) \; ,
\]
where $\Delta_E$ and $\Delta_W$ denote the maximum number of 4-cycles sharing a single edge or a single wedge.
%,  means the maximum number of 4-cycles sharing a single wedge. 

There are two important insights from the analysis: first, this simple sampling scheme can output a good estimate to the number of 4-cycles on graphs that do not have too many heavy edges and heavy wedges (the definitions of heavy will be shown later). Second, assuming that we can store all the heavy edges, then at the end of the stream we can also estimate the number of 4-cycles that have exactly one heavy edge but do not have heavy wedges.
%: for each heavy edge $uv$, we compute the number of 4-cycles that formed with $uv$ and the light edges which have been sampled.

For the 4-cycles that have heavy wedges, we use an idea proposed in~\cite{McGregor2020, SV20}: for any node pair $u$ and $v$, if we know their number of common neighbors (denoted by $k$), we can compute the exact number of 4-cycles with $u, v$ as a diagonal pair (i.e.,  the four cycle contains two wedges with the endpoints $u, v$), and this counts to $\binom{k}{2}$. Furthermore,
if $k$ is large (in this case we say all the wedges with endpoints $u,v$ are heavy), we can detect it and obtain a good estimation to $k$ by a similar vertex sampling method mentioned in Section~\ref{sec:arbitrary_main}.
%(at the beginning of the stream, we sample a node set $S$ and then during the stream we save the edges that are incident to $S$). 
We can then estimate the total number of 4-cycles that have heavy wedges with our samples. 
%A problem here is if a 4-cycle is involved in two heavy diamonds, it will be counted twice. However, ~\cite{SV20} shows this double-counting is at most $O(T^{3/2}) = O(\epsilon T)$ which means we can ignore this kind of double-counting. 

At this point, we have not yet estimated the number of 4-cycles having more than one heavy edge but without heavy wedges. However, \cite{McGregor2020} shows this class of 4-cycles only takes up a small fraction of $T$, and hence we can get a $(1 \pm \epsilon)$-approximation to $T$ even without counting this class of 4-cycles.
\begin{algorithm}[!t]
   \caption{Counting 4-cycles in the Arbitrary Order Model}
   \label{alg:3}
\begin{algorithmic}[1]
\STATE {\bfseries Input:} Arbitrary Order Stream and an oracle that outputs \textsc{true} if $N_{xy} \ge T / \rho$ and \textsc{false} otherwise.
   \STATE {\bfseries Output:} An estimate of the number $T$ of 4-cycles.
   \STATE Initialize $A_l \leftarrow 0$, $A_h \leftarrow 0$, $A_w \leftarrow 0$ $E_L \leftarrow \emptyset$ $E_H \leftarrow \emptyset$, $E_S \leftarrow \emptyset$, and $W \leftarrow \emptyset$. Set $\rho \leftarrow T^{1/3} $, $p \leftarrow \alpha \epsilon^{-2} \log n / \rho$ for a sufficiently large $\alpha$, and Let $S$ be a random subset of nodes such that each node is in $S$ with probability $p$. %Let edge set $E_1 \leftarrow \emptyset and E_2 \leftarrow \emptyset$
   \WHILE{seeing edge $uv$ in the stream}
   \IF{$u \in S$ or $v \in S$}
    \STATE $E_S \leftarrow \{uv\} \cup E_S$ \; .
   \ENDIF
   \IF{the oracle outputs \textsc{FALSE}}
   \STATE With probability $p$, $E_L \leftarrow \{uv\} \cup E_L$ \; .
   \STATE Find pair $(w,z)$ such that $uw, wz,  \ \textnormal{and} \ zv \in E_L $, let $D \leftarrow D \cup \{(u,w,z,v)\}$ \; .
   \ELSE \STATE $E_H \leftarrow \{uv\} \cup E_H$ \; .
   \ENDIF
   \ENDWHILE
   \FOR{each node pair $(u, v)$}
        \STATE  let $q(u, v)$ be the number of wedges with center in $S$ and endpoints $u$ and $v$.
        \IF{$q(u,v) \ge p T^{1/3}$}
            \STATE $A_w \leftarrow A_w + \binom{q(u,v)}{2}$ \;.
            \STATE $W \leftarrow W \cup \{ (u, v) \}$ \; .
        \ENDIF
   \ENDFOR
   \FOR{each 4-cycle $d$ in $D$}
        \IF{the end points of wedges in $d$ are not in $W$}
            \STATE $A_l \leftarrow A_l + 1$
        \ENDIF
   \ENDFOR
   \FOR{each edge $uv$ in $E_H$}
        \FOR{each 4-cycle $d$ formed with $uv$ and $e \in E_L$} %  edges in
        \IF{the end points of wedges in $d$ are not in $W$}
            \STATE $A_h \leftarrow A_h + 1$
        \ENDIF
        \ENDFOR
   \ENDFOR
   \STATE {\bfseries return:} $A_l / p^3 + A_h / p^3 + A_w$ \; .
\end{algorithmic}
%\vspace{-10pt}
\end{algorithm}

The reader is referred to Algorithm~\ref{alg:3} for a detailed version of our one-pass, 4-cycle counting algorithm. Before the stream, we randomly select a node set $S$, 
where each vertex is in $S$ with probability $p$ independently, 
and we later store all edges that are incident to $S$ during the stream. In the meantime, we define the edge $uv$ to be \textit{heavy} if $N_{uv} \ge T^{2/3}$ and train the oracle to predict whether $uv$ is heavy or not when we see the edge $uv$ during the stream. Let $p = \tilde{O} (\epsilon^{-2} / T^{1/3})$. We store all the heavy edges and sample each light edge with probability $p$ during the stream. Upon seeing see a light edge $uv$, we look for the 4-cycles that are formed by $uv$ and the light edges that have been sampled before, and then record them in set $D$. At the end of the stream, we first find all the node pairs that share many common neighbors in $S$ and identify them as heavy wedges. Then, for each 4-cycle $d \in D$, we check if $d$ has heavy wedges, and if so, remove it from $D$. Finally, for each heavy edge $uv$ indicated by the oracle, we compute the number of 4-cycles that are formed by $uv$ and the sampled light edges, and without heavy wedges. This completes all parts of our estimation procedure. 


We now prove Theorem~\ref{theorem_four_cycle}, restated here for the sake of convenience.
\thmFourCycles*

\begin{proof}
From the Lemma 3 in ~\cite{SV20}, we know that with probability at least $9/10$, we can get an estimate $A_w$ such that
\[
A_w = T_w \pm \epsilon T.
\]
Where $T_w$ is the number of the 4-cycles that have at least one heavy wedge. We note that if a 4-cycle has two heavy wedges, it will be counted twice. However, \cite{SV20} shows that this double counting is at most $O(T^{2/3}) = O(\epsilon)T$. 

For the edge sampling algorithm mentioned in~\ref{sec:four_cycle_intuition}, from the analysis in~\cite{SV20}, we have 
\[
\textbf{Var}[{A_l}/{p^3}] \le O(T / p^3 + T\Delta_E / p + T\Delta_W / p^2)\; .  
\]
Notice that in our algorithm, the threshold of the heavy edges and heavy wedges are $N_{uv} \ge T^{2/3}$ and $N_w \ge T^{1/3}$, respectively, which means $\textbf{Var}[\frac{A_l}{p^3}] = O(\epsilon^2 T^2)$. Hence, we can get an estimate $A_l$ such that with probability at least $9/10$, 
\[
A_l = T_l \pm \epsilon T\;,
\]
where $T_l$ is the number of 4-cycles that have no heavy edges. 
Similarly, we have with probability at least $9/10$, 
\[
A_h = T_h \pm \epsilon T\;,
\]
where $T_h$ is the number of 4-cycles that have at most one heavy edge.

One issue is that the algorithm has not yet estimated the number of 4-cycles having more than one heavy edge, but without heavy wedges. However, from Lemma 5.1 in~\cite{McGregor2020} we get that the number of this kind of 4-cycles is at most $O(T^{5/6}) = O(\epsilon)T$. Hence putting everything together, we have
\[
|A_l/p^3 + A_h/p^3 + A_w - T| \le O(\epsilon) T \;,
\]
which is what we need.

Now we analyze the space complexity. The expected number of light edges we sample is $O(mp) = \tilde{O}(\epsilon^{-2} m / T^{1/3})$ and the expected number of nodes in $S$ and edges in $E_S$ is $O(2mp) = \tilde{O}(\epsilon^{-2} m / T^{1/3})$. The expected number of 4-cycles we store in $D$ is $O(T p^3) = \tilde{O}(\epsilon^{-6})$. We store all the heavy edges, and the number of heavy edges is at most $O(T^{1/3})$. Therefore, the expected total space is $\tilde{O}(T^{1 / 3} + \epsilon^{-2}m / T^{1/3})$.
\end{proof}


==> OldStuff/CMUGang/experiment.tex <==
\section{Experiments}
\label{sec: experiments}
We perform our triangle counting experiments on the following two networks:
\begin{itemize}[topsep = 1 pt]
\setlength{\itemsep}{1pt}
\setlength{\parsep}{0pt}
\setlength{\parskip}{0pt}

    \item \textbf{Twitch}\cite{rozemberczki2019}: A user-user social network of gamers who stream in a certain language. Vertices are the users themselves and the links are mutual friendships between them. Each vertex contains a binary vector of features, based on the games the user played and liked, location of the user, and the user's streaming habits. The entire dataset contains six network graphs for six different languages, and the one that is used for testing our algorithm contains 6549 nodes and 112666 edges.
    % \footnote{http://snap.stanford.edu/data/twitch-social-networks.html}
    \item \textbf{Wikipedia}\cite{MM11}: This is a co-occurrence network of words appearing in the first million bytes of the Wikipedia dump. The network has 4777 nodes, 92406 edges, and 40 different labels associated.
\end{itemize}
\textbf{Experimental Setup}: %The experiment setting is as follows: 
For each of the two networks, we randomly remove $50\%$ of the total edges to be the training data set, and use the remaining edges as the testing data set. For the Twitch network, our set of links that we will try to predict are between two nodes that have a common neighbor in the training network, but do not form a link in the training network. This is about 3.8 million pairs, and we call this the candidate set. We do this for memory considerations. For the remaining node pairs, we set the probability they form a link to be $0$. For the Wikipedia network, we randomly select a link candidate set of size $20$ times the number of edges (about $1$ million pairs) from the entire set of testing links. These link candidate sets will be used by the oracle to determine heaviness. 

% A brief results summary?

\textbf{Training of the Oracle}: Our oracle is based on Link Prediction, where the task is to
estimate the likelihood of the existence of edges or to find missing links in the network. Here we use the method and code proposed in~\cite{ZC18}. For each target link, it will extract a local enclosing subgraph around a node pair, and use a Graph Neural Network to learn general graph structure features for link prediction. For the Twitch network, we use all the training links as the training data for the graph neural network, while for the Wikipedia network, we use $30\%$ of the training links as the training data due to memory limitations. Then, we use this network to do our prediction for all links in our candidate sets for the two networks.

Now we are ready to build our heavy edge oracle. For the adjacency list model, when we see the edge $uv$ in the stream, we know all the neighbors of $u$, and hence, we only need to predict the neighbors of $v$. Let $\mathrm{deg}(v)$ be the degree of $v$ in the training graph. The training graph and testing graph are randomly split. Hence, we can use the training set to provide a good estimation to the degree of $v$.  
Next, we choose the largest $\mathrm{deg}(v)$ edges incident to $v$ from the candidate set, in terms of their predicted likelihood given by the the neural network, as our prediction of $N(v)$, which leads to an estimate of $R_{uv}$. For the arbitrary order model, we use the same technique as above to predict $N(u)$ and $N(v)$, and estimate $N_{uv}$. 

% We show the accuracy of the oracle in Appendix~\ref{appendix:F}.
\begin{figure*}[ht]

\centering
\begin{minipage}{0.45\textwidth}
\vspace{-0.3cm}
\includegraphics[width=7cm]{images/twitch_adj_new.png}
%\hfill
\end{minipage}
\begin{minipage}{0.45\textwidth}
\vspace{-0.3cm}
\includegraphics[width=7cm]{images/Wikipedia_new.png}
\end{minipage}
\caption{Estimation error in the adjacency list model. The left is for Twitch and the right is for Wikipedia.}
\label{fig:1}
\end{figure*}

\begin{figure*}[ht]

\centering

\begin{minipage}{0.45\textwidth}
\vspace{-0.4cm}
\includegraphics[width=7cm]{images/twitch_arb.png}
%\hfill
\end{minipage}
\begin{minipage}{0.45\textwidth}
\vspace{-0.4cm}
\includegraphics[width=7cm]{images/Wikipedia_arb.png}
\end{minipage}

\caption{Estimation error in the arbitrary order model. The left is for Twitch and the right is for Wikipedia.}
\label{fig:2}

\end{figure*}
\subsection{Adjacency List Model}

In the adjacency list model, we compare our learning-based algorithms with the sampling-based algorithms in~\cite{MVV16} by fixing the sampling rate $p$ and comparing the multiplicative error of these two algorithms. 
For the sampling-based algorithm, we know when $R_{uv} \ge \epsilon^{-2} / p$, and so we can obtain a $(1 \pm \epsilon)$-approximation to $R_{uv}$ using the edges we have sampled. However, it is not easy to determine the optimal threshold for $R_{uv}$. To make it easier to compare, we assume that one can obtain the exact value of $R_{uv}$ when $R_{uv} \ge 5 / p$ for the sampling-based algorithm. This assumption will only make the results of the sampling-based algorithm better. 
For the learning-based algorithm, we set the $k = M / 10$ edges with the highest predicted $R_{uv}$ values to be the heavy edges, and store them during the stream, where $M$ is the expected space complexity (i.e., we use $10\%$ of the total space for storing the heavy edges). For the remaining edges, we use a similar sampling-based method. Note that it is impossible to know the $k$-heaviest edges before we see all the edges in the stream. However, in our implementation we can maintain the $k$ heaviest edges we currently have seen so far, and evict the smallest edge in the set when a new heavy edge is predicted by the oracle. We also consider the multi-layer sub-sampling algorithm mentioned in Section~\ref{sec:adj_mul}, which uses more information from the oracle. For this algorithm, we use $10\%$ of the total space for storing the top $k = M / 10$ edges, $20\%$ of the space for sub-sampling the edges $xy$ for which the oracle predicts $R_{xy} \ge 10$ (there are about $10^3$ such edges in both networks), and $70\%$ of the space for sub-sampling the remaining edges. 

The results are shown in Figure~\ref{fig:1}. We plot the estimation error vs. the expected number of edges we store (computed by the sampling rate) where the error takes an average over 1000 independent trials and all trials share a same node arrival order. From the plots we can see our learning-based algorithm can reduce $20\%$-$30\%$ error in all cases for the Twitch network and $30\%$-$40\%$ error for the Wikipedia network. Compared to the learning-based algorithm that just uses the oracle to select the top edges, our multi-layer sampling algorithm can still reduce error by $20\%$-$30\%$ in the Twitch network and reduce error by $10\%$-$20\%$ in the Wikipedia network. We also plot the curve when the oracle is perfectly accurate, and we can see that the performance of our trained oracle is very close to the ideal oracle.

\subsection{Arbitrary Order Model}

In the arbitrary order model, we compare our learning-based algorithm with the one-pass edge sampling algorithm mentioned in section~\ref{sec:arbitrary_triangle_intuition}. In both networks, we say an edge $uv$ is a heavy edge if the prediction value $N_{uv} \ge 60$, which corresponds roughly to the top $100$ edges in the Twitch network and top $200$ in Wikipedia network. For the heavy edge $uv$, we use the prediction $\hat{N}_{uv}$ as our estimate of $N_{uv}$ and $\sum_{uv \textnormal{ is heavy}} N_{uv}$ as our estimate of the number of triangles that have at least one heavy edge (this may cause some triangles to be counted more than once, but the number of the heavy edges is small so we ignore such double counting). We then count the triangles with three light edges with the same edge sampling algorithm. 

The results are shown in Figure~\ref{fig:2}. We plot the estimation error vs. the expected number of edges stored, where the error is calculated by averaging over 100 independent trial streams, each with a random arrival order. From the plot we can see that for the Twitch network, our learning-based algorithm can reduce the error by $10\%$-$20\%$. For the Wikipedia network, the learning-based algorithm can reduce the error by $20\%$-$35\%$.

We also study the relationship between the accuracy and the threshold $k$ we set in the experiments. The results are in Appendix~\ref{appendix:E}.


==> OldStuff/CMUGang/introduction.tex <==

\section{Introduction}
Counting the number of cycles is an extremely important problem in the graph stream model, especially with the special case of counting triangles being one of the most widely studied problems \cite{AGD08, BC17, S13, Kolountzakis_2010, Yossef}. There are a wide range of applications for triangle counting in graph streams, including discovering motifs in protein interaction networks \cite{Milo824}, understanding social networks \cite{Welles10}, and evaluating large graph models \cite{Leskovec08}. It is also closely connected to the field of fine-grained complexity, where studies involve various computational models such as distributed shared-memory and MapReduce \cite{S13, AGD08}. More recently, attention has been focused on the more general problem of counting larger cycles and subgraphs \cite{BC17, KJM19}. 

While detecting whether a graph contains a triangle or four-cycle is not possible in sublinear space with constant probability of success, a lot of work has been focused on computing a $(1 \pm \epsilon)$-approximation to the subgraph count $T$ using a small space randomized algorithm. A common difficulty in designing these algorithms is that the edges that are involved in a lot of triangles or four-cycles, i.e., the \textit{heavy} edges, are not known in advance. For a sub-sampling algorithm, these edges are often the key to accurate estimation, and people have developed multiple techniques to determine whether an edge is heavy such as processing a smaller subset of the stream as an oracle in the random order model \cite{McGregor2020, BS20} or using more passes \cite{MVV16}. 

Recently, machine learning techniques were incorporated into the data stream model, with the training of a heavy-hitter oracle, based on the observation that many underlying patterns in real world data sets such as the heavy link in a network does not change from day-to-day \cite{hsu2018}. It turns out that with the assistance of such a learning-based supporting oracle, a wide range of significant problems in big data processing, including estimating the number of distinct elements, computing the $F_p$-Moment, calculating the $(k,p)$-Cascaded Norm, support estimation, and nearest neighbor search, can all achieve better or even optimal space bounds, see, e.g., \cite{Jiang2020, EINR+2021, Dong2020}. 

One may wonder whether such techniques can be applied to the problem of subgraph counting. Namely, 
\begin{quote}
\em   
Is it possible to train a heavy edge oracle, and how does it improve the space complexity of subgraph counting in the graph stream model?
\end{quote}
% We consider estimating triangles and four cycles in the following two graph stream models:
% \begin{itemize}
%     \item 
%     Adjacency List Model: the edges incident to the same node arrive together.
%     \item
%     Arbitrary Order Model: the edges arrive in arbitrary order. 
% \end{itemize}
\subsection{Our Results and Comparison to Previous Work}

There are two major graph edge streaming models: the adjacency list model and arbitrary order models.
We show that the training of a heavy edge oracle is possible in practice, and it can lead to new algorithms that greatly improve the space complexity of triangle and four-cycle counting under both models.

\textbf{Adjacency List Model}. In the adjacency list model, the edges incident to the same node arrive together.
The best existing one-pass, $(1 \pm \epsilon)$-approximation algorithm for triangle counting has space complexity $\tilde{O}(\epsilon^{-2} m/\sqrt{T})$\footnote{ We use $\tilde{O}(f)$ to denote $O(f \mathrm{polylog}(f))$} \cite{MVV16}. Our first result is as follows: 

\textbf{Theorem~\ref{theorem_adjacency}}
\textit{There exists a one-pass algorithm with space complexity $\tilde{O}( \min(\epsilon^{-2}m^{2/3}/T^{1/3}, \epsilon^{-1} m^{1/2}))$ in the adjacency list model using a learning-based oracle that returns a $(1 \pm \epsilon)$-approximation to T with probability $7 / 10$. \footnote{the success probability can be replaced by $1 / \delta$ by running $\log(1/\delta)$ copies of the algorithm and taking the median.}  }


We also study the case when the oracle cannot only indicate an edge is heavy or not, but give an  $\alpha$-approximation to the value of the heavy edges. 
%We also show a lower bound for this setting.
%and show that a lower order bound could be achieved in theory.

\textbf{Arbitrary Order Model}. In the arbitrary order model, the edges arrive in the stream in an arbitrary order. 
In this model, we present a one-pass algorithm for triangle counting and another one-pass algorithm for four cycle counting, both reducing the number of passes from the algorithms with the currently best known space complexity. 

For triangle counting in this model, the best known space complexity for a general graph is $\tilde{O}(\epsilon^{-2}m^{3/2}/T)$ with three passes, or $\tilde{O}(\epsilon^{-2}m/\sqrt{T})$ using two passes \cite{MVV16}. Other results often contain specific parameters of the graph, including an $\tilde{O}(\epsilon^{-2}(m/\sqrt{T} + m \Delta_E / T))$ space bound using one pass\cite{PT12}, an  $\tilde{O}(\epsilon^{-2}(m/T^{2/3} + m \Delta_E / T + \sqrt{\Delta_V} / T))$ space bound using one pass\cite{KP17}, where $\Delta_E$ and $\Delta_V$ mean the maximum number of triangles sharing an edge or a vertex, respectively, and an almost tight bound of $\Tilde{O}(\mathrm{poly}(\epsilon^{-1})m\kappa/T)$, where $\kappa$ is the degeneracy of the graph, but requiring a constant number of passes \cite{BS20}. Our next result is as follows: 

\textbf{Theorem~\ref{theorem_arbitrary}}
\textit{There exists a one-pass algorithm with space complexity $\tilde{O}(\epsilon^{-2}\max(m/\sqrt{T}, \sqrt{m}))$ in the arbitrary order model using a learning-based oracle that returns a $(1 \pm \epsilon)$-approximation to T with probability at least $7 / 10$.
}

We also show a lower bound for this setting(Theorem~\ref{thm:lower_bound_arbitrary}).

For four cycle counting, the best existing bound for a $(1 \pm \epsilon)$-approximation is $\tilde{O}(\epsilon^{-4}m/T^{1/2})$ using 2 passes and $\tilde{O}(\epsilon^{-2}m/T^{1/3})$ using 3 passes \cite{McGregor2020, SV20}. We design our algorithm based on the 3-pass algorithm with a trained oracle for predicting heavy edges. We show:

\textbf{Theorem~\ref{theorem_four_cycle}}
\textit{
There exists a one-pass algorithm with space complexity $\tilde{O}(T^{1 / 3} + \epsilon^{-2}m / T^{1/3})$ in the arbitrary order model using a learning-based oracle that returns a $(1 \pm \epsilon)$-approximation to $T$ with probability at least $7 / 10$.}

We refer the reader to Table~\ref{comparison-table} for a summary of our results in comparison to prior work.

\textbf{Experiments.}
We conduct experiments to verify our results for triangle counting using two real world networks: a Twitch user-user social network and a word co-occurrence network from Wikipedia. In the training of the heavy edge oracle, we apply the method of link prediction \cite{ZC18}. 
%In particular, we first train a degree predictor for each vertex, and upon seeing edge $xy$, we perform link prediction on a target set of vertices to estimate whether $xy$ have a large number of common neighbors, which serves as our heavy edge oracle. 
More details of our experiments will be discussed in Section~\ref{sec: experiments}.

We found that in the adjacency list model, when using the same amount of memory, our learning-augmented algorithm reduces the error by $20\%$-50$\%$ compared to the baseline algorithm without learning. In the arbitrary order model, our algorithm can reduce the error by around $20\%$ when using the same amount of space compared to the non-augmented %$\tilde{O}(m/\sqrt{T})$ algorithm while using only 
$\tilde{O}(\epsilon^{-2}(m/\sqrt{T} + m \Delta_E / T))$ one-pass edge sampling algorithm. 

\begin{table}[t]
% \vspace{-3pt}
\caption{Our results compared to existing algorithms}
\label{comparison-table}

\begin{center}

\begin{tabular}{ | m{4em} | m{8em}| m{8em} | } 

\hline
Problem & Previous Results & Our Results \\
\hline
\multirow{2}{4em}{Triangle, Adjacency} & \multirow{2}{8em}{$\tilde{O}(\epsilon^{-2} m/\sqrt{T})$} &  $\tilde{O}(\min(\epsilon^{-2}\frac{m^{2/3}}{T^{1/3}},$ \\
& & $\epsilon^{-1} m^{1/2}))$ \\
\hline

\multirow{12}{4em}{Triangle, Arbitrary}& 
\multirow{2}{8em}{$\tilde{O}(\epsilon^{-2}m^{3/2}/T)$, 3-pass}& \multirow{12}{8em}{$O(\epsilon^{-2}\max(m/\sqrt{T},$ $m^{1/2}))$, 1-pass} \\
& & \\
& \multirow{2}{8em}{$\tilde{O}(\epsilon^{-2}m/\sqrt{T})$, 2-pass} & \\
& & \\
& \multirow{3}{8em}{$\tilde{O}(\epsilon^{-2}(m/\sqrt{T} + m \Delta_E / T))$, 1-pass} & \\
& & \\
& & \\
& \multirow{3}{8em}{$\tilde{O}(\epsilon^{-2}(m/T^{2/3} + m \Delta_E / T + \sqrt{\Delta_V} / T))$, 1-pass} & \\
& & \\
& & \\
& \multirow{3}{8em}{$\Tilde{O}(\mathrm{poly}(\epsilon^{-1})m\kappa/T)$, multi-pass} & \\
& & \\
& & \\
\hline

\multirow{6}{4em}{4-cycle, Arbitrary} &
\multirow{3}{8em}{$\tilde{O}(\epsilon^{-4}m/T^{1/2})$, 2-pass} &
\multirow{6}{8em}{$\tilde{O}(T^{1/3} + \epsilon^{-2}m/T^{1/3})$, 1-pass} \\
& & \\
& & \\
& \multirow{3}{8em}{$\tilde{O}(\epsilon^{-2}m/T^{1/3})$, 3-pass} & \\
& & \\
& & \\
\hline
\end{tabular}

\end{center}
\vspace{-20pt}
\end{table}

==> OldStuff/CMUGang/new_value_prediction.tex <==
\section{New Value Prediction Oracle for Adjacency List Model}
\label{sec:value_oracle}

In this section, we consider the following oracle model.

\textbf{Definition~\ref{def:value_oracle}}
\textit{
A value-prediction oracle with parameter $(\alpha,\beta)$ can, for a given edge $e$, 
%indicate if (i) $R_{xy} \le T / \beta$, or (ii) $R_{xy} > T / \beta$, and 
output a value $p(e)$ for which $\alpha t(e) + \beta \ge \mathbb{E}[p(e)]$, and $\mathbf{Pr}[p(e) < \frac{t(e) - \beta}{\lambda}] \le e^{-\lambda}$.
%$\alpha$-approximation of $R_{xy}$ .
}

Our algorithm is based on the following stability property of exponential random variables (see e.g.~\cite{Andoni17})

\begin{lemma}
\label{lem:exp_stable}
Let $x_1, x_2, ..., x_n > 0$ be real numbers, and let $u_1, u_2, ...u_n$ be i.i.d. standard exponential random variables with parameter $\lambda = 1$. Then we have that the random variable $\max(\frac{x_1}{u_1}, ..., \frac{x_n}{u_n}) \sim \frac{x}{u}$, where $x = \sum_i x_i$ and $u \sim \mathrm{Exp}(1)$.
\end{lemma}

\begin{lemma}
\label{lem:exp_median}
Let $r = O(\ln(1 / \delta) / \epsilon^{2})$ and $\epsilon \le 1/3$. If we take $r$ independent samples $X_1, X_2, ... , X_r$ from $\mathrm{Exp}(1)$ and let $X = \mathrm{median}(X_1, X_2, ..., X_r)$, then with probability $1 - \delta$, $X \in [\ln{2}(1-\epsilon), \ln{2}(1 + 5\epsilon)]$.
\end{lemma}
\begin{proof}
We first prove the following statement: with probability $1-\delta$, $F(X) \in [1/2-\epsilon, 1/2 + \epsilon]$, where $F$ is the cumulative density function of a standard exponential random variable.

Consider the case when $F(X) \le 1/2 - \epsilon$. We use the indicator variable $Z_i$ where $Z_i = 1$ if $F(X_i) \le 1/2 - \epsilon$ or $Z_i = 0$ otherwise. Notice that when $F(X) \le 1/2 - \epsilon$, at least half of the $Z_i$ are $1$, so $Z = \sum_i Z_i \ge r / 2$. On the other hand, we have $\mathbb{E}[Z] = r / 2 - r \epsilon$, by a Chernoff bound. We thus have 
\[
\mathbf{Pr}[|Z - \mathbb{E}[Z]| \ge \epsilon r] \le 2e^{-\epsilon^{2}r/3} \le \delta / 2\; .
\]
Therefore, we have with probability at most $\delta/2$, $F(X) \le 1/2 - \epsilon$. Similarly, we have that with probability at most $\delta / 2$, $F(X) \ge 1/2 + \epsilon$. Taking a union bound, we have that with probability at least $1-\delta$, $F(X) \in [1/2-\epsilon, 1/2 + \epsilon]$.

Now, condition on $F(X) \in [1/2-\epsilon, 1/2 + \epsilon]$. Note that $F^{-1}(x) = -\ln(1 - x)$, so if we consider the two endpoints of $F(X)$, we have 
\[
F^{-1} (1/2 -\epsilon) = -\ln(1/2 + \epsilon) \ge (1-\epsilon)\ln{2},
\]
and
\[
F^{-1} (1/2 +\epsilon) = -\ln(1/2 - \epsilon) \le (1+5\epsilon)\ln{2}.
\]
which indicates that $X \in [\ln{2}(1-\epsilon), \ln{2}(1 + 5\epsilon)]$.
\end{proof}

The algorithm is shown in Algorithm~\ref{alg:4}. For the light edges, from the assumption of the oracle we know that $R_{xy} \le T / \beta$, we can sub-sample with sampling rate $O(\epsilon^{-2} \beta)$ to estimate $T_L$. For the heavy edges, we can obtain an $\alpha$-approximation to $R_{xy}$ from the oracle at this time. As shown in our algorithm, we run $O(\epsilon^{-2})$ copies of the subroutine and we will show that each subroutine will output the maximum value of $R_{xy} / u_{xy}^i$ with high probability, where the $u_{e}^i$ are exponential random variables. From Lemma~\ref{lem:exp_stable} and Lemma~\ref{lem:exp_median} we can obtain $O(\epsilon^{-2})$ independent samples from $T_H / u$, where $u \sim \mathrm{Exp}(1)$, and after taking a median among all samples we can obtain a $(1 \pm \epsilon)$-approximation to $T_H$.

\begin{algorithm}[!h]
   \caption{Counting Triangles in the Adjacency List Model with a Value Prediction Oracle}
   \label{alg:4}
\begin{algorithmic}[1]
   \STATE {\bfseries Input:} Adjacency list edge stream and an value prediction oracle with parameter$(\alpha, \beta)$. 
   \STATE {\bfseries Output:} An estimate of the number $T$ of triangles.
   \STATE Initialize $X \leftarrow \emptyset$ and $H = O(\epsilon\alpha)$\; .
   %\STATE On :$H = O(T)$
   \FOR{$i = 0$ {\bf to} ${O(\epsilon^{-2})}$}
        \STATE $S^{i} \leftarrow \emptyset, Q^{i} \leftarrow \emptyset$, and $A^i \leftarrow 0 $ \; .
        % \STATE $v_i \leftarrow 0$ \textnormal{as the maximum value in $Q^i$} \; .
        % \STATE $w_i \leftarrow 0$ \textnormal{as the minimum value in $Q_i$} \;%\textnormal{as the evict threshold in $Q^i$} 
        \STATE \textnormal{Generate} $u_{xy}^i \sim \textrm{Exp}(1)$ for all $x$ and $y$ \; . 
   \ENDFOR
    \WHILE{seeing edges adjacent to $y$ in the stream} \STATE For all $ab \in S_L$: if $a, b \in N(y)$ then $C_{ab} \leftarrow C_{ab} + 1$\; 
    % \FOR{$i = 0$ {\bf to} ${O(\epsilon^{-2})}$}
    \STATE For all $ab \in S^i$: if $a, b \in N(y)$ then $C_{ab}^i \leftarrow C_{ab}^i + 1$\; 
    %  \ENDFOR
    \FOR{each incident edge $yx$}
    
    \IF{the oracle outputs \textsc{True}}
    \IF{$xy \in S_L$} 
        \STATE $A_l \leftarrow A_l + C_{xy}$ \;.
    \ELSE 
    \STATE With probability $p_l$, $S_L \leftarrow \{yx\} \cup S_L$ \;.
    \ENDIF
    \ELSE 
        \FOR{$i = 0$ {\bf to} ${O(\epsilon^{-2})}$} 
            \IF{$xy \in S^i$} 
            \STATE $A^i \leftarrow \max(A^i,  C_{xy}^i / u_{xy}^i)$ \;.
            \ELSE
            \STATE Let $\hat{R}_{yx}$ be the predicted value of $R_{yx}$.
            \STATE $Q^i \leftarrow Q^i \cup \{\hat{R}_{yx}/u_{yx}^i\}, S^i \leftarrow S^i \cup \{xy\}$
            \IF{$|Q| > k$}
            \STATE Let $ab$ be the edge for which $\hat{R}_{ab} / u_{ab}^i$ is the smallest item in $Q^i$
            \STATE $Q^i \leftarrow Q^i / \{\hat{R}_{ab}/u_{ab}^i\}, S^i \leftarrow S^i / \{ab\}$
            \ENDIF
            \ENDIF
    \ENDFOR
    
    \ENDIF
    \ENDFOR
    \ENDWHILE
    \FOR{$i = 0$ {\bf to} ${O(\epsilon^{-2})}$}
        \STATE $u^i \leftarrow \max(Q^i)$ and $v^i \leftarrow \min(Q^i)$  \; .
        \IF{$u^i > \alpha v^i$}
        \STATE $X \leftarrow X \cup \{A^i\}$
        \ENDIF
   \ENDFOR
    \STATE {\bfseries return:} $A_l / p_l + \mathrm{median}(X) / \ln{2}$ \; .
\end{algorithmic}
\end{algorithm}

\textbf{Theorem~\ref{thm:value_oracle}}
\textit{
Given an oracle with parameter $(\alpha, \beta)$, there exists a one-pass algorithm with space complexity $O(\epsilon^{-2} (m / \beta + \alpha + \log n(\log\log n)^2))$ in the adjacency list model that returns a $(1 \pm \epsilon)$-approximation to $T$ with probability at least $7 / 10$. 
}

\begin{proof}
For the light edges, from Lemma~\ref{lem:adjlist_light} we get that with probability at least $9/10$, 
\[
A_l / p_l = T_L \pm \epsilon T \;.
\]
Now we focus on estimating $T_H$. It is easy to see that for the $i$-th subroutine, $Q^i$ and $S^i$ sample the edge $xy$ for which $\hat{R}_{xy} / u_{xy}^i$ is among the current top $k$ values we have seen. At the end of the stream, $Q^i$ and $S^i$ sample edge $xy$ for which $\hat{R}_{xy} / u_{xy}^i$ is among the top $k$ largest values among all edges. If the edge $ab$, for which the true value $R_{ab} / u_{ab}^i$ is the maximum value among $E$, is included in $S^i$, then the output of the $i$-th subroutine will be a sample from $T_H / u$, where $u \sim \mathrm{Exp}(1)$. Recall that $\hat{R}_{xy}$ is an $\alpha$-approximation to $R_{xy}$, and hence we have that 
\[
\max_{xy \in E} \hat{R}_{xy} / u_{xy}^i \le \alpha \hat{R}_{ab} / u_{ab}^i \;,
\]
which means if $u_i \ge \alpha v_i$ ($u_i$ and $v_i$ are the maximum and minimum values in $Q^i$ after the stream), then $ab$ should be included in $S^i$.

From Claim~2.1 in~\cite{Andoni17}, for each subroutine $i$, in expectation there will be at most $O(\alpha)$ edges $wz$ satisfying 
\[
\max_{xy \in E} \hat{R}_{xy} / u_{xy}^i \le \alpha \hat{R}_{wz} / u_{wz}^i \;,
\]
Hence, using Markov's inequality, with probability at least $9 / 10$, $u_i > \alpha v_i$ holds for the $i$-th subroutine (this is because, at this time there are at most $O(\alpha)$ edges within an $\alpha$ factor of $\max_{xy \in E} \hat{R}_{xy} / u_{xy}^i$, and $v_i$ is the $k = l \alpha$ largest edge). Therefore, in expectation there will be at least a $9/10$-fraction of our total  $O(\epsilon^{-2})$ number of subroutines which can output a sample drawn from $T_H / u$. From Lemma~\ref{lem:exp_median}, we get that after taking a median, we obtain a $(1 \pm O(\epsilon))$-approximation to $T_H$.

Next we analyze the space complexity. For the light edges, we sample each edge with probability $O(\epsilon^{-2}/\beta)$, and hence the expected space we use is $O(\epsilon^{-2} m / \beta)$. For the heavy edges, we run $O(1/\epsilon^{2})$ subroutines and the number of edges each subroutine stores is $O(\alpha)$. From Theorem~5 in \cite{JW18}, generating the exponential random variables can be derandomized in $O(\epsilon^{-2} (\log n (\log\log n)^2))$ space. Therefore, we get that the total expected space we use is $O(\epsilon^{-2}(m / \beta + \alpha + \log n (\log\log n)^2))$.
\end{proof}

\begin{remark}
An alternative way to solve this problem is to divide the triangles into the intervals $[0, T/\beta], [2T/ \beta, 4T/ \beta],..., [2^i T/\beta, 2^{i+1} T / \beta], ...$ and put the edges into the intervals according to the predicted value the oracle gives. For the edges in interval $[2^i T / \beta, 2^{i + 1} T / \beta]$, we can sub-sample with rate $O(\epsilon^{-2} \alpha 2^{i + 1} /\beta )$. The total space we use will be $\tilde{O}(\epsilon^{-2} (m / \beta + \alpha \log n))$.
\end{remark}

==> OldStuff/MITGang/preamble.tex <==
%packages

\usepackage{amsthm}
\usepackage{mathtools} 
\usepackage{paralist}
\usepackage[colorlinks,urlcolor=blue,citecolor=blue,linkcolor=blue]{hyperref}
\usepackage{xcolor,soul}


%comments
\DeclareRobustCommand{\hltalya}[1]{{\sethlcolor{yellow}\hl{#1}}}
\newcommand{\tnote}[1]{\hltalya{[\textbf{T}: #1]}}

%theorems and proofs
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{notation}[theorem]{Notation}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{claim}[theorem]{Claim}
%\theoremstyle{remark}
\newtheorem{remark}{Remark}

%shortcuts
\newcommand{\eps}{\epsilon}
\newcommand{\mO}{\mathcal{O}_\theta}
\newcommand{\heavy}{\textsf{heavy}}
\newcommand{\light}{\textsf{light}}
\newcommand{\mT}{\mathcal{T}}
\newcommand{\mH}{\mathcal{H}}
\newcommand{\mS}{\mathcal{S}}
\newcommand{\oT}{\overline{T}}

%procedures
\newcommand{\AT}{\hyperref[AT]{\textup{\color{black}{\sf Approx-Triangles}}}}

%useful
\newcommand{\EX}{\textbf{\textrm{Ex}}}
\newcommand{\Var}{\textbf{\textrm{Var}}}
\newcommand{\Cov}{\textbf{\textrm{Cov}}}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\paren}[1]{\left(#1\right)}
\newcommand{\set}[1]{\left\{#1\right\}}
\newcommand{\sqb}[1]{\left[#1\right]}
\newcommand{\sucht}{\,\middle|\,}
\renewcommand{\th}{^{\textrm{th}}}
\newcommand{\poly}{\textrm{poly}}
